FedPerm: Private and Robust Federated Learning by Parameter Permutation

Federated Learning (FL) is a distributed learning paradigm that enables mutually untrusting clients to collaboratively train a common machine learning model. Client data privacy is paramount in FL. At the same time, the model must be protected from poisoning attacks from adversarial clients. Existing solutions address these two problems in isolation. We present FedPerm, a new FL algorithm that addresses both these problems by combining a novel intra-model parameter shuffling technique that amplifies data privacy, with Private Information Retrieval (PIR) based techniques that permit cryptographic aggregation of clients' model updates. The combination of these techniques further helps the federation server constrain parameter updates from clients so as to curtail effects of model poisoning attacks by adversarial clients. We further present FedPerm's unique hyperparameters that can be used effectively to trade off computation overheads with model utility. Our empirical evaluation on the MNIST dataset demonstrates FedPerm's effectiveness over existing Differential Privacy (DP) enforcement solutions in FL.

==> FedPerm/AdvFedPerm.tex <==
\section{Computation/Communication and Utility Tradeoff in \Name}
\label{sec:FedpermAdv}

%\subsection{Privacy and Computation/Communication Cost in \Name}

Each \Name client perturbs its local update (vector $x_i$ containing
$d$ parameters) with randomizer $\mathcal{R}^d$ which is
$\varepsilon_d$-LDP, and then shuffles its parameters.  We use the
Laplacian mechanism as the randomizer.  Based on the n\"aive
composition theorem from Lemma~\ref{lemma-PrivacyFold1}, the
client perturbs each parameter value with $\mathcal{R}$ which
satisfies $\varepsilon_{wd}$-LDP where
$\varepsilon_{wd}=\frac{\varepsilon_d}{d}$ (Appendix~\ref{sec:Laplace}
contains additional details).  Corollary~\ref{coll-FedPermDP11} shows
the privacy amplification from $\varepsilon_d$-LDP to
$(\varepsilon_{\ell}, \delta_{\ell})$-DP after the parameter
shuffling.  Corollary~\ref{coll-FedPermDP11} is derived from
Corollary~\ref{coll-blanket-balle-generic}, by substituting the number
of participating clients $n$ by the number of parameters $d$ in the
model.

\begin{corollary}
If $\mathcal{R}$ is $\varepsilon_{wd}$-LDP, where $\varepsilon_{wd} \leq
\log{(d / \log{(1/\delta_{\ell})})}/2$, \Name $\mathcal{F}=\mathcal{A}
\circ \mathcal{S}_{d} \circ \mathcal{R}^d$ satisfies
$(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O(
(1 \wedge \varepsilon_{wd}) e^{\varepsilon_{wd}}
\sqrt{\log{(1/\delta_{\ell})}/d})$.
\label{coll-FedPermDP11}
\end{corollary}

Thus, larger the number of parameters in the model, greater is the
privacy amplification.  With large models containing millions or
billions of parameters, the privacy amplification can be immense.
However, the model dimensionality also affects the computation (and
communication) cost in \Name.  Each \Name client generates a
$d$-dimensional PIR query for every parameter in the model, resulting
in a PIR query matrix containing $d^2$ entries.  This results in a
quadratic increase in client encryption time, server aggregation time,
and client-server communication bandwidth consumption.  This increase
in communication, and more importantly computation, resources is
simply infeasible for large models containing billions of parameters.
To address this problem \Name introduces additional hyperparameters
that present an interesting trade off between
computation/communication overheads and model utility.

\begin{comment}
\subsection{Computation/Communication Cost of \Name}



In this section, we first show the privacy level and
computation/communication cost of \Name and then introduce new
hyperparameters for \Name to adjust the computation/communication cost
vs.  utility tradeoff.  In particular, for a fixed privacy budget, if
we increase the computation and communication resources, we can train
a more accurate model as we need to inject less local noise (as the
result of privacy amplification of shuffling the parameters).
Corollary~\ref{coll-FedPermDP11} shows the privacy amplification from
$\varepsilon_d$-LDP to $(\varepsilon_{\ell}, \delta_{\ell})$-DP after
the parameter shuffling.  Corollary~\ref{coll-FedPermDP11} is derived
from Corollary~\ref{coll-blanket-balle-generic}, by substituting the
number of participating clients $n$ by the number of parameters $d$ in
the model.


\subsection{Privacy vs.  Computation/Communication in \Name}

Each \Name client perturbs its local update (vector $x_i$ containing
$d$ parameters) with randomizer $\mathcal{R}^d$ which is
$\varepsilon_d$-LDP, and then shuffles its parameters.  We use Laplace
Mechanism as the randomize function $\mathcal{R}$ in \Name design.
Based on the na\"ive composition theorem described in
Lemma~\ref{lemma-PrivacyFold1}, the client perturbs each parameter
value with $\mathcal{R}$ which satisfies $\varepsilon_{wd}$-LDP where
$\varepsilon_{wd}=\frac{\varepsilon_d}{d}$.  We explain more about
this parameter randomizing in Appendix~\ref{sec:Laplace}.
Corollary~\ref{coll-FedPermDP11} shows the privacy amplification from
$\varepsilon_d$-LDP to $(\varepsilon_{\ell}, \delta_{\ell})$-DP after
the parameter shuffling.  Corollary~\ref{coll-FedPermDP11} is derived
from Corollary~\ref{coll-blanket-balle-generic}, where in \Name we are
\emph{intra-model} parameter shuffling instead of \emph{inter-model}
client update shuffling in Corollary~\ref{coll-FedPermDP11}.  This
means in \Name, the number of clients participating in shuffling ($n$)
will be replaced by number of parameters ($d$).




\begin{corollary}
If $\mathcal{R}$ is $\varepsilon_{d}$-LDP, where $\varepsilon_{d} \leq \log{(d / \log{(1/\delta_{\ell})})}/2$,
\Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{d} \circ \mathcal{R}^d$ satisfies $(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}) e^{\varepsilon_{d}} \sqrt{\log{(1/\delta_{\ell})}/d})$.
\label{coll-FedPermDP11}
\end{corollary}



In \Name, each client encrypts $d^2$ values of $\{0,1\}$ for PIR query
generation, and it consumes $O(d^2)$ extra upload bandwidth to send
the PIR query along with the shuffled parameters.  This makes the
client encryption time, server aggregation time, and client upload
bandwidth consumption increase quadratically with $d$ (number of
parameters).
%Table~\ref{tab:FedpermResult1} shows encryption time (at clients),
%server aggregation time, and decryption time at clients for different
%values of $d$.
Existing deep neural networks have a large number of parameters which
makes the \Name very expensive.  In following, we present
computation/communication-utility tradeoff hyperparameters for \Name
to adjust the computation/communication burden for a proper utility
goal.
 %introduce additional mechanisms to decrease these costs.

\end{comment}


%###############################k1###########################

\subsection{\Name with Smaller Shuffling Pattern}

%In \Name, each client generates $d$ PIR queries, that each one
%requires $d$ encryptions.  To reduce the size of each PIR query, we
%need to reduce the size of shuffling patterns ($\pi_u$ for user $u$),
%which is secret for each client.  To do so,

Instead of shuffling all the $d$ parameters, the \Name client can
partition its parameters into several identically sized windows, and
shuffle the parameters in each window with the \emph{same} shuffling
pattern.  Thus, instead of creating a very large random
shuffling pattern $\pi$ with $d$ indices (i.e.,
$\pi=\textsc{RandomPermutations}[1,d]$), each client creates a
shuffling pattern with $k_1$ indices (i.e.,
$\pi=\textsc{RandomPermutations}[1,k_1]$), and shuffles
($\mathcal{S}_{k_1}$) each window with these random indices.
%Note that the same shuffling pattern will be applied inside each
%window.

The window size $k_1$ is a new \Name hyperparameter that can be used
to control the computation/communication and model utility trade off.
%Now, we can adjust \Name computation and communication cost by
%choosing a proper window size ($k_1$).
Once we set the size of shuffling pattern to $k_1$, each client needs
to perform $d \cdot k_1$ encryptions and consumes $O(d \cdot k_1)$
network bandwidth to send its PIR queries to the server.
%Note that \Name without window size means $k_1=d$.  By random
%guessing, the adversary's success rate of finding the right order of
%parameters in \Name is $\frac{1}{d!}$ as there are $d!$ possible
%permutation of parameters.  When we are shuffling with smaller
%shuffling pattern with $k_1$ indices, the adversary's success
%probability of finding the original order is $\frac{1}{k_1!}$.


\paragraphb{Superwindow:} A shuffling window size of $k_1$, partitions
each \Name client $u$'s local update $x_u$ ($d$ parameters) into
$w=d/k_1$ windows, each containing $k_1$ parameters.  Each \Name
client, independently from other \Name clients, chooses its shuffling
pattern $\pi$ uniformly at random with indices $\in [1,k_1]$, and
shuffles each window with this pattern.  This means that every
position $j$ ($1\le j \le k_1$) in each window $k$ ($1\le k \le w$)
will have the same permutation index ($\pi_j$).  Thus all of the
$j^{th}$ positioned parameters ($x_u^{(k,j)} \; \text{for} \; 1\le k
\le w$) will contain the value from the $\pi_j^{th}$ slot in window
$k$.
%be shuffled with the same pattern $\pi_j$.
For a given index $j$ ($1\le j \le k_1$), we define a
\emph{superwindow} as the set of all of the parameters $x_u^{(k,j)}$
for $1\le k \le w$.  If we structure the parameter vector $x_u$ (with
$d$ parameters) as $\mathbb{R}^{k_1 \times w}$ (a matrix with $k_1$
rows and $w$ columns), each row of this matrix is a superwindow.


%The local update $\theta$ with $d$ parameters can be seen as a set of
%windows where we have $w=d/k_1$ windows and each window has $k_1$
%parameters.  If we look at the update $\theta$ with $d$ parameters as
%$\mathbb{R}^{k_1 \times w}$ (a matrix with $k_1$ rows and $w$
%columns), we define \emph{superwindow} as each row of this matrix.
%It means that the parameters inside each superwindow gets permuted
%with the same shuffling pattern.

\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{Images/superwindow.pdf} 
\vspace{-0.15in}
\caption{\Name example with $k_1=3$ and $d=12$. The red boxes are
  showing the windows that the parameters inside them are going to be
  shuffled with the same shuffling pattern $\pi$.}
\label{fig:example}
\end{figure}

Figure~\ref{fig:example} depicts an example model containing $12$
parameters $\theta=[\theta_1, \theta_2, ..., \theta_{12}]$.  The
original \Name algorithm mandates a shuffling pattern $\pi$ with $12$
indices $\in [1,12]$, where the PIR query generates $12\times12=144$
encryptions.  However, a shuffling pattern $\pi$ of three indices
$k_1=3$ ($\pi=[3,1,2]$ in the figure) requires only $3\times3=9$
encryptions.  This shuffling pattern creates $4$ windows of size $3$
(red boxes in the 2-D matrix in the figure), and each row in the 2-D
matrix, represented more succintly by $[\Theta_A,\Theta_B,\Theta_C]$,
itself constitutes a superwindow.  The shuffling pattern $\pi=[3,1,2]$
applied to $\theta = [\Theta_A,\Theta_B,\Theta_C]$ swaps entire
superwindows to give $\mathcal{S}_{k_1}(\theta) =
[\Theta_C,\Theta_A,\Theta_B]$.


\begin{comment}

\paragraphb{Example:} Suppose one client has a model update of 12
parameters $\theta=[\theta_1, \theta_2, ..., \theta_{12}]$.  If we
want to use the original \Name, the client needs to create a shuffling
pattern $\pi$ with 12 indices $\in [1,12]$, where in PIR query
generation it needs, $12\times12=144$ encryptions.  However, if the
client create a shuffling pattern of three indices (e.g,$\pi=[3,1,2]$
with $k_1=3$), then it only requires $3 \times 3=9$ encryptions.
Figure~\ref{fig:example} shows how the client breaks the update
parameters into windows for applying the shuffling pattern $\pi$.  The
\Name client first divides the parameters into $w=4$ windows each
contains $k_1=3$ parameters (shown with red boxes), and permutes
parameters inside each window with the same shuffling pattern $\pi$.
Here, each row of the matrix is a superwindow, and the elements of
superwindows are shuffled with the same shuffling pattern.

%This means that in \Name, we have $k_1$ superwindows and each super window has $w=d/k_1$ elements. 
%If we choose $k_1=3$, then we have 4 windows where each row is a superwindow. 
%Each column is a window, and parameters inside each window are going to be shuffled. 


\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{Images/superwindow.pdf} 
\vspace{-0.15in}
\caption{\Name example with $k_1=3$ and $d=12$. The red boxes are
  showing the windows that the parameters inside them are going to be
  shuffled with the same shuffling pattern $\pi$.}
\label{fig:example}
\end{figure}


%\begin{equation}
%\theta=
%\begin{bmatrix}
%\Theta_A \\
%\Theta_B \\
%\Theta_C
%\end{bmatrix}
%=
%\begin{bmatrix}
%\theta_1 & \theta_4 & \theta_7 & \theta_{10}\\
%\theta_2 & \theta_5 & \theta_8 & \theta_{11} \\
%\theta_3 & \theta_6 & \theta_9 & \theta_{12} 
%\end{bmatrix}
%\end{equation}



Above example is equivalent to a scenario in FL when we have an external shuffler (doing inter-model parameter shuffling, where there are $3$ clients and each one has a local update of 4 parameters $\Theta_u$. 
In this case, client 1 update is 
$\Theta_A = [\theta_1, \theta_4, \theta_7, \theta_{10}]$, client 2 update is $\Theta_B = [\theta_2, \theta_5, \theta_8, \theta_{11}]$ and client 3 update is $\Theta_C= [\theta_3, \theta_6, \theta_9, \theta_{12}]$.
Now the inter-model shuffler permutes the updates $[\Theta_A, \Theta_B, \Theta_C]$ uniformly randomly with shuffling pattern $\pi=[3,1,2]$.
The output of the inter-model shuffler would be $\mathcal{S}_{k_1}(\theta)=[\Theta_C, \Theta_A, \Theta_B]$ where all the parameters in the first row of $\theta$ goes to the second row of shuffling output,  the second row goes to the third row, and so on.

%If we have $w=d/k_1$ windows, then each window has $k_1$ parameters. 

\end{comment}

Shuffling of superwindows, instead of individual parameters, leads to
a significant reduction in the computation (and communication)
overheads for \Name clients.  However, this comes at the cost of
smaller privacy amplification.  Corollary~\ref{thm-FedPermDP2a} shows
the privacy amplification of \Name from $\varepsilon_d$-LDP to
$(\varepsilon_{\ell}, \delta_{\ell})$-DP after superwindow shuffling
(with window size $k_1$).  After applying the randomizer $\mathcal{R}$
that is $\varepsilon_d$-LDP on the local parameters, each superwindow
is $\varepsilon_w$-LDP where $\varepsilon_w=w \cdot
\varepsilon_{wd}=\frac{d}{k_1} \cdot
\varepsilon_{wd}=\frac{\varepsilon_{d}}{k_1}$.  Since we are shuffling
the superwindows, we can derive Corollary~\ref{thm-FedPermDP2a} for
\Name by setting the shuffling pattern size to $k_1$ from
Corollary~\ref{coll-blanket-balle-generic}.  
%Furthermore, replacing
%the number of clients $n$ with the number of superwindows $k_1$ gives
%us:

%the shuffling is applied on the superwindows, From
%Corollary~\ref{coll-blanket-balle-generic}, we can show
%Corollary~\ref{thm-FedPermDP2a} where \Name with $k_1$ as window size
%is $(\varepsilon_{\ell}, \delta_{\ell})$-DP.


% then we need to make each superwindow $\varepsilon_w$-LDP using a
%randomizer $\mathcal{R}^w$.  Theorem~\ref{thm-FedPermDP2a} shows that
%\Name with $k_1$ as window size is $(\varepsilon_{\ell},
%\delta_{\ell})$-DP.


%For example, for above example, each row of matrix $\theta$ is a
%superwindow.  This means that in \Name, we have $k_1$ superwindows
%and each super window has $w=d/k_1$ elements.



\begin{corollary}
For \Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{k_1} \circ
\mathcal{R}^{w}$ with window size $k_1$, where $\mathcal{R}^w$ is
$\varepsilon_w$-LDP and $\varepsilon_{w} \leq \log{(k_1 /
  \log{(1/\delta_{\ell})})}/2$, the amplified privacy is
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w}) e^{\varepsilon_{w}}
\sqrt{\log{(1/\delta_{\ell})}/k_1}$.
\label{thm-FedPermDP2a}
\end{corollary}

%\begin{corollary} For \Name $\mathcal{F}=\mathcal{A} \circ
%\mathcal{S}_{k_1} \circ \mathcal{R}^{w}$ with window size $k_1$,
%where $\mathcal{R}^w$ is $\varepsilon_w$-LDP, $\varepsilon_{w} =
%\varepsilon_{d}/k_1$ and $\varepsilon_{d} \leq k_1 \cdot \log{(k_1 /
%\log{(1/\delta_{\ell})})}/2$, the amplified privacy is
%$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/k_1)
%e^{(\varepsilon_{d}/k_1)}
%\sqrt{\log{(1/\delta_{\ell})}/k_1}$.  \label{thm-FedPermDP2b} \end{corollary}





%This Theorem is the result of applying
%Corollary~\ref{coll-blanket-balle-generic} on the superwidnows.











%##############################k2###########################################
\subsection{\Name with Multiple Shuffling Patterns}

%In previous section, we assume that each \Name client permutes the
%parameters inside each window with the same shuffling pattern
%($\pi$).
An additional way to adjust the computation/communication vs. utility
trade off is by using multiple shuffling patterns.  Each \Name client
chooses $k_2$ shuffling patterns $\{\pi_1, \dots, \pi_{k_2}\}$
uniformly at random where each
$\pi_i=\textsc{RandomPermutations}[1,k_1] \; \text{for} \; 1 \le i \le
k_2$.  Then, each \Name client partitions the $d$ parameters into
$d/k_1$ windows, where it permutes the parameters of window $k$ ($1
\le k \le d/k_1$) with shuffling pattern $\pi_{i} \; \text{s.t.}\; i=k
\; \text{mod} \; k_2$.  In this case, each \Name client needs $k_2
\cdot k_1^2$ encryptions to generate the PIR queries.



%In this section, we are analyzing the privacy amplification of \Name
%when we have $k_2$ shuffling patterns.

%\paragraphb{Example:}
Figure~\ref{fig:example2} shows \Name for $d=12$, $k_1=3$ and $k_2=2$,
i.e., there are two shuffling patterns $\pi_1$ (shown with red box)
and $\pi_2$ (shown with blue box) and each one has 3 shuffling
indices.  In this example, the client partitions the 12 parameters
into $4$ windows that it shuffles with $\pi_1$ (1st and 3rd windows)
and $\pi_2$ (2nd and 4th windows).  This example is equivalent to an
FL scneario with \emph{two} external inter-model shufflers (with
shuffling patterns $\pi_1, \pi_2$) and three FL clients ($A,B,C$).
Each client sends $2$ ($w=d/(k_1 k_2)$) parameters to each shuffler
for shuffling with other clients.  Two different shuffling patterns
$\pi_1$ and $\pi_2$ are applied on $[\Theta_{A1}, \Theta_{B1},
  \Theta_{C1}]$ and $[\Theta_{A2}, \Theta_{B2}, \Theta_{C2}]$
respectively.



\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{Images/superwindow_k2.pdf} 
\vspace{-0.15in}
\caption{\Name example with $k_1=3$ and $k_2=2$. We have two shuffling patterns $\pi_1$ and $\pi_2$ shown with red and blue boxes.}
\label{fig:example2}
\end{figure}


%\begin{equation}
%\theta=
%\begin{bmatrix}
%\Theta_{A1} & \Theta_{A2} \\
%\Theta_{B1} & \Theta_{B2} \\
%\Theta_{C1}, & \Theta_{C2}
%\end{bmatrix}
%=
%\begin{bmatrix}
%[\theta_1, \theta_7] & [\theta_4, \theta_{10}]\\
%[\theta_2, \theta_8] & [\theta_5, \theta_{11}] \\
%[\theta_3, \theta_9] & [\theta_6, \theta_{12}] 
%\end{bmatrix}
%\end{equation}




%When we have $k_2$ patterns, it is like running \Name for $k_2$ times
%with $k_1$ users participating in FL that each one have a local
%update with $w=d/(k_1 k_2)$ parameters.
When we have $k_2$ shuffling patterns and each shuffling pattern has
$k_1$ indices, the size of each superwindow is $w=d/(k_1 k_2)$.
Therefore, each client perturbs each superwindow with a randomizer
$\mathcal{R}^w$ that satisfies $\varepsilon_{w}$-LDP where
$\varepsilon_w=w \cdot \varepsilon_{wd}=\frac{d}{k_1 k_2} \cdot
\varepsilon_{wd}=\frac{\varepsilon_{d}}{k_1 k_2}$.  Take
$\varepsilon_w$ to Corollary~\ref{coll-blanket-balle-generic} on the
superwindows to find the amplified local privacy and then using strong
composition in Lemma~\ref{lemma-PrivacyFold2} we can easily derive the
Theorem~\ref{thm-FedPermDP3aa} for \Name with
$\mathcal{S}_{k_1}^{k_2}$.
%Theorem~\ref{thm-FedPermDP3aa} shows that \Name with $k_1$ as window
%size and $k_2$ as the number of shuffling patterns is
%$(\varepsilon_{\ell}, \delta_{\ell})$-DP.  This Theorem is the result
%of first applying Corollary~\ref{coll-blanket-balle-generic} on the
%superwidnows and then applying advanced composition on $k_2$
%components.

\begin{theorem}
For \Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{k_1}^{k_2} \circ
\mathcal{R}^{w}$ with window size $k_1$, and $k_2$ shuffling patterns,
where $\mathcal{R}^w$ is $\varepsilon_w$-LDP and $\varepsilon_{w} \leq
\log{( k_1 / \log{((k_2 +1)/\delta_{\ell})})}/2$, the amplified
privacy is $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w})
e^{\varepsilon_{w}} \log{(k_2/\delta_{\ell})} \sqrt{k_2/k_1})$.
\label{thm-FedPermDP3aa}
\end{theorem}


%\begin{corollary}
%For \Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{k_1}^{k_2} \circ \mathcal{R}^{w}$ with window size $k_1$, and $k_2$ shuffling patterns, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP, $\varepsilon_{w} = \varepsilon_{d} / (k_1 k_2)$ and $\varepsilon_{d} \leq (k_1 k_2) \cdot \log{( k_1 / \log{((k_2 +1)/\delta_{\ell})})}/2$, 
%the amplified privacy is 
%$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/(k_1 k2)) e^{(\varepsilon_{d}/(k_1 k2))} \log{(k_2/\delta_{\ell})} \sqrt{k_2/k_1})$. 
%\label{coll-FedPermDP3b}
%\end{corollary}







\begin{figure}[h!]
\centering
%\begin{subfigure}{.22\textwidth}
%\centering
%\includegraphics[width=.99\linewidth]{Images/fedperm_epsc_k1_B.png} 
%\caption{Impact of $k_1$ and $\varepsilon_{wd}$.}
%\label{fig:Priv1}
%\end{subfigure}
\begin{subfigure}{.22\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/fedperm_epsc_k1k2.png} 
\caption{Impace of $k_1$ and $k_2$,}
\label{fig:Priv2}
\end{subfigure}
\begin{subfigure}{.22\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/fedperm_epsc_d.png} 
\caption{Impact of $d$ and $\varepsilon_{wd}$.}
\label{fig:Priv3}
\end{subfigure}
\vspace{-0.1in}
\caption{Privacy amplification of \Name from $\varepsilon_d$-LDP to
  ($\varepsilon_{\ell},\delta_{\ell}$)-DP.  We illustrate the overal
  amplification with Bennett inequality for the Laplace
  Mechanism. 
%\vjm{Use bigger fonts for legends and X-/Y-axis
   % captions in all figures.}
}
\label{fig:Priv-ALL}
\end{figure}

\subsection{Privacy Analysis} 
In Figure~\ref{fig:Priv-ALL}, we show the relationship of our introduced varibales $k_1$, $k_2$, $\varepsilon_d$ and $d$ on the privacy amplification in \Name. 
Figure~\ref{fig:Priv2} shows the privacy amplification effect from $\varepsilon_{d}$-LDP to ($\varepsilon_{\ell},\delta_{\ell}$)-DP for the local model updates after shuffling with $k_2$ shuffling patterns each with size of $k_1$. 
%Figure~\ref{fig:Priv2} shows the amplification of privacy when we have different $k_1$ and $k_2$s.
We can see that each client can use larger shuffling patterns (i.e. , increasing $k_1$) or more shuffling patterns (i.e., increasing $k_2$) and get larger privacy amplification.
However, this comes with a price where this imposes more computation/communication burden on the clients to create the PIR queries as they need to encrypt $k_2 \times k_1^2$ values 
and send them to the server, and it also imposes higher computation on the server as it should multiply larger matrices.
Figure~\ref{fig:Priv3} shows the amplification of privacy for fixed value of $k_1=100, k_2=10$ for various model sizes. 
From this figure we can see that if we want to provide same privacy level for larger models, we need to increase values of $k_1$ or $k_2$ (i.e. more computation/communication cost).















%We know that $\varepsilon_{w} = \varepsilon_{d}/d$ so Corollary~\ref{coll-FedPermDP5} shows the privacy amplification based on $\varepsilon_{d}$.
%
%\begin{corollary}
%If $\mathcal{R}$ is $\varepsilon_{w}$-LDP, where $\varepsilon_{w} = \varepsilon_{d}/d$ and $\varepsilon_{d} \leq d \cdot \log{(d / \log{(1/\delta_{\ell})})}/2$,
%\Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{d} \circ \mathcal{R}$ satisfies $(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/d) e^{(\varepsilon_{d}/d)} \sqrt{\log{(1/\delta_{\ell})}/d})$.
%\label{coll-FedPermDP5}
%\end{corollary}



%\begin{table}[h!] 
%\caption{Measured time for different operations in \Name for different number of parameters when $n=15$}
%\begin{center}
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%$d$ & Enc (s) & AGR (s) & Dec(s)\\
%\hline
%
%50 & 1.02 & 17.61 & 0.02 \\
%\hline
%
%100 & 3.46 & 70.71 & 0.05 \\
%
%\hline
%200 & 22.48 & 350.16 & 0.80 \\
%
%\hline
%300 & 29.33 & 639.50 & 1.41 \\
%
%\hline
%400 & 52.19 & 1152.18 & 1.41 \\
%
%\hline
%500 & 81.72 & 1793.07 & 2.46 \\
%
%
%\hline
%\end{tabular}
%\label{tab:FedpermResult1}
%\end{center}
%\end{table}





















\iffalse
%\subsection{\Name with Recursion}

\subsection{Computation and Communication Costs of \Name}

\begin{table*}[h!]
\caption{Communication and Computation Cost of \Name}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{\textit{Algorithm}} & Client: Number of Encs & Upload BW & Server: AGR & Prob Random Guess\\
\hline
FL with Homomorphic Enc& $d$ & $O(d)$ & $O(n  d)$ & - \\
\hline
\Name & $d^2$ & $O(d^2)$ & $O(n  d^3)$ & $\frac{1}{d!}$ \\

\hline
\Name with $k_1$ as window size & $k_1  d$ & $O(k_1  d)$ & $O(n  k_1  d^2)$ & $\frac{1}{k_1!}$ \\

\hline
{\vtop{\hbox{\strut \Name with $k_1$ as window size}\hbox{\strut and $k_2$ shuffling patterns}}} & $k_2  k_1^2$ & $O(k_2  k_1^2)$ & $O(n  k_2  k_1^2  d )$ & ${\left(\frac{1}{k_1!}\right)}^{k_2}$\\

\hline
\Name with recursion $(k_3)$ & $d  k_3  \sqrt[k_3]{d}$& $O(d  k_3  \sqrt[k_3]{d})$& $O(n  k_3  \sqrt[k_3]{d}  d^2)$ & $\frac{1}{d!}$\\

\hline
{\vtop{\hbox{\strut \Name with $k_1$ as window size,}\hbox{\strut and recursion $(k_3)$}}} & $k_1  k_3  \sqrt[k_3]{k_1}$& $O(k_1  k_3  \sqrt[k_3]{k_1})$& $O(n  k_3  k_1  \sqrt[k_3]{k_1}  d)$ & $\frac{1}{k_1!}$ \\

\hline
{\vtop{\hbox{\strut \Name with $k_1$ as window size,}\hbox{\strut $k_2$ shuffling patterns and recursion $(k_3)$}}} & $k_2  k_3^2  \sqrt[k_3]{k_1^2}$& $O(k_2  k_3^2  \sqrt[k_3]{k_1^2})$& $O(n  k_2  k_3^2  \sqrt[k_3]{k_1^2}  d )$&${\left(\frac{1}{k_1!}\right)}^{k_2}$ \\


\hline
\end{tabular}
\label{tab1}
\end{center}
\end{table*}
\fi


==> FedPerm/Con.tex <==
\begin{comment}
\section{Discussion and Future Work}

\paragraphb{Utilizing recursion in cPIR.}  A solution to reduce the
number encryptions and upload bandwidth at the clients would be using
recursion in our cPIR.  In this technique, the dataset is represented
by a $k_3$-dimensional hypercube, and this allows the PIR client to
prepare and send $k_3 \sqrt[k_3]{d}$ encrypted values where $k_3$
would be another hyperparameter.  For future work, we can use this
technique and reduce the number of encryptions which makes the upload
bandwidth consumption lower too.  For instance, if we have one
shuffling pattern $k_2=1$, the number of encryption decreases from
$k_1 d$ to $ k_3 \sqrt[k_3]{k_1} d$.

\paragraphb{Plugging newer PIR protocol.}  \Name utilizes cPIR for
private aggregation, and in particular we use ~\cite{chang2004single}
which is based on Paillier. However, any other cPIR protocol can be
used in \Name. For example, SealPIR~\cite{angel2018pir} can be used to
reduce the number of encryptions at the client. SealPIR is based on a
SEAL which is a lattice based fully HE. The authors show how to
compress the PIR queries and achieve size reduction of up to
$274\times$. We defer analyzing \Name with other cPIR schemes to
future work.

\paragraphb{Combination of an external client shuffler for more
  privacy amplification.}  For further privacy amplification, we can
use an external shuffler that shuffles the $n$ sampled clients'
updates similar to FLAME~\cite{liu2021flame}.  For future work, we can
use double amplification by first shuffling the parameters at the
clients (i.e. , detaching the parameter values from their position)
and then shuffle the client's updates at the external shuffler (i.e.,
detaching the updates from their client’s ID).
\end{comment}

\section{Conclusion}
%In this work, we present \Name, a novel approach to perform FL that
%concurrently achieves two goals: (i) client data privacy, and (ii)
%robustness to model poisoning attacks by adversarial clients.

We presented \Name, a new FL algorithm that combines LDP, intra-model
parameter shuffling at the federation clients, and a cPIR based
technique for parameter aggregation at the federation server to
deliver both client data privacy and robustness from model poisoning
attacks.  Our intra-model parameter shuffling significantly amplifies
the LDP guarantee for clients' training data.  The cPIR based
technique we employ allows cryptographic parameter aggregation at the
server.  At the same time, the server clips the clients' parameter
updates to ensure that model poisoning attacks by adversarial clients
are effectively thwarted.  We also presented windowing hyperparameters
in \Name that let us trade off compute resources with model utility.
Our empirical evaluation on the MNIST dataset demonstrates \Name's
privacy amplification benefits and studies the trade off between
computation and model utility.  We leave the study of extensions to
\Name\ -- (i) an additional dimension of the hyperparameters ($k_3$)
that takes the computation-utility trade offs to hypercube space (see
Appendix~\ref{sec:future-work}), (ii) plugging in other PIR protocols,
and (iii) combining an external client shuffler with \Name\ -- to
future work.



==> FedPerm/Exp.tex <==
\section{Experiments}
In this section, we investigate the utility and computation trade offs
in \Name.  We use MNIST dataset and a logistic regression model with
$d=7850$ parameters to evaluate these trade offs.




\subsection{Comparison with Baselines}
We compare our results with following baselines: \textbf{(a)}
FedAvg~\cite{mcmahan2017communication} with no privacy, \textbf{(b)}
CDP-FL~\cite{mcmahan2018learning, geyer2017differential}, \textbf{(c)}
LDP-FL~\cite{wang2019collecting, liu2020fedsel} with Gaussian
Mechanism.
%We run our experiments for 50 global rounds, and in each round we use
%$N=n=15$ clients.


\begin{figure}[h!]
\centering
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/Acc2.png} 
\caption{Final test accuracy.}
\label{fig:Acc1}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/acc3.png} 
\caption{Accuracy per FL round.}
\label{fig:Acc2}
\end{subfigure}
\vspace{-0.1in}
\caption{Test accuracy for different FL algorithms for MNIST over 15 clients.}
\label{fig:AccAll}
\end{figure}


Figure~\ref{fig:Acc1} shows the test accuracy of that model that was
trained using different FL algorithms running for $T=50$ rounds.  The
MNIST dataset is divided across $n=15$ clients with a Dirichlet
distribution.  Figure~\ref{fig:Acc2} shows the test accuracy for these
algorithms per FL round when the total privacy budget is fixed to
$\varepsilon=4.0$.  We compared two versions of \Name in these
experiments: \textbf{(a)} \Name with $k_1=400$ and $k_2=1$ which is a
``light'' version where encryption and decryption time at clients
takes around $52.2$ and $2.4$ seconds respectively.  It also imposes
$21$ minutes computation time at the server. \textbf{(b)} \Name with
$k_1=800$ and $k_2=10$ which is a ``heavy'' version where client
encryption, decryption, and server aggregation time takes around
$32.1$ minutes,  $2.4$ seconds and $16.4$ hours
respectively.

As we mentioned earlier, \Name provides a trade-off between privacy
amplification and compute resources -- larger the values of $k_1$ and
$k_2$, greater are the compute resources for training, which in turn
provides higher privacy amplification that results in better model
utility.  The heavy version of \Name needs more resources to be as
fast as the lighter version, but it can provide much more utility
(because the privacy amplification is larger so the amount of noise is
added is smaller).  For instance, after $T=50$, and total privacy
budget $(4.0, 1e^{-5})$, the heavy version provides $72.38\%$ test
accuracy while the light version provides $32.85\%$ test accuracy.
From these figures we can see if we invest enough computation
resources in \Name, we can provide higher utility compared to CDP-FL,
without trusting the \Name server.  Non-private FedAvg, CDP-FL and
LDP-FL also provides $91.02\%$, $53.50\%$, and $13.74\%$ test
accuracies for the same total $(\varepsilon, \delta)$ respectively.



\subsection{Time Analysis}
We evaluate the impacts of our hyperparameters $k_1$, $k_2$, $n$, and
$d$s on the encryption, decryption and sever aggregation time in
Figure~\ref{fig:Time-ALL}.  We use Paillier encryption system and we
use a key size of $2048$ bits in our experiments.  For measuring time,
we use 64CPUs and 64GB memory for the client and server simulations.
Note that we opt to not use GPU as model training is not a bottleneck
in our system compared to HE operations.  Also note that these figures
are data independent as we are working with encryption and decryption
and homomorphic multiplication with plaintext and homomorphic
addition.

\begin{figure}[h!]
\centering
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/time_k1_v2.png} 
\caption{Impact of $k_1$.}
\label{fig:Time1}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/time_k2_v2.png} 
\caption{Impact of $k_2$.}
\label{fig:Time2}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/time_d.png} 
\caption{Impact of $d$.}
\label{fig:Time3}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/time_n.png} 
\caption{Impact of $n$.}
\label{fig:Time4}
\end{subfigure}
\vspace{-0.1in}
\caption{Client encryption, decryption, and server aggregation time in \Name .}
\label{fig:Time-ALL}
\end{figure}


\paragraphb{Client encryption time:} In \Name, each client must do
$k_1^2 \cdot k_2$ encryptions for its query, therefore client
encryption time has a quadratic and linear relationship with window
size ($k_1$) and number of shuffling patterns ($k_2$) respectively
(Figures~\ref{fig:Time1} and~\ref{fig:Time2}). We also show in
Figure~\ref{fig:Priv-ALL} that increasing the $k_1$ has more impact
(close to quadratic impact) compared to increasing $k_2$ on the
privacy amplification. This means that if we invest more computation
resources on the clients and are able to do more encryption, we get
greater privacy amplification by parameter shuffling.  For instance,
when we increase the $k_1$ from $100$ to $200$ (while fixing $k_2=1$),
the average client encryption time increases from $3.4$ to $13.1$
seconds for $d=7850$ parameters.  And while fixing the $k_1=100$, if
we increase the number of shuffling patterns from $1$ to $10$, the
encryption time goes from $3.4$ to $32.7$ seconds.  When we fix the
value of $k_1$ and $k_2$, the number of encryption is fixed at the
clients, so the encryption time would be constant if we increase the
number of parameters ($d$) %or number of selected clients ($n$) in
each round (Figure~\ref{fig:Time3}).% and~\ref{fig:Time4}).


\paragraphb{Client decryption time:}
%As we mention in Section~\ref{sec:FedpermAdv}, based on the threat
%model, clients are fully decrypting or partially decrypting the
%parameters.
Changing $k_1$, $k_2$, and $n$ does not have any impact on decryption
time, as each client should decrypt $d$ parameters
(Figures~\ref{fig:Time1} and~\ref{fig:Time2}).  In
figure~\ref{fig:Time3}, we show the linear relationship of decryption
time and number of parameters.  For instance by increasing the number
of parameters from ${10}^5$ to ${10}^6$, the decryption time increases
from $1.01$ to $9.91$ seconds.


\paragraphb{Server aggregation time:} In \Name, the server first
multiplies the encrypted binary mask to the corresponding shuffled
model parameters for each client participating in the training round,
and then sums the encrypted unshuffled parameters to compute the
encrypted global model.  We employ joblib to parallelize matrix
multiplication over superwindows. Thus, larger the superwindows
greater is the parallelism. However, as we increase $k_1$ and/or $k_2$
the superwindow size goes down, and hence the parallelism, which leads
to increase in running time as observed in Figures~\ref{fig:Time1} and
~\ref{fig:Time2}.
\begin{comment}
\blue{We employ joblib to parallelize operations at the server.  We
  create $ d/(k_1 k_2)$ parallel matrix broadcasting of PIR queries
  ($k_2,k_1 n , k_1$) to reshaped shuffled parameters ($d/(k_1
  k_2),k_2, 1, k_1 n$) which results in encrypted global vector with
  $d=d/(k_1 k_2) \cdot k_1 \cdot k_2$ items.  This means that
  Increasing $k_1$ or $k_2$ reduces the number of parallel operations
  ($d/(k_1 k_2)$), so it results in getting less benefit from
  multiprocessing so the server time has a close to quadratic and
  linear relatioship with increasing $k_1$ and $k_2$ respectively
  (Figure~\ref{fig:Time1} and ~\ref{fig:Time2}).}
\end{comment}
Moreover, increasing $n$, $d$ has a linear relationship with server
aggregation time (Figure~\ref{fig:Time3} and~\ref{fig:Time4}).  For
instance, when we increase the $n$ from $5$ to $10$ the server
aggregation time increases from $157.47$ to $326.72$ seconds for
$d=7850$, $k_1=100$, and $k_2=1$.


%\blue{This aggregation involves of $n \cdot d/(k_1)$ matrix
%multiplications of matrices ($k_1 \times k_1$) to ($ k_1 \times 1$), and summing
%all the $n$ result vectors (each contains $d$ encrypted parameters).
%Increasing $k_1$ or $k_2$ reduces the number of parallel operations ($d/(k_1 k_2)$), so it results in  
%getting less benefit from multiprocessing so the server time has a close to quadratic and linear relatioship 
%with  increasing $k_1$ and $k_2$ respectively (Figure~\ref{fig:Time1} and ~\ref{fig:Time2}).}
%
%
%This means that increasing $k_1$ has a
%close to quadratic relationship with server aggregation time
%(Figure~\ref{fig:Time1}). 
%
%
%
%
%\blue{We employ joblib to parallel the operations at the server. 
%We create $ d/(k_1 k_2)$ parallel matrix braodcasting of PIR queries ($k_2,n\cdot k_1, k_1$) to reshaped shuffled 
%parameters ($k_2, 1, k_1 \cdot n$) which results in encrypted global vector with $d=d/(k_1 k_2) \cdot k_1 \cdot k_2$ items.
%This means that increasing $k_1$ has a
%close to quadratic relationship with server aggregation time
%(Figure~\ref{fig:Time1}). }
%\blue{This aggregation involves of $n \cdot d/(k_1 k_2) \cdot k_2$ matrix
%multiplications of matrices ($k_1 \times k_1$) to ($ k_1 \times 1$), and summing
%all the $n$ result vectors (each contains $d$ encrypted parameters).
%Increasing $k_2$ influences the number of parallel operations and when $d/(k_1 k_2)$ is smaller 
%we are getting less benefit of multiprocessing so the server time is inreasing by increasing $k_2$ (Figure~\ref{fig:Time2}).
%And increasing  $n$, $d$ has a
%linear relationship with server aggregation time
%(Figure~\ref{fig:Time3}and~\ref{fig:Time4}).  For
%instance, when we increase the $n$ from $5$ to $10$ the server
%aggregation time increases from $157.47$ to $326.72$ seconds for
%$d=7850$, $k_1=100$, and $k_2=1$.}
%\blue{This aggregation involves of $n$ matrix
%braodcasting (i.e.,  matrices ($k_2 \cdot k_1 \cdot k_1$) to ($d/(k_1 k_2) \cdot k_2 \cdot k_1 \cdot 1$)), and summing
%all the $n$ result vectors (each contains $d$ encrypted parameters).}
%\vjm{This sentence seems illegible, I don't follow
%  it. I think your are trying to say that unshuffling a superwindow
%  requires $k_2$ matrix multiplications (of $k1 \times k1$ matrices)
%  and $k_1 \cdot k_2 \cdot n$ additions are needed for the addition of
%  the $n$ clients' unshuffled parameters (for the superwindow)?
%  Please clarify/elaborate.}.  
%This means that increasing $k_1$ has a
%close to quadratic relationship with server aggregation time
%(Figure~\ref{fig:Time1}). 
%%and depends on the matrix multiplication
%%algorithm we use (naïve algorithm needs $O(n^3)$ time complexity, but
%%existing algorithms are faster).  
%And increasing $k_2$, $n$, $d$ has a
%linear relationship with server aggregation time
%(Figure~\ref{fig:Time2}, ~\ref{fig:Time3}and~\ref{fig:Time4}).  For
%instance, when we increase the $n$ from $5$ to $10$ the server
%aggregation time increases from $157.47$ to $326.72$ seconds for
%$d=7850$, $k_1=100$, and $k_2=1$.





%\subsection{Privacy Analysis}






%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/time_k1.png} 
%\caption{Client encryption, server multiplication, and decryption time for various window sizes $(k_1)$ in \Name.}
%\label{fig1}
%\end{figure}
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/time_k2.png} 
%\caption{Client encryption, server multiplication, and decryption time for various window sizes $(k_1)$ in \Name.}
%\label{fig1}
%\end{figure}

%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/acc1.png} 
%\caption{Accuracy of \Name for different privacy budgets.}
%\label{fig1}
%\end{figure}



%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/time_d.png} 
%\caption{\Name client encryption, server multiplication, and decryption time for various number of parameters ($d$) in each round.}
%\label{fig1}
%\end{figure}
%
%
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/time_n.png} 
%\caption{\Name Server processing time for different number of selected clients ($n$) in each round.}
%\label{fig1}
%\end{figure}




==> FedPerm/FedPerm.tex <==
\section{\Name: Private and Robust Federated Learning by parameter
  Permutation}

We assume a dual threat model setting where (i) the federation server
acts as an \emph{honest but curious} aggregator, and (ii) the
federation clients can maliciously attempt to poison the trained model
using manipulated local parameter updates.
%by manipulating its local parameter updates before sending them to
%the server for aggregation.

\begin{comment}
\subsection{\Name Overview} 
Figure~\ref{fig:allDP}(d) depicts the \Name framework that consists of
three components, $\mathcal{F} = \mathcal{A} \circ \mathcal{S} \circ
\mathcal{R}^{d}$.  In \Name: \textbf{(1)} There are $N$ total clients
and $n$ clients are selected randomly in each round.  Each selected
client $i$ computes its local update $x_i \in \mathbb{R}^d$ and
applies a local randomizer $\mathcal{R}^d$ on it to produce $y_i \in
\mathbb{R}^d$.  \textbf{(2)} Now each client shuffles (i.e.,
$\mathcal{S}$) the parameters inside $y_i$ to produce $y_i^{\pi_i}$
where $\pi_i$ is a random shuffling pattern that the client $i$
produces for each round.  Note that the shuffling occurs inside the
clients and there is no need for a trusted shuffler outside the client
in \Name.  The client also creates an encrypted PIR query $c_i$. Then
the client sends $(y_i^{\pi_i}, c_i)$ to the server for aggregation.
\textbf{(3)} After collecting all the shuffled local updates, with
corresponding encrypted PIR query, from $n$ clients, the server
aggregates (i.e., $\mathcal{A}$) the local updates to produce the
global update for next round.  As this global aggregated update is
encrypted, so we propose different decryption methods relevant
different thread models discussed below.
\end{comment}


\subsection{FedPerm: Design}

\Name utilizes computational Private Information Retrieval
(cPIR)~\cite{chor1997computationally,stern1998new} for secure
aggregation at the federation server.  In particular, \Name\ uses the
cPIR algorithm by Chang~\cite{chang2004single} that leverages the
algorithm by Paillier~\cite{paillier1999public}.
Algorithm~\ref{alg:algorithm1} depicts \Name.
%Note that \Name is orthogonal to the specific cPIR scheme used, and
%can work with other cPIR techniques such as
%SealPIR~\cite{angel2018pir}.
%We present \Name as $\mathcal{F} = \mathcal{A} \circ \mathcal{S}
%\circ \mathcal{R}^{d}$ with three building processes: randomizing
%$\mathcal{R}^{d}$, shuffling and encoding $\mathcal{S}$, and
%analyzing $\mathcal{A}$.  We describe each component in this section.
Figure~\ref{fig:allDP}(d) depicts the \Name framework that consists of
three components, $\mathcal{F} = \mathcal{A} \circ \mathcal{S} \circ
\mathcal{R}^{d}$, denoting the client-side parameter randomizer
($\mathcal{R}^d$), the client-side shuffler ($\mathcal{S}$), and the
server-side aggregator ($\mathcal{A}$).

\paragraphb{Key Distribution} Paillier is a partial HE (PHE) algorithm
that relies on a public key encryption scheme (details of Paillier HE
in Appendix~\ref{sec:HE}).  Since Paillier is employed to protect
client updates from a curious federation server, \Name\ requires an
independent key server that generates a pair of public and secret
homomorphic keys $(Pk, Sk)$.  This key pair is distributed to all
federation clients, and just the public key $Pk$ is sent to the
federation server (for aggregation).  The key server itself can be
implemented as an independent third party server, or a leader among
the federation clients may be chosen to play that
role~\cite{zhang2020batchcrypt}.


\begin{algorithm}[h!]
\caption{\footnotesize \Name where \serverbox{green} and \clientbox{blue} colors show execution by server and client respectively.}
\label{alg:algorithm1}
{\scriptsize
\textbf{Input}: number of FL rounds $T$, number of local epochs $E$,
number of selected users in each round $n$, learning rate $\eta$,
local privacy budget $\varepsilon_d,$ number of model parameters $d$,
parameter update clipping threshold $C$\\
\textbf{Output}: $\theta_{g}^{T}$
\begin{algorithmic}[1] %[1] enables line numbers
\STATE \serverbox{$\theta_g^{0} \gets$ Initialize weights}
\FOR{each iteration $t \in [T]$}
\STATE \serverbox{$U \gets$ set of $n$ randomly selected clients out of $N$ total clients}
\FOR{$u$ in $U$}
\STATE \clientbox{$\theta_{u}^t \gets \textsc{LocalUpdate}(\theta_g^{t}, \eta, E)$}
\STATE \clientbox{$\bar{\theta}_{u}^t \gets \textsc{Clip}(\theta_{u}^t, -C, C )$}
\STATE \clientbox{$\tilde{\theta}_{u}^t \gets (\bar{\theta}_{u}^t + C)/ (2C)$ }
\STATE \clientbox{$y_{u}^{t} \gets \textsc{Randomize}(\tilde{\theta}_{u}^t, \varepsilon_d)$}
\STATE \clientbox{$\pi_u \gets $ Shuffling pattern $\textsc{RandomPermutations} \in [1,d]$ }
\STATE \clientbox{$\tilde{y}_{u}^{t} \gets \textsc{Shuffle}(y_{u}^{t}, \pi_u)$}
\STATE \clientbox{$b_{u}^{t} \gets \textsc{BinaryMask}(\pi_u)$}
\STATE \clientbox{$c_{u}^{t} \gets \textsc{Enc}_{pk}(b_{u}^{t} )$}
\STATE \clientbox{Client $u$ sends $(\tilde{y}_{u}^{t}, c_{u}^{t})$ to the server}
\ENDFOR
%\STATE \serverbox{Server checks the norm of updates $\tilde{y}_{u\in U}^{t}$}
\STATE \serverbox{norm bounding: $\tilde{y}_{u}^{t} \gets \tilde{y}_{u}^{t}\cdot \min(1, \frac{M}{{||\tilde{y}_{u}^{t}||}_2})$ for $u \in U$}
\STATE \serverbox{$\bar{z} \gets \frac{1}{n} \sum_{u \in U} \left( c_{u}^{t} \times \tilde{y}_{u}^{t} \right) $}
%\STATE \clientbox{\%Threat Model 1: Decryption happens on Clinets}
\STATE \clientbox{$z \gets \textsc{Dec}_{sk}(\bar{z})$}
\STATE \clientbox{normalize $z \gets C \cdot \left(2z - 1\right)$}
\STATE \clientbox{update model $\theta_g^{t+1} \gets \theta_g^{t} + z$}
%\STATE \serverbox{\%Threat Model 2: Decryption happens on Server}
%\STATE \serverbox{$D \gets$ pick t clients randomly for decryption of $\bar{z}$ }
%\STATE \serverbox{${P}_{u \in D} \gets Dec_{sk_{u \in D}}(\bar{z}) $}
%\STATE \serverbox{Validate partial decryptions $({P}_{u \in D} )$}
%\STATE \serverbox{$z \gets \textsc{Combine}({P}_{u \in D} )$}
%\STATE \serverbox{normalizes $z \gets C \cdot \left(2z - 1\right)$}
%\STATE \serverbox{updates model $\theta_g^{t+1} \gets \theta_g^{t} + z$}

\ENDFOR
\STATE \textbf{return} $\theta_g^{T}$
\end{algorithmic}
}
%\vjm{Perhaps use color coding to indicate what part of the pseudo code
  %is executed by the server}
\end{algorithm}

%\subsubsection{Clients: Computing Local Updates}

\paragraphb{Client Local Training:} In the $t^{th}$ round, the server
randomly samples $n$ clients among total $N$ clients.  Each sampled
client locally retrains a copy of the global model it receives from
the server ($\theta_g^{t}$), optimizing the model using its local data
and local learning rate $\eta$ (Algorithm~\ref{alg:algorithm1}, line
5).

\paragraphb{Randomizing Update Parameters:} After computing local
updates $\theta_u^t$, client $u$ clips the update using threshold $C$
and normalizes the parameters to the range $[0,1]$
(Algorithm~\ref{alg:algorithm1}, lines 6-7).  Now the client applies
the randomizer (i.e., $\mathcal{R}^d$) on its local parameters to make
them $(\varepsilon_d)$-differentially private
(Algorithm~\ref{alg:algorithm1}, line 8).  We use the Laplacian
Mechanism as a local randomizer with privacy budget $\varepsilon_d$.
%, but any generic randomizer can be applied in this step which does not
%affect our corollaries later.

\paragraphb{Shuffling:} After clipping and perturbing the local
update, each client shuffles the parameters $y_u^t$ using the random
shuffling pattern $\pi_u$
%of model parameter indices $\in [1,d]$
(Algorithm~\ref{alg:algorithm1}, lines 9-10).  Shuffling amplifies the
privacy budget $\varepsilon_d$, which we discuss in
Section~\ref{sec:FedpermAdv}.

\paragraphb{Generating PIR queries:} Now the client encodes the
shuffle indices $\pi_u$ using a PIR protocol.
%To do so, the client retrieves each parameter out of $d$ model
%parameters privately.
This process comprises two steps: first creating a binary mask of the
shuffled index, and then encrypting it using the public key of HE that
the client received in first step (Algorithm~\ref{alg:algorithm1} line
11-12).  Generally, a PIR client needs access to the $j^{th}$ record
privately from an untrusted PIR server that holds a dataset $\theta$
with $d$ records; i.e. the PIR server cannot know that the client
requested the $j^{th}$ record.  To do so, the PIR client creates a
unit vector (binary mask) $\Vec{b}_j$ of size $d$ where all the bits
are set to zero except the $j^{th}$ position being set to one:
\begin{equation}\label{eq:vecquery}
{\footnotesize
\Vec{b}_{j}=
\begin{bmatrix}
0 & 0 & \dots & 1 & \dots & 0 & 0\\
\end{bmatrix}
}
\end{equation}
If the PIR client does not care about privacy, it would send
$\Vec{b}_j$ to the PIR server, and the server would generate the
client's response by multiplying the binary mask into the database
matrix $\theta$ ($ \theta_{j} = \Vec{b}_{j} \times \theta $).  A PIR
technique allows the client to obtain this response without revealing
$\Vec{b}_j$ to the PIR server.  For example in~\cite{chang2004single},
the PIR client uses HE to encrypt $\Vec{b}_j$ element by element
before sending it to the PIR server.  During the data recovery phase,
the client extracts its target record by decrypting the component of
$\textsc{Enc}(\Vec{b}_j) \times \theta$.  Equation~\ref{eq:PIR11}
shows retrieving the $j^{th}$ record by this PIR query.  Note that a
HE system has a property that $m_1 \times m_2 \gets \textsc{Dec}
\left( \textsc{Enc}[m_1] \times m_2 \right)$.
%\vspace{-0.1in}
\begin{equation}~\label{eq:PIR11}
{\footnotesize
\begin{aligned}
&\textsc{Dec} ( \textsc{Enc}(\Vec{b}_j) \times \theta )= \\
&\textsc{Dec} \left( \textsc{Enc}[0] \cdot \theta_1 + \dots + \textsc{Enc}[1] \cdot \theta_j + \dots + \textsc{Enc}[0] \cdot \theta_d \right) =\\
&\textsc{Dec} \left( \textsc{Enc}[\theta_j] \right) = \theta_j
\end{aligned}
}
\end{equation}
%\vspace{-0.1in}
A \Name client creates $d$ PIR queries to retrieve each parameter
privately.  (In Section~\ref{sec:FedpermAdv}, we discuss additional
parameters to reduce the number of PIR queries.)  In this case, the
shuffled parameters ($\tilde{y}_{u}^{t}$) are the dataset located at
the PIR server and each shuffled index in $\pi_u$ is the secret record
row number (i.e. $j^{th}$ in above) that the PIR client is interested
in.  Client $u$ first creates $b_u^t$ which is a collection of $d$
binary masks of shuffled indices in $\pi_u$, similar to PIR query
$\Vec{b}_j$ in Equation~\ref{eq:vecquery}.  Then the client encrypts
the binary masks and sends the shuffled parameters and the PIR query
(encrypted binary masks) to the server for aggregation.

\paragraphb{Correctness:} Note that for every client $u$ and every round
$t$, decrypting the multiplication of the encrypted binary masks to
the shuffled parameters produces the original unshuffled parameters.
It means that for $y_u^t = \textsc{Dec} \left( c_{u}^{t} \times
\tilde{y}_{u}^{t} \right)$. So for any $( \tilde{y},c, )$ we have:
\begin{equation}\label{eq:PIRcorrect1}
{\footnotesize
\begin{aligned}
&\textsc{Dec} \left( c \times \tilde{y} \right)= \\
&\textsc{Dec} \left(
\begin{bmatrix}
\textsc{Enc}(\Vec{b}_{\pi_1}) \\ \textsc{Enc}(\Vec{b}_{\pi_2}) \\ \dots \\ \textsc{Enc}(\Vec{b}_{\pi_d}) \\
\end{bmatrix} \times 
\begin{bmatrix}
\tilde{y}_1 \\ \tilde{y}_2 \\ \dots \\ \tilde{y}_d \\
\end{bmatrix} 
\right) =\\
&\textsc{Dec} \left(
\begin{bmatrix}
\textsc{Enc}[0] & \dots & \textsc{Enc}[1] & \dots & \textsc{Enc}[0] \\ 
\textsc{Enc}[0] & \dots & \textsc{Enc}[1] & \dots & \textsc{Enc}[0] \\ 
\dots & \dots & \dots & \dots & \dots\\ 
\textsc{Enc}[0] & \dots & \textsc{Enc}[1] & \dots & \textsc{Enc}[0] \\
\end{bmatrix} \times 
\begin{bmatrix}
y_1^{\pi} \\ y_2^{\pi} \\ \dots \\ y_d^{\pi} \\ 
\end{bmatrix}
\right) =\\
&\textsc{Dec} \left(\begin{bmatrix}
\textsc{Enc}[y_1] & \textsc{Enc}[y_2] & \dots & \textsc{Enc}[y_d] \\
\end{bmatrix} \right) = \\
& \begin{bmatrix}
y_1 & y_2 & \dots & y_d \\
\end{bmatrix}
\end{aligned}
}
\end{equation}

\paragraphb{Server: norm bounding}
After collecting all the local updates $(\tilde{y}_{u}^{t},
c_{u}^{t})$ for selected clients in round $t$, the \Name server first
applies $\ell_2$-norm bounding to the threshold $M$ on the shuffled
parameters $\tilde{y}_{u}^{t}$ (Algorithm~\ref{alg:algorithm1}, line
15).  Note that unlike other robust AGRs, \emph{norm bounding} is the
only robust AGR scheme that does not require the true position of the
parameters because it works by calculating the $\ell_2$ norm of the
parameter updates as a whole irrespective of their order
(i.e. $\ell_2(\tilde{y}_{u}^{t}) = \ell_2(y_{u}^{t})$).  Prior
works~\cite{nguyen2021flame,naseri2020local,sun2019can} have shown the
effectiveness of norm bounding in defense against poisoning attacks by
malicious clients.
%~\vjm{The pseudo code
%  lines 15-16 does not show the server dropping off the updates whose
%  norms are higher.  Also, I thought that the server could force the
%  norm to its threshold by clipping it.  Whatever it is we are doing,
%  we should make it explicit in the pseudo code and description.}.

\paragraphb{Server: Aggregation}
Then the server aggregates all the updates into global update
$\bar{z}$ (Algorithm~\ref{alg:algorithm1}, line 16).  This aggregation
is averaging the update parameters for $n$ collected updates by
calculating $\frac{1}{n} \sum_{u \in U} \left( c_{u}^{t} \times
\tilde{y}_{u}^{t} \right)$.  The expression $c_{u}^{t} \times
\tilde{y}_{u}^{t}$ has the effect of ``unshuffling'' client $u$'s
parameters.  At the same time, the resulting vector is encrypted, thus
kept hidden from the server.
\begin{comment}
Figure~\ref{fig:AGRE} shows the \Name
aggregation where \Name server is averaging the shuffled parameters
without knowing the true position of each parameter as their indices
are encrypted.
\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{Images/FedpermAGRprocess.pdf} 
\caption{\Name aggregation. The superscript $j$ of all the
  $\theta_i^j$s refers to the original index of the parameter; $i$ is
  the $i^{th}$ client participating in the training round.~\vjm{If we
    are in a space crunch, we can eliminate this figure; its is quite
    nice, but is not crucial to help readers understand the
    aggregation algorithm.}}
\label{fig:AGRE}
\end{figure}
\end{comment}

\paragraphb{Correctness of Aggregation:} In
Equation~\ref{eq:PIRcorrect1}, we show that $\forall t \in [T], u \in
U \;\; y_u^t = \textsc{Dec} \left( c_{u}^{t} \times \tilde{y}_{u}^{t}
\right)$.  
Based on the two main properties of a HE system 
\textbf{(a)} $m_1 \times m_2 \gets \textsc{Dec} \left( \textsc{Enc}[m_1] \times m_2 \right)$, 
\textbf{(b)} $m_1 + m_2 \gets \textsc{Dec} \left( \textsc{Enc}[m_1] + \textsc{Enc}[m_2] \right)$, and 
Equation~\ref{eq:PIRcorrect1}, we can derive the Equation~\ref{eq:PIRcorrect3}:
%

%~\vjm{This is not all that
  %obvious.  Perhaps refer to Paillier's property of additive
 % homomorphism to reach to this conclusion}:
\begin{equation}\label{eq:PIRcorrect3}
{\footnotesize
  \textsc{Dec} \left( \frac{1}{n} \sum_{u \in U} ( c_{u}^{t} \times \tilde{y}_{u}^{t}) \right)=\frac{1}{n} \sum_{u \in U} y_u^t
}
\end{equation}


\paragraphb{Updating Global Model} The server aggregates local updates
$(\tilde{y}_{u}^{t}, c_{u}^{t})$ without knowing the true position of
the parameters as they are detached from their positions.  Result of
aggregation $\frac{1}{n} \sum_{u \in U} \left( c_{u}^{t} \times
\tilde{y}_{u}^{t} \right)$ is vector of encrypted parameters, and they
need to be decrypted to be used for updating the global model
(Algorithm~\ref{alg:algorithm1} lines 17-19).  This decryption is done
at each client using Paillier's secret key.
%As we mentioned in Section~\ref{Sec:TM}, there are two decryption
%scenarios: \textbf{(1)} For honest-but-curious aggregator threat
%model, the decryption happens at the clients, and each client will
%update the global model locally \textbf{(2)} For curious and colluding
%participants threat model, the partial decryption happens at the
%selected $t$ clients and the server combines the partial decryptions
%to find unencrypted global update, and then announces it to the
%clients for next round training.









==> FedPerm/FedPermDP.tex <==





\section{Privacy Guarantees by Shuffling Parameters}

\subsection{\Name}
In \Name, each client randomizes each value in its updates with randomizer $\mathcal{R}$ and then shuffle all the $d$ values (i.e., parameters in the local update) that each value is $\varepsilon_{w}$-LDP.
From Corollary~\ref{coll-blanket-balle-generic}, we can show Corollary~\ref{coll-FedPermDP1}. 
The intuition is that we map the clients in Corollary~\ref{coll-blanket-balle-generic} to parameters in Corollary~\ref{coll-FedPermDP1}. 
This means in \Name, the number of clients participating in shuffling ($n$) will be replaced by number of parameters ($d$).


\begin{corollary}
If $\mathcal{R}$ is $\varepsilon_{w}$-LDP, where $\varepsilon_{w} \leq \log{(d / \log{(1/\delta_{\ell})})}/2$,
\Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{d} \circ \mathcal{R}$ satisfies $(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w}) e^{\varepsilon_{w}} \sqrt{\log{(1/\delta_{\ell})}/d})$.
\label{coll-FedPermDP1}
\end{corollary}

We know that $\varepsilon_{w} = \varepsilon_{d}/d$ so Corollary~\ref{coll-FedPermDP5} shows the privacy amplification based on $\varepsilon_{d}$.

\begin{corollary}
If $\mathcal{R}$ is $\varepsilon_{w}$-LDP, where $\varepsilon_{w} = \varepsilon_{d}/d$ and $\varepsilon_{d} \leq d \cdot \log{(d / \log{(1/\delta_{\ell})})}/2$,
\Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{d} \circ \mathcal{R}$ satisfies $(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/d) e^{(\varepsilon_{d}/d)} \sqrt{\log{(1/\delta_{\ell})}/d})$.
\label{coll-FedPermDP5}
\end{corollary}










%-------------------------------------------------------------Fedperm with k1--------------------------------------------

\subsection{\Name with Window Size $k_1$}


\paragraphb{Superwindow}: If we have $w=d/k_1$ windows, then each window has $k_1$ parameters. If we look at the update $\theta$ with $d$ parameters as $\mathbb{R}^{k_1 \times w}$ (a matrix with $k_1$
rows and $w$ columns), each column is a window and each row is a superwindow. For example, for above example, each row of matrix $\theta$ is a superwindow. 
This means that in \Name, we have $k_1$ superwindows and each super window has $w=d/k_1$ elements. 

Now, since the shuffling is applied on the superwindows, then we need to make each superwindow $\varepsilon_w$-LDP using a randomizer $\mathcal{R}^w$.
Theorem~\ref{thm-FedPermDP2a} shows that \Name with $k_1$ as window size is $(\varepsilon_{\ell}, \delta_{\ell})$-DP. 

\begin{theorem}
For \Name $\mathcal{F}=\mathcal{A}  \circ \mathcal{S}_{k_1} \circ \mathcal{R}^{w}$ with window size $k_1$, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP and $\varepsilon_{w} \leq \log{(k_1 / \log{(1/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w}) e^{\varepsilon_{w}} \sqrt{\log{(1/\delta_{\ell})}/k_1}$. 
\label{thm-FedPermDP2a}
\end{theorem}

\begin{corollary}
For \Name $\mathcal{F}=\mathcal{A}  \circ \mathcal{S}_{k_1} \circ \mathcal{R}^{w}$ with window size $k_1$, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP, $\varepsilon_{w} = \varepsilon_{d}/k_1$ and $\varepsilon_{d} \leq k_1 \cdot \log{(k_1 / \log{(1/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/k_1) e^{(\varepsilon_{d}/k_1)} \sqrt{\log{(1/\delta_{\ell})}/k_1}$. 
\label{thm-FedPermDP2b}
\end{corollary}





This Theorem is the result of applying Corollary~\ref{coll-blanket-balle-generic} on the superwidnows.


%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/fedperm_epsc_k1_B.png} 
%\caption{Effect of $k_1$ and $\varepsilon_{wd}$ on the central privacy budget. We illustrate the overal amplification with Bennett inequality for the Laplace Mechanism.}
%\label{fig1}
%\end{figure}







%-------------------------------------------------------------Fedperm with k1 and k2--------------------------------------------
\subsection{\Name with Window Size $k_1$ and $k_2$ Patterns}


When we have $k_2$ patterns, it is like running \Name for $k_2$ times with $k_1$ users 
participating in FL that each one have a local update with $w=d/(k_1 k_2)$ parameters.
In this case, the size of each super window is $w=d/(k_1 k_2)$.
Therefore, each client needs to apply a randomizer $\mathcal{R}^w$ with $\varepsilon_{w}$ on its superwindows.

Theorem~\ref{thm-FedPermDP3a} shows that \Name with $k_1$ as window size and $k_2$ as the number of different shuffling patterns is $(\varepsilon_{\ell}, \delta_{\ell})$-DP. 


\begin{theorem}
For \Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{k_1}^{k_2} \circ \mathcal{R}^{w}$ with window size $k_1$, and $k_2$ shuffling patterns, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP and $\varepsilon_{w} \leq \log{( k_1 / \log{((k_2 +1)/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w}) e^{\varepsilon_{w}} \log{(k_2/\delta_{\ell})} \sqrt{k_2/k_1})$. 
\label{thm-FedPermDP3a}
\end{theorem}


\begin{corollary}
For \Name $\mathcal{F}=\mathcal{A}  \circ \mathcal{S}_{k_1}^{k_2} \circ \mathcal{R}^{w}$ with window size $k_1$, and $k_2$ shuffling patterns, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP, $\varepsilon_{w} = \varepsilon_{d} / (k_1 k_2)$ and $\varepsilon_{d} \leq (k_1 k_2) \cdot \log{( k_1 / \log{((k_2 +1)/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/(k_1 k2)) e^{(\varepsilon_{d}/(k_1 k2))} \log{(k_2/\delta_{\ell})} \sqrt{k_2/k_1})$. 
\label{coll-FedPermDP3b}
\end{corollary}




This Theorem is the result of first applying Corollary~\ref{coll-blanket-balle-generic} on the superwidnows and then applying advanced composition on $k_2$ components. 


\begin{figure}[h!]
\centering
\begin{subfigure}{.22\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{Images/fedperm_epsc_k1_B.png}  
    \caption{Impact of $k_1$ and $\varepsilon_{wd}$.}
    \label{fig:Priv1}
\end{subfigure}
\begin{subfigure}{.22\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{Images/fedperm_epsc_k1k2.png}  
    \caption{Imapct of $k_1$ and $k_2$,}
    \label{fig:Priv2}
\end{subfigure}
\begin{subfigure}{.22\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{Images/fedperm_epsc_d.png}  
    \caption{Impact of $d$ and $\varepsilon_{wd}$.}
    \label{fig:Priv3}
\end{subfigure}
\caption{We illustrate the overal amplification with Bennett inequality for the Laplace Mechanism.}
\label{fig:Priv-ALL}
\end{figure}

\paragraphb{Privacy Analysis} In Figure~\ref{fig:Priv-ALL},  we show the relationship of our introduced varibales $k_1$, $k_2$, $\varepsilon_w$ and $\varepsilon_{wd}$ on the privacy amplifiction in \Name. 
Figure~\ref{fig:Priv1} shows the relationship of 
Figure~\ref{fig:Priv2}
Figure~\ref{fig:Priv3}




\subsection{Privacy Gurantee for T rounds}
We are doing Fedperm for a sequence of T adaptive $\mathcal{F}_1,\dots, \mathcal{F}_T$ where each $\mathcal{F}_t$ for $t \in [T]$ staitisifes the privacy gurantees stated in Theroemes~\ref{} dends on using pure \Name,  or $k_1$ or $k_2$.
Now we invoke the strong compositing stated in Lemma~\ref{} to obtain the pruvacy gurantee of the \Name for $T$ rounds.  We can conlude that for any $\delta'>0$,  \Name is $(\varepsilon, \delta)$-DP for 
\begin{equation}
	\varepsilon = \sqrt{2T\log{(1/\delta')}} \varepsilon_{\ell} + T \varepsilon_{\ell} (e^{\varepsilon_{\ell}}-1),  \delta=T \delta_{\ell}+ \delta'
\end{equation}



































==> FedPerm/FedPerm_TM.tex <==
\section{\Name: Private Federated Learning by parameter Permutation}

\begin{comment}
FL involves mutually untrusting clients.  Hence, a \emph{poisoning
  adversary} may own or compromise some of the FL clients, called
\emph{malicious clients}, with the goal of mounting a \emph{targeted}
or \emph{untargeted} poisoning attack.  In a targeted
attack~\cite{bhagoji2019analyzing, sun2019can}, the goal is to reduce
the utility of the model on specific test inputs, while in the
untargeted attack~\cite{baruch2019a,
  fang2020local,shejwalkar2021manipulating}, the goal is to reduce the
utility for all (or most) test inputs. It is
shown~\cite{blanchard2017machine} that even a single malicious client
can mount an effective untargeted attack on FedAvg.

Using secure aggregation makes it very easy for the poisoning
adversary to craft very large updates and destroy the global model
without being detected.  In order to make FL robust to the presence of
such malicious clients, the literature has designed various
\emph{robust aggregation rules (AGR)}~\cite{blanchard2017machine,
  mozaffari2021fsl, YinCRB18,chang2019cronus}, which aim to remove or
attenuate the updates that are more likely to be malicious according
to some criterion.  Unfortunately, these robust AGRs are not usable in
an FL with secure aggregation because the parameters are encrypted or
secrete shared.  On the other hand, it has been
shown~\cite{naseri2020local,sun2019can} that LDP-FL can defend against
targeted and untargeted attacks as the model updates are bounded.

In this work, we present \Name, a novel approach to perform FL while
concurrently achieving two goals of privacy and robustness.  \Name
provides higher utility compared to LDP-FL as each client is shuffling
the parameters, so the privacy is amplified (i.e. less noise is
required for the same level of LDP).  In this section, we describe our
algorithm overview and clarify different threat models we consider in
this paper.
\end{comment}
\vjm{Removed 3 paras from here since they seem redundant.}
We now overview \Name\ and decsribe different threat models we
consider in our work.

\subsection{\Name Overview} 
Figure~\ref{fig:allDP}(d) depicts the \Name framework that consists of
three components, $\mathcal{F} = \mathcal{A} \circ \mathcal{S} \circ
\mathcal{R}^{d}$.
In \Name:
\textbf{(1)} There are $N$ total clients and $n$ clients are selected
randomly in each round.  Each selected client $i$ computes its local
update $x_i \in \mathbb{R}^d$ and applies a local
randomizer $\mathcal{R}^d$ on it to produce $y_i \in \mathbb{R}^d$.
\textbf{(2)} Now each client shuffles (i.e., $\mathcal{S}$) the
parameters inside $y_i$ to produce $y_i^{\pi_i}$ where $\pi_i$ is a
random shuffling pattern that the client $i$ produces for each
round.  Note that the shuffling occurs inside the clients and
there is no need for a trusted shuffler outside the client in \Name.
The client also creates an encrypted PIR query $c_i$. Then
the client sends $(y_i^{\pi_i}, c_i)$ to the server for aggregation.
\textbf{(3)} After collecting all the shuffled local updates, with
corresponding encrypted PIR query, from $n$ clients, the server
aggregates (i.e., $\mathcal{A}$) the local updates to produce the
global update for next round.  As this global aggregated update is
encrypted, so we propose different decryption methods relevant
different thread models discussed below.




==> FedPerm/app.tex <==

%\section{Differential Privacy in FL Algorithms}

\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{Images/Fedperm2_TM.pdf} 
\caption{Different threat models.}
\label{fig:TM}
\end{figure}


\section{Threat Models}\label{Sec:TM}
In this section, we describe two threat models that are of interest to
our work, and illustrated in Figure~\ref{fig:TM}.

\subsection{Honest-but-Curious Aggregator}
In this threat model, we assume that the server correctly follows the
aggregation algorithm, but may try to learn clients' private
information by inspecting the model updates sent by the
participants. This is a common assumption that previous
works~\cite{zhang2020batchcrypt, xu2019hybridalpha,
  bonawitz2017practical, truex2019hybrid} also consider.  For creating
the PIR queries, we use Paillier~\cite{paillier1999public} homomorphic
encryption. We explain different homomorphic encryption systems that
we use in Appendix~\ref{sec:HE}.  Before starting \Name, we need a key
server to generate and distribute the keys for the homomorphic
encryption (HE).  A key server generates a pair of public and secret
homomorphic keys $(Pk, Sk)$, sends them to the clients, and sends only
the public key to the server.  Either a trusted external key server or
a leader client can be responsible for this role.  For the leader
client, similar to previous works~\cite{zhang2020batchcrypt}, before
the training starts, the FL server randomly selects a client as the
leader.  The leader client then generates the keys and distributes
them to the clients and the server as above.
%This key server role can be In this threat model for distributing the
%keys for the homomorphic encryption (HE), we can have one of the
%followings: \begin{itemize} \item \emph{External Key Server:} A
%trusted external key server generates a pair of public and private
%homomorphic keys $(Pk, Sk)$, sends them the clients, and sends only
%the public key to the server.  \item \emph{Leader client:} Similar to
%previous works~\cite{zhang2020batchcrypt}, before the training
%starts, the FL server randomly selects a client as the leader who
%generates the keys and distribute them among the clients and the
%server.  \end{itemize}

The steps of \Name for this threat model (Figure~\ref{fig:TM}(a)) are
as follows:
\textbf{(1)} The pair of keys are distributed by the key server to all
the clients.
\textbf{(2)} In each round of training, the clients learn their local
updates, generate encrypted PIR query and shuffled parameters, and
send them to the server.  Next, the server aggregates the updates, and
sends the aggregated update to the clients.
\textbf{(3)} Each client can decrypt the encrypted global parameters
received from the server using the private key and updates its model.


\subsection{Curious and Colluding Clients}
In this threat model, we assume that some clients may collude with the
FL server to get private information about a victim client by
inspecting its model update.  For this threat model, we use
thresholded Paillier~\cite{damgaard2001generalisation}.  In the
thresholded Paillier scheme, the secret key is divided to multiple
shares, and each share is given to a different client.  For this
threat model, we need an external key server that generates the keys
and sends $(Pk, Sk_i)$ to each client, and sends the public key to the
server.  Now each client can partially decrypt an encrypted
message, but if less than a threshold, say $t$, combine their partial
decrypted values, they cannot get any information about the real
message.  On the other hand, if we combine $\geq t$ partial decrypted
values, we can recover the secret.  We explain how thresholeded
Paillier scheme works in Appendix~\ref{sec:HE}.

The steps of \Name for this threat model (Figure~\ref{fig:TM}(b)) are
as follows:
\textbf{(1)} The pairs of keys are distributed to the clients by the
key server.
\textbf{(2)} In each round of training, the clients learn their local
updates,generate encrypted PIR query and shuffled parameters, and send
them to the server.  Next, the server aggregates the local updates to
produce global model update (which is encrypted).
\textbf{(3)} The server randomly chooses $t$ clients to partially
decrypt the global model update. The \Name server sends the encrypted
global update to these clients.
\textbf{(4)} Each client decrypts the global model with its specific
partial secret key $Sk_i$, and sends the result back to the server.
\textbf{(5)} The server first authenticates each partial decryption
that is done by the true $Sk_i$ (by a zero-knowledge proof provided by
thresholded Paillier~\cite{damgaard2001generalisation}).  Then the
\Name server combines the partial decrypted updates and broadcasts
plain unshuffled model updates to all the clients for the next round
of \Name.

At present our implementation of \Name does not support this threat
model, and we leave it for future work.

\section{Central Differential Privacy in FL (CDP-FL)}
Algorithm~\ref{alg:CDP-FL} shows how CDP-FL works which is also
discussed in ~\cite{mcmahan2018learning, geyer2017differential,
  naseri2020local}.  In CDP-FL, the server receives model updates
capped by norm $C$, and after averaging them, it adds i.i.d sampled
noise to the parameters $\theta_g^{t+1} \gets \theta_g^{t} +
\frac{1}{n} \sum_{u \in U} \theta_u^{t} + \mathcal{N} (0, \sigma^2
\mathbb{I})$ where $\sigma \gets \frac{\Delta_2}{\varepsilon} \sqrt{2
  ln(1.25) / \delta }$ and the $\ell_2$ sensitivity is $\Delta_2=C$.

\begin{algorithm}[h!]
\caption{Central Differential Privacy in FL (CDP-FL)}
\label{alg:CDP-FL}
\textbf{Input}: number of FL rounds $T$, number of local epochs $E$,
number of all the clients $N$, number of selected users in each round
$n$, total privacy budget $TP$, probability of subsampling clients
$q$, learning rate $\eta$, noise scale $z$, bound $C$
\\ \textbf{Output}: global model $\theta_{g}^{T}$
\begin{algorithmic}[1] %[1] enables line numbers
\STATE  $\theta_g^{0}  \gets$ Initialize weights
\STATE Initialize MomentAccountant$(\varepsilon,  \delta,  N)$

\FOR{each iteration $t \in [T]$}
	\STATE $U \gets$ set of $n$ randomly selected clients out of $N$ total clients with probability of $q$
	\STATE $p_t \gets $ MomentAccountant.getPrivacySpent()  \COMMENT{\% privacy budget spent till this round}
	\IF{$p_t > TP$} 
		\STATE \textbf{return} $\theta_g^{T}$ \COMMENT{\% if spent privacy budget is passed over the threshold finish FL training}
	\ENDIF
    	\FOR{$u$ in $U$}
		\STATE $\theta \gets \theta_g^{t}$
		\FOR{local eopoch $e \in [E]$}
			\FOR{batch $b \in [B]$}
				\STATE $\theta \gets \theta - \eta \triangledown L(\theta,  b)$ 
				\STATE $\triangle \gets \theta - \theta_g^{t}$
				\STATE $\theta \gets \theta_{g}^{t} + \triangle \min{(1,  \frac{C}{{||\triangle||}_2})}$
			\ENDFOR
		\ENDFOR
		\STATE Client $u$ sends $\theta_{u}^{t}=\theta-\theta_{g}^{t}$ to the server
	\ENDFOR
	\STATE $\sigma \gets z C/q$
	\STATE  $\theta_g^{t+1} \gets \theta_g^{t} +  \frac{1}{n} \sum_{u \in U} \theta_u^{t} + \mathcal{N} (0,  \sigma^2 \mathbb{I}) $
	\STATE MomentAccountant.accumulateSpentBudget$(z)$
\ENDFOR
\STATE \textbf{return} $\theta_g^{T}$
\end{algorithmic}
\end{algorithm}






%\subsection{Local Differential Privacy in FL}
%In this setting,  each client utilizes differentialy private stochastic gradient descent (DP-SGD)~\cite{abadi2016deep} to train a private model on top of its data.  
%Algorithm~\ref{alg:LDP-FL} shows how DP-SGD in local differentaially private FL works.
%
%Please note that in a mini-batch,  the gradient for each data item is computed and clipped speprtedly to limit the sensitivity of each data item on the output of loss function's gradient.


%\begin{algorithm}[h!]
%\caption{Local Differential Privacy in FL (LDP-FL)}
%\label{alg:LDP-FL}
%\textbf{Input}:  number of FL rounds $T$, number of local epochs $E$,  number of all the clients $N$,  number of selected users in each round $n$,  sampling probability $p$,  
%learning rate $\eta$,  noise scale $z$,  bound $C$ \\
%\textbf{Output}: global model $\theta_{g}^{T}$
%\begin{algorithmic}[1] %[1] enables line numbers
%\STATE  $\theta_g^{0}  \gets$ Initialize weights
%
%\FOR{each iteration $t \in [T]$}
%	\STATE $U \gets$ set of $n$ randomly selected clients out of $N$ total clients
%    	\FOR{$u$ in $U$}
%		\STATE $\theta_0 \gets \theta_g^{t}$
%		\FOR{local eopoch $e \in [E]$}
%			\FOR{$(x,y) \in $ random batch from training dataset wtih probability $p$}
%				\STATE $g_e (x_i) \gets  \triangledown_{\theta_e} L(\theta_e, (x_i,y_i))$ 
%			\ENDFOR
%			\STATE $\bar{g}_e (x_i) \gets g_e (x_i) \min{(1,  \frac{C}{{||g_e (x_i)||}_2})}$
%			\STATE ${\tilde{g}}_e \gets \frac{1}{pD} \left( \sum_{i \in batch} \bar{g}_e (x_i) +  \mathcal{N} (0,  C^2 \sigma^2 \mathbb{I}) \right)$ 
%			\STATE $\theta_{e+1} \gets \theta_e - \eta {\tilde{g}}_e$
%	\ENDFOR
%	\STATE Client $u$ sends $\theta_{u}^{t}=\theta_{E}$ to the server
%	\ENDFOR
%	\STATE updates model $\theta_g^{t+1} \gets \frac{1}{n} \sum_{u \in U} \theta_{u}^{t}$
%	\ENDFOR
%\STATE \textbf{return} $\theta_g^{T}$
%\end{algorithmic}
%\end{algorithm}





%\subsection{Client Shuffling Differential Privacy in FL}









%/section{Privacy Backgrounds}

\section{Laplace Mechanism}~\label{sec:Laplace}
The most common mechanism for achieving pure $\varepsilon_{\ell}$-DP
is Laplace mechanism~\cite{}, where

\begin{definition}
Let $f: \mathcal{X}^n \rightarrow \mathbb{R}^{k}$.  The
$\ell_1$-sensitivity of $f$ is:
\begin{equation}
\Delta_1^{(f)} = \max_{X, X'} {|| f(X) - f(X')||}_1
\end{equation}
where $X, X' \in \mathcal{X}^n$ are neighbering datasets differing
from each other by a single data record.
\end{definition}

Sensitivity gives an upper bound on how much the output of the
randomizer can change by switching over to a neighboring dataset as
the input.

\begin{definition}
Let $f: \mathcal{X}^n \rightarrow \mathbb{R}^{k}$. The Laplace
mechanism is defined as:
\begin{equation}
\mathcal{R} (X) = f(X) + [Y_1,  \dots, Y_k]
\end{equation}
Where the $Y_i$s are drawn i.i.d from
Laplace$(\Delta^{(f)}/\varepsilon)$ random variable.  This
distribution has density of
$p(x)=\frac{1}{2b}\exp{\left(-\frac{|x|}{b} \right)}$ where $b$ is the
scale and equal to $\Delta^{(f)}/\varepsilon$.
\end{definition}

In \Name, each client $i$ applies the Laplace mechanism as a
randomizer $\mathcal{R}$ on its local model update $(x_i)$.  Each
model update contains $d$ parameters in range of $[0,1]$, so the
sensitivity of the entire input vector is $d$.  It means that applying
$\varepsilon_d$-DP on the vector $x_i$ is equal to applying
$\varepsilon_{wd}=\varepsilon_{d}/d$ on each parameter independently.
Therefore, applying $\varepsilon_d$-DP randomizer $\mathcal{R}$ on the
vector $x_i$ means adding noise from Laplace distribution with scale
$b=\frac{1}{\varepsilon_{wd}}=\frac{1}{\frac{\varepsilon_d}{d}}=\frac{d}{\varepsilon_d}$.

%The major strength of the Gaussan mechanims is that it draw noise from normal distribution with L2 sensitivity and in which L2 sensitivity is much lower than L1 sensitivity, the Gaussian mechanism allows adding much less noise.

\iffalse
\section{\Name Privacy Gurantee for T rounds}
We are doing \Name for a sequence of $T$ rounds $\mathcal{F}_1,\dots,
\mathcal{F}_T$ where each $\mathcal{F}_t$ for $t \in [T]$ satisfies
the privacy gurantees stated above for different settings of \Name.
Now we invoke the strong composition theorem stated in
Lemma~\ref{lemma-PrivacyFold2} to obtain the privacy gurantee of the
\Name for $T$ rounds.  We can conclude that for any $\delta'>0$, \Name
is $(\varepsilon, \delta)$-DP for
\begin{equation}
	\varepsilon = \sqrt{2T\log{(1/\delta')}} \varepsilon_{\ell} + T \varepsilon_{\ell} (e^{\varepsilon_{\ell}}-1),  \delta=T \delta_{\ell}+ \delta'
\end{equation}
\fi


\section{Background}
\subsection{Robustness to poisoning attacks} 
Most of the distributed learning algorithms, including FedAvg~\cite{mcmahan2017communication}, 
operate on mutually untrusted clients and server. This makes distributed learning susceptible to the threat of poisoning~\cite{kairouz2019advances, shejwalkar2021back}. 
A \emph{poisoning adversary} can either own or control a few of FL clients, called \emph{malicious clients}, and instruct them to share malicious updates with the central server in order to reduce the performance of the global model. There are two approaches to poisoning FL: \emph{untargeted}~\cite{baruch2019a, fang2020local,shejwalkar2021manipulating} attacks aim to reduce the utility of global model on arbitrary test inputs; and \emph{backdoor}~\cite{bagdasaryan2020backdoor,wang2020attack, xie2019dba} attacks aim to reduce the utility on test inputs that contain a specific signal called the trigger.

In order to make FL robust to  the presence of such malicious clients, the literature has designed various \emph{robust aggregation rules (AGR)}~\cite{blanchard2017machine, DBLP:conf/icml/MhamdiGR18, YinCRB18,mozaffari2021fsl}, which aim to remove or attenuate the updates that are more likely to be malicious according to some criterion. For instance, Multi-krum~\cite{blanchard2017machine} repeatedly removes updates that are far from the geometric median of all the updates, and Trimmed-mean~\cite{YinCRB18} removes the largest and smallest values of each update dimension and calculates the mean of the remaining values.
It is not possible to use these AGRs in secure aggregation as the parameters are encrypted.

\subsection{Private Information Retrieval (PIR)}
Private information retrieval (PIR) is a technique to provide query
privacy to users when fetching sensitive records from untrusted
database servers.  That is, PIR enables users to query and retrieve
specific records from untrusted database server(s) in a way that the
servers cannot identify the records retrieved.  There are two major
types of PIR protocols. The first type is \emph{computational PIR}
(CPIR)~\cite{chang2004single} in which the security of the protocol
relies on the computational difficulty of solving a mathematical
problem in polynomial time by the servers, e.g., factorization of
large numbers. Most of the CPIR protocols are designed to be run by a
single database server, and therefore to minimize privacy leakage they
perform their heavy computations on the whole database (even if a
single entry has been queried). Most of these protocols use
homomorphic encryption (Section~\ref{sec:HE}) to make their queries
private.  The second major class of PIR is \emph{information-theoretic
  PIR} (ITPIR)~\cite{mozaffari2020heterogeneous}.  ITPIR protocols
provide information-theoretic security, however, existing designs need
to be run on more than one database servers, and they need to assume
that the servers do not collude.  Our work uses computational PIR
(cPIR) protocols to make the shuffling private.

\subsection{Homomorphic Encryption (HE)}\label{sec:HE}
Homomorphic encryption (HE) allows application of certain arithmetic
operations (e.g., addition or multiplication) on the ciphertexts
without decrypting them.  Many recent works~\cite{chang2004single}
advocate using partial HE, that only supports addition, to make the FL
aggregation secure.  In this section we describe two important HE
systems that we use in our paper.

\paragraphb{Paillier}
%Existing works~\cite{} use Paillier~\cite{paillier1999public} to
%provide secure aggregation in FL.
An additively homomorphic encryption system provides following
property:

\begin{equation}
  Enc(m_1) \circ Enc(m_2) = Enc(m_1 + m_2)
\end{equation}
where $\circ$ is a defined function on top of the ciphertexts. 

In these works, the clients encrypt their updates, send them to the
server, then the server can calculate their sum (using the $\circ$
operation) and sends back the encrypted results to the clients.  Now,
the clients can decrypt the global model locally and update their
models.  Using HE in these scenario does not produce any accuracy loss
because no noise will be added to the model parameters during the
encryption and decryption process.
%The process is as follows:
%\begin{itemize}
%	\item \emph{Key generation:} 
%	\item \emph{Encryption:} 
%	\item \emph{Decryption:} 
%\end{itemize}


\paragraphb{Thresholded Paillier}
In~\cite{damgaard2001generalisation}, the authors extend the Paillier
system and proposed a thresholded version.  In the thresholded
Paillier scheme, the secret key is divided to multiple shares, and
each share is given to a different participant.  Now each participant
can partially decrypt an encrypted message, but if less than a
threshold, say $t$, combine their partial decrypted values, they
cannot get any information about the real message.  On the other hand,
if we combine $\geq t$ partial decrypted values, we can recover the
secret.  In this system, the computations are in group
$\mathbb{Z}_{n^2}$ where $n$ is an RSA modulus.  The process is as
follows:

\begin{itemize}
\item \emph{Key generation:} First find two primes $p$ and $q$
  that statisfies $p=2p'+1$ and $q=2q'+1$ where $p',q'$ are
  also prime.  Now set the $n=pq$ and $m=p'q'$.  Pick $d$ such
  that $d=0\; \text{mod} \; m$ and $d=1 \; \text{mod} \;
  n^2$. Now the key server creates a polynomial
  $f(x)=\sum_{i=0}^{k-1} a_i x^i \; \text{mod} \; n^2m$ where
  $a_i$ are chosen randomly from $\mathbb{Z}^{*}_{n^2m}$ and
  the secret is hidden at $a_0=d$.  Now each secret key share
  is calculated as $s_i=f(i)$ for $\ell$ shareholders and the
  public key is $n$. For verification of correctness of
  decryption another public value $v$ is also generated where
  the verification key for each shareholder is $v_i=v^{\Delta
    s_i} \; \text{mod} \; n^2$ and $\Delta=\ell$.
\item \emph{Encryption:} For message $M$, a random number $r$
  is chosen from $\mathbb{Z}^{*}_{n^2}$ and the output
  ciphertext is $c=g^{M} \cdot r^{n^2} \; \text{mod} \; n^2$.
\item \emph{Share decryption:} The $i^{th}$ shareholder
  computes $c_i = c^{2 \Delta s_i}$ for ciphertext $c$. And
  for zero-knowlege proof, it provides $\log_{c^4}
  {(c_i^2)}=\log_{v} {(v_i)}$ which provides gurantee that the
  shareholder really uses its secret share for decryption
  $s_i$.
\item \emph{Share combining:} After collecting $k$ partial
  decryption, the server can combine them into the original
  plain-text message $M$ by $c'=\Pi_{i\in [k]}
  c_i^{2\lambda_{0,i}^S} \; \text{mod} \; n^2$ where
  $\lambda_{0,i}^S=\Delta \Pi_{i' \in [k] , i'\ne i}
  \frac{-i}{i-i'}$.  And use it to generate the $M$.
\end{itemize}


\section{Discussion and Future Work}
\label{sec:future-work}
\paragraphb{Utilizing recursion in cPIR.}  A solution to reduce the
number encryptions and upload bandwidth at the clients would be using
recursion in our cPIR.  In this technique, the dataset is represented
by a $k_3$-dimensional hypercube, and this allows the PIR client to
prepare and send $k_3 \sqrt[k_3]{d}$ encrypted values where $k_3$
would be another hyperparameter.  For future work, we can use this
technique and reduce the number of encryptions which makes the upload
bandwidth consumption lower too.  For instance, if we have one
shuffling pattern $k_2=1$, the number of encryption decreases from
$k_1 d$ to $ k_3 \sqrt[k_3]{k_1} d$.

\paragraphb{Plugging newer PIR protocol.}  \Name utilizes cPIR for
private aggregation, and in particular we use ~\cite{chang2004single}
which is based on Paillier. However, any other cPIR protocol can be
used in \Name. For example, SealPIR~\cite{angel2018pir} can be used to
reduce the number of encryptions at the client. SealPIR is based on a
SEAL which is a lattice based fully HE. The authors show how to
compress the PIR queries and achieve size reduction of up to
$274\times$. We defer analyzing \Name with other cPIR schemes to
future work.

\paragraphb{Combination of an external client shuffler for more
  privacy amplification.}  For further privacy amplification, we can
use an external shuffler that shuffles the $n$ sampled clients'
updates similar to FLAME~\cite{liu2021flame}.  For future work, we can
use double amplification by first shuffling the parameters at the
clients (i.e. , detaching the parameter values from their position)
and then shuffle the client's updates at the external shuffler (i.e.,
detaching the updates from their client’s ID).




%\section{Reproducibility Checklist}
%
%
%
%This paper:
%\begin{itemize}
%\item Includes a conceptual outline and/or pseudocode description of AI methods introduced: \textbf{yes}
%\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results: \textbf{yes}
%\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper: \textbf{yes}
%\item Does this paper make theoretical contributions? \textbf{yes} \\
%If yes, please complete the list below.
%\item All assumptions and restrictions are stated clearly and formally.  \textbf{yes}
%\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
%\item Proofs of all novel claims are included. (yes/partial/no)
%\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
%\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
%\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
%\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
%\item Does this paper rely on one or more datasets? (yes/no)
%\item If yes, please complete the list below.
%\item A motivation is given for why the experiments are conducted on the selected datasets. (yes/partial/no/NA)
%\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)
%\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
%\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)
%\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)
%\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)
%\end{itemize}




\iffalse

\section{Private Information Retrieval (PIR)}
PIR algorithms have been suggested to be used in various application scenarios involving  untrusted database servers~\cite{olumofin2010privacy,mittal2011pir,gupta2016scalable,pir-ecommerce,hafiz2017querying,cappos2013avoiding,borisov2015dp5,piotrowska2017annotify,li2017rpir}, from retrieving Tor relay information~\cite{mittal2011pir} to privacy-preserving querying of location services~\cite{ghinita2008private} to registering Internet domains~\cite{olumofin2010privacy}. 



 Private information retrieval (PIR) is a technique to provide query privacy to users when fetching sensitive records from untrusted databases. 
There are two major types of PIR protocols. The first type is \emph{computational PIR} (CPIR)~\cite{chor1997computationally, kushilevitz1997replication, aguilar2007lattice, aguilar2016xpir, brakerski2014efficient, cachin1999computationally, dong2014fast, kiayias2015optimal, lipmaa2017simpler, stern1998new, angel2018pir} in which the security of the protocol relies on the computational difficulty of  solving a mathematical problem in polynomial time by the servers, e.g., factorization of large numbers. Most of the CPIR protocols are designed to be run by a single database server, and therefore to  minimize privacy leakage they  perform their heavy computations on the whole database (even if a single entry has been queried). Consequently, existing CPIR protocols suffer from very high computation overheads. 
 The second major class of PIR is \emph{information-theoretic PIR} (ITPIR)~\cite{demmler2014raid,henry2013one, beimel2002robust, chor1995private, gertner1998random, goldberg2007improving, beimel2002breaking, devet2012optimally}. ITPIR protocols provide information-theoretic security, however,  existing designs need to be run on more than one database servers, and they need to assume that the servers do not collude. Existing ITPIR protocols impose lower computation overheads compared to CPIR algorithms, but at the price of requiring the non-collusion assumption for the servers. Therefore, (multi-server) ITPIR protocols are best fit to scenarios involving multiple (potentially competing) data owners who collaborate to run a service privately, therefore colluding is not in their best interest, e.g., \cite{li2017rpir, mittal2011pir, borisov2015dp5}. Our work focuses on this class of  PIR, i.e., multi-server PIR protocols. 


\paragraphb{Computational PIR (CPIR) protocols}
Most of CPIR protocols use a single server which is computationally bounded for retrieving data. It means the security of these protocols is based on a very difficult mathematical problem, and if the adversary finds a solution for the problem, or if she has enough time and computation resources, some data will be leaked. 

\paragraphb{Stern et al.\ CPIR} Stern et al.~\cite{stern1998new} propose a CPIR protocol that its algorithm is based on additively homomorphic cryptosystem which has these functions: (i) $Gen$: function of generating public and private keys $pk, sk$ and system parameters , (ii) $Enc$: Encryption function with public key ,and (iii) $Dec$: Decryption function. 

The important point in this scheme is that the cryptosystem is non-deterministic i.e. the $Enc$ is a randomize function that encrypts the same input to different output each time. $Dec$ function will cancel the effect of the random variable that was used in $Enc$ function. The most famous non-deterministic cryptosystem that is used for CPIR is Paillier~\cite{paillier1999public}. 

XPIR~\cite{aguilar2016xpir} proposes a new CPIR based on this protocol by looking at each record of the database as a polynomial (the elements of the databases are encoded as coefficients of the polynomial). However, the bandwidth consumption is not very good, so SealPIR~\cite{angel2018pir} introduce a way to compress the queries in this system.

\paragraphb{Kushilevitz and Ostrovsky CPIR} \label{app:kush}
One of the merits of CPIR is that the client can run the protocol recursively to reduce the bandwidth consumption. This idea was used by Kushilevitz and Ostrovsky~\cite{kushilevitz1997replication} in their scheme for improving the communication cost. First, they split the database into several virtual blocks, and each one of these blocks contains some of the real blocks, then the client sends her query for a specific virtual block, then server will calculate the result of that query on the database and will look at the result as a new database, the next query will be applied to this temporary database, and this process continues until one vector of size $s$ will be sent to the client, and client can recover her requested index out of this result.





\section{Poisoning Attacks and Byzanthine-Robust Aggregation Rules in FL}
FL involves mutually untrusting  clients. 
Hence, a \emph{poisoning adversary} may own or compromise some of the FL clients, called \emph{malicious clients}, with the goal of mounting a \emph{targeted} or \emph{untargeted} poisoning attack. In a targeted attack~\cite{bhagoji2019analyzing, sun2019can}, the goal is to reduce the utility of the model on specific test inputs, while in the untargeted attack~\cite{baruch2019a, fang2020local,shejwalkar2021manipulating}, the goal is to reduce the utility for all (or most)  test inputs. It is shown~\cite{blanchard2017machine} that even a single malicious client can mount an effective untargeted attack on FedAvg. 

In order to make FL robust to  the presence of such malicious clients, the literature has designed various \emph{robust aggregation rules (AGR)}~\cite{blanchard2017machine, DBLP:conf/icml/MhamdiGR18, YinCRB18,chang2019cronus}, which aim to remove or attenuate the updates that are more likely to be malicious according to some criterion. For instance, Multi-krum~\cite{blanchard2017machine} repeatedly removes updates that are far from the geometric median of all the updates, and Trimmed-mean~\cite{YinCRB18} removes the largest and smallest values of each update dimension and calculates the mean of the remaining values.
% 
% In order to make FL robust to  the presence of such malicious clients, the literature has proposed multiple aggregation rules (AGRs)~\citep{blanchard2017machine,mhamdi2018the,xie2018generalized,diakonikolas2019sever} with theoretical robustness guarantees. 
Unfortunately, these robust AGRs are not very effective in  non-convex FL settings and multiple works have demonstrated strong targeted~\cite{wang2020attack,bhagoji2019analyzing} and untargeted attacks~\cite{shejwalkar2021manipulating,fang2020local} on them.

\fi



==> FedPerm/bg.tex <==
\section{Preliminaries}

%To provide privacy guarantees in FL, different \emph{differentially
%  private federated learning} algorithms has been introduced.
%  Differential Privacy provides statistical guarantees for the
%  leaking information that an adversary can infer by inspecting the
%  output of a randomized mechanism.  In this section, we first
%  describe different FL algorithms (illustrated in
%  Figure~\ref{fig:allDP}), and then introduce properties we use
%  throughout the paper.  Table~\ref{table:notation} shows the
%  notations we use in this paper.

%We now present existing FL algorithms (see Figure~\ref{fig:allDP}),
%and their properties that are relevant to \Name{}'s design.
%Table~\ref{table:notation} shows the notations we use in this paper.

%\subsection{Notations}



\begin{comment}
\begin{table}
\centering
\small
{\footnotesize
\caption{List of notations}
\label{table:notation}
\begin{tabular}{ |c|c| }
\hline
$\mathcal{A}$ & Analyzer (e.g. FL server)\\
\hline
$\mathcal{R}$ & Randomizer function \\
\hline
$\mathcal{S}$ & Shuffler \\
\hline
$N$ & Total number of clients participating in FL \\
\hline
$n$ & Number of selected clients in each round of FL \\
\hline
$d$ & Number of parameters in Model \\
\hline 
$x_i$ & Local update for $i^{th}$ client $\in \mathbb{R}^d$\\
\hline
$k_1$ & Window size \\
\hline 
$k_2$ & Number of shuffling Patterns\\
\hline
 $\mathcal{S}_{k_1}^{k_2}$ & {\vtop{\hbox{\strut Shuffling function with $k_2$ shuffling patterns}\hbox{\strut each pattern consits of $k_1$ indices}}} \\
\hline
%$\mathcal{S}_{k_1}^{k_2}$ & Shuffling function with $k_2$ shuffling patterns each consits of $k_1$ indices. \\
%\hline
$\pi$ & Shuffling pattern\\
\hline
$\varepsilon_{\ell}$ & Local differential privacy budget after amplification\\
\hline
$\varepsilon_{d}$ & Local differential privacy budget before amplification\\
\hline
%$E$ & Number of local epochs\\
%\hline
%$T$ & Number of global rounds\\
%\hline
%$\eta$ & Local learning rate\\
%\hline
\end{tabular}
}
\end{table}
\end{comment}






%/subsection{Secure Aggregation in FL} Secure
%aggregation~\cite{bonawitz2017practical} is proposed to limit the
%server inferences from the local updates, i.e., the server is only
%learning the aggregated updates and not learning anything from the
%clients' updates.





%\section{Federated Learning with Differential Privacy} We first
%illustrate how existing differential private federated learning work
%in Figure~\ref{fig:allDP}, and then introduce properties that will be
%used throughout the paper.  To provide privacy guarantees in FL,
%different \emph{differentially private federated learning} algorithms
%has been introduced.  Differential Privacy provides statistical
%guarantees for the leaking information that an adversary can infer by
%inspecting the output of a randomized mechanism.
%############Existing DP-FL works########### The existing works are
%categorized in three groups: \textbf{(1)} \emph{Centralized
%differentially private FL (CDP-FL)}~\cite{mcmahan2018learning,
%geyer2017differential} in which the clients send their raw model
%updates to a trusted server, and the server aggregates them into a
%global model and randomizes the global model.  \textbf{(2)}
%\emph{Locally differentially private FL
%(LDP-FL)}~\cite{wang2019collecting, liu2020fedsel} in which each
%client randomizes its local update before sending then to an
%untrusted server.  The CDP-FL provides better utility with cost of
%trusting the server, but the LDP-FL preserves strong local privacy
%with cost of low utility.  \textbf{(3)} \emph{Differentially private
%FL by shuffling updates
%(DP-FL-S)}~\cite{girgis2021shuffled,liu2021flame} in which.


\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{Images/Fedperm1.pdf} 
\vspace{-0.1in}
\caption{Different models of differential privacy in Federated
  Learning. Red dots are showing the trust boundaries.}
\label{fig:allDP}
\end{figure}


%\subsection{Non-Private Federated Learning (FL)}
In FL~\cite{mcmahan2017communication, kairouz2019advances,
  konevcny2016federated}, $N$ clients collaborate to train a global
model without directly sharing their data.  In round $t$, the
federation server samples $n$ out of $N$ total clients and sends them
the most recent global model $\theta^t$. Each client re-trains
$\theta^t$ on its private data
%starting from the $\theta^t$
using stochastic gradient descent (SGD), and sends back the model
parameter updates ($x_i$ for $i^{th}$ client) to the server. The
server then aggregates (e.g., averages) the collected parameter
updates
%($x_i$ for $i \in [n]$)
and updates the global model for the next round ($\theta^t \gets
\theta^{t-1} + \frac{1}{n} \sum_{i=1}^n x_i$).
%  FL can be either cross-device or
%cross-silo~\cite{kairouz2019advances}. In cross-device FL, N is large
%(from few thousands to billions) and only a small fraction of clients
%is chosen in each FL training round, i.e., $n \ll N$. By contrast, in
%cross-silo FL, N is moderate (up to 100) and all clients are chosen
%in each round, i.e., $n = N$.  In this work, we evaluate the
%performance of \Name and other FL baselines for both cross-device and
%cross-silo FL under realistic production FL settings.


\subsection{Central Differential Privacy in FL (CDP-FL)}
In CDP-FL~\cite{mcmahan2018learning, geyer2017differential},
illustrated in Figure~\ref{fig:allDP}(a) , a \emph{trusted} server
first collects all the clients' raw model updates ($x_i \in
\mathbb{R}^d$), aggregates them into the global model, and then
perturbs the model with carefully calibrated noise to enforce
differential privacy (DP) guarantees.  The server provides
participant-level DP by the perturbation.  Formally, consider
\emph{adjacent} datasets ($X, X' \in \mathbb{R}^{n\times d}$) that
differ from each other by the data of one federation client.  Then:

%The privacy goal of CDP-FL is providing indistinguishability for any
%outputs for all the neighboring datasets ($X, X' \in
%\mathbb{R}^{n\times d}$) that are different by replacing one user's
%data.  Following definition shows this goal:

\begin{definition} [Centralized Differential Privacy (CDP)]
A randomized mechanism $\mathcal{M}: \mathcal{X} \rightarrow
\mathcal{Y}$ is said to be $(\varepsilon, \delta)$-differential
private if for any two adjacent datasets $X, X' \in \mathcal{X}$, and
any set $Y \subseteq \mathcal{Y}$:
\begin{equation}
\Pr [\mathcal{M}(X) \in Y] \leq e^{\varepsilon} \Pr [\mathcal{M}(X')
  \in Y] +\delta
\end{equation}
\end{definition}
where $\varepsilon$ is the privacy budget (lower the $\varepsilon$,
higher the privacy), and $\delta$ is the failure probability.



\subsection{Local Differential Privacy in FL (LDP-FL)}
%\red{ in which each client randomizes its local update before sending
%then to an untrusted server.  The CDP-FL provides better utility with
%cost of trusting the server, but the LDP-FL preserves strong local
%privacy with cost of low utility.}
CDP-FL relies on availability of a trusted server for collecting raw
model updates.  On the other hand, LDP-FL~\cite{wang2019collecting,
  liu2020fedsel} does not rely on this assumption and each client
perturbs its output locally using a randomizer $\mathcal{R}$
(Figure~\ref{fig:allDP}(b)).  If each client perturbs its model
updates locally by $\mathcal{R}$ which satisfies $(\varepsilon_{\ell},
\delta_{\ell})$-LDP, then observing collected updates
$\{\mathcal{R}(x_1), \dots, \mathcal{R}(x_n)\}$ also implies
$(\varepsilon_{\ell}, \delta_{\ell})$-DP~\cite{dwork2014algorithmic}.

\begin{definition} [Local Differential Privacy (LDP)]
A randomized mechanism $\mathcal{R}: \mathcal{X} \rightarrow
\mathcal{Y}$ is said to be $(\varepsilon_{\ell},
\delta_{\ell})$-locally differential private if for any two inputs $x,
x' \in \mathcal{X}$ and any output $y \in \mathcal{Y}$,:
\begin{equation}
\Pr [\mathcal{R}(x) = y] \leq e^{\varepsilon_{\ell}} \Pr
    [\mathcal{R}(x') = y] +\delta_{\ell}
\end{equation}
\end{definition}

In LDP-FL, each client perturbs its local update ($x_i$) with
$\epsilon_{\ell}$-LDP.  Unfortunately, LDP hurts the utility,
especially for high dimensional vectors.  Its mean estimation error is
bounded by $O(\frac{\sqrt{d \log{d}}}{\varepsilon_{\ell} \sqrt{n}})$
meaning that for better utility we should increase the privacy budget
or use larger number of users in each
round~\cite{bhowmick2018protection}.



\subsection{Privacy Amplification by Shuffling Clients' updates}
Recent works~\cite{liu2021flame, girgis2021shuffled} utilize the
privacy amplification effect by shuffling model parameters across
client model updates from participating clients to improve the LDP-FL
utility (illustrated in Figure~\ref{fig:allDP}(c)).  FL frameworks
based on shuffling clients' updates consists of three building
processes: $\mathcal{M}=\mathcal{A} \circ \mathcal{S} \circ
\mathcal{R}$.  Specifically, they introduce a shuffler $\mathcal{S}$,
which sits between the FL clients and the FL server, and it shuffles
the locally perturbed updates (by randomizer $\mathcal{R}$) before
sending them to the server for aggregation ($\mathcal{A}$).  More
specifically, given parameter index $i$, $\mathcal{S}$ randomly
shuffles the $i^{th}$ parameters of model updates received from the
$n$ participant clients.  The shuffler thus detaches the model updates
from their origin client (i.e. anonymizes them).  Previous
works~\cite{balle2019differentially, balcer2019separating,
  ghazi2019scalable} focused on shuffling one-dimensional data $x \in
X$, and corollary~\ref{coll-blanket-balle-generic} shows the privacy
amplification effect by shuffling.
%But Recent works~\cite{liu2021flame, girgis2021shuffled} use
%shuffling in FL for privacy amplification.  SLDP-FL introduces a
%shuffler, which sits between the FL clients and the FL server, and it
%shuffles the locally randomized updates before sending them to the
%server.  in SLDP-FL, The shuffler detaches the model updates from
%their origin client (i.e. anonymizes them).


%\begin{lemma}~\cite{balle2019privacy}
%For $\sqrt{\frac{14 \log{(2/\delta_c)}(b-1)}{n-1}}<\varepsilon_c\leq 1$,
%if $R_{\gamma,b}$ satisfies $\varepsilon_{\ell}$-LDP, we have $(\varepsilon_{c}, \delta_{c})$ 
%for shuffling the randomized outputs where $\varepsilon_c = \sqrt{\frac{14 \log{(2/\delta_c)} (e^{\varepsilon_\ell}+b-1)}{n-1}}$
%\label{thm-blanket-balle-radnomizerR}
%\end{lemma}

\begin{corollary}~\cite{balle2019privacy}
In shuffle model, if $R$ is $\varepsilon_{\ell}$-LDP, where
$\varepsilon_{\ell} \leq \log{(n / \log{(1/\delta_c)})}/2$.  $M$
statisfies $(\varepsilon_{c}, \delta_{c})$-DP with $\varepsilon_{c}=O(
(1 \wedge \varepsilon_{\ell}) e^{\varepsilon_{\ell}}
\sqrt{\log{(1/\delta_c)}/n})$ where '$\wedge$' shows minimum function.
\label{coll-blanket-balle-generic}
\end{corollary}


From above corollary, the privacy amplification has a direct
relationship with $\sqrt{n}$ where $n$ is the number of selected
clients for aggregation, i.e., increasing the number of clients will
increase the privacy amplification.  Note that in \Name, the clients
are responsible for shuffling, and instead of shuffling the $n$
clients' updates (inter-model shuffling), each client locally shuffles
its $d$ parameters (intra-model shuffling).  In real-world settings
there is a limit on the value of $n$, so the amount of amplification
we can achieve is also limited.  However, in \Name we can see much
more amplification because we are shuffling the parameters and $n \ll
d$.





\subsection{Privacy Composition}
We use following naive and strong composition
theorems~\cite{dwork2010boosting} in this paper:

\begin{lemma}[N{\"a}ive Composition]
$\forall \varepsilon \geq 0, t \in \mathbb{N}$, the family of $\varepsilon$-DP mechanism 
satisfies $t\varepsilon$-DP under $t$-fold adaptive composition.
\label{lemma-PrivacyFold1}
\end{lemma}

\begin{lemma}[Strong Composition]
$\forall \varepsilon, \delta, \delta' > 0, t \in \mathbb{N}$, the family of $(\varepsilon, \delta)$-DP mechanism satisfies
$(\sqrt{2t \ln{(1/\delta'})} \cdot \varepsilon + t \cdot \varepsilon (e^{\varepsilon} - 1), t \delta + \delta' )$-DP
under $t$-fold adaptive composition. 
\label{lemma-PrivacyFold2}

\end{lemma}




==> FedPerm/intro.tex <==
\section{Introduction}
Federated Learning (FL) is a distributed learning paradigm where
mutually untrusting \emph{clients} collaborate to train a shared
model, called the \emph{global model}, without explicitly sharing
their local training data. FL training involves a \emph{server} that
aggregates, using an \emph{aggregation rule} (AGR), model updates that
the clients compute using their local private data.  The aggregated
\emph{global model} is thereafter broadcasted by the server to a
subset of the clients.  This process repeats for several rounds until
convergence or a threshold number of rounds.  Though highly promising,
FL faces multiple challenges~\cite{kairouz2019advances} to its
practical deployment.  Two of these challenges are (i) data privacy
for clients' training data, and (ii) robustness of the global model in
the presence of malicious clients.

The data privacy challenge emerges from the fact that raw model
updates of federation clients are susceptible to privacy attacks by an
adversarial server as demonstrated by several recent
works~\cite{li2022,lim2021,nasr2019comprehensive,wei2020,zhu2019deep}.
Two classes of approaches can address this problem in significantly
different ways: First, \emph{Local Differential
  Privacy}~\cite{duchi13,kasiviswanathan08,truex20,warner65} in FL
(LDP-FL) enforces a strict theoretical privacy guarantee to model
updates of clients.  The guarantee is enforced by applying carefully
calibrated noise to the clients' local model updates using a local
randomizer $\mathcal{R}$.  In addition to the privacy guarantee,
LDP-FL can defend against poisoning attacks by malicious clients, thus
providing robustness to the global model
~\cite{nguyen2021flame,naseri2020local,sun2019can}.  However, the
model update perturbation needed for the LDP guarantee significantly
degrades model utility.

The other approach to enforce client data privacy is \emph{secure
  aggregation (sAGR)}, where model update aggregation is done using
cryptographic techniques such as homomorphic encryption or secure
multi-party computation~\cite{bonawitz2017practical,
  zhang2020batchcrypt, bell2020secure,fereidooni2021safelearn}.  sAGR
protects privacy of clients' data from an adversarial server because
the server sees just the encrypted version of clients' model updates.
Moreover, this privacy is enforced without compromising global model
utility.  However, the encrypted model updates themselves provide the
perfect cover for a malicious client to poison the global
model~\cite{fereidooni2021safelearn, nguyen2021flame} -- the server
cannot tell the difference between a honest model update and a
poisoned one since both are encrypted.
\begin{comment}
%So perhaps we can remove it or demote it to a footnote.
Furthermore, the trained model
remains susceptible to \emph{inference attacks}~\vjm{Citations
  needed}.
\end{comment}

\begin{comment}
It has been shown that sharing raw local updates with an
\emph{untrusted} server compromises clients'
privacy~\cite{nasr2019comprehensive, zhu2019deep}.  To provide local
privacy guarantees in FL against the untrusted server, two main
approaches are suggested: \emph{Locally differentially private
  federated learning (LDP-FL)}~\cite{wang2019collecting,
  liu2020fedsel} and \emph{secure aggregation
  (sAGR)}~\cite{bonawitz2017practical}.  In LDP-FL, each client
perturbs its local update by applying a randomize function
$\mathcal{R}$ which is $\varepsilon_d$-LDP, before sending to the
untrusted server.  Secure aggregation is also proposed to limit the
server inferences from the local updates, i.e., the server is only
learning the aggregated updates and not learning anything from the
clients' updates.  Secure aggregation can be achieved using different
techniques such as fully or partially homomorphic encryption or secret
sharing.  LDP-FL provides formal privacy guarantee, and it has been
shown~\cite{naseri2020local,sun2019can} that LDP-FL can defend against
poisoning attacks.  However, LDP-FL is notorious for low utility, and
this results in significant accuracy drop in the final trained model.
On the other hand, secure aggregation provides good accuracy, but it
is vulnerable to poisoning attacks as the server cannot utilize any
robust AGR to exclude the malicious poisoning updates from
aggregation.
\end{comment}

%############Fedperm###########
In this paper we answer the dual question: \emph{Can we design an
  efficient federated learning algorithm that achieves local privacy
  for participating clients at a low utility cost, while ensuring
  robustness of the global model from malicious clients?}
%The key question we try to answer is: \emph{Can we design an efficient
%  federated learning algorithm that achieves both local privacy and
%  robustness?}
To that end, we present \emph{\Name}, a new FL protocol that combines
LDP~\cite{duchi13,kasiviswanathan08,warner65}, model parameter
shuffling~\cite{erlingsson2019amplification}, and \emph{computational
  Private Information Retrieval
  (cPIR)}~\cite{chor1997computationally,chang2004single,
  aguilar2016xpir, angel2018pir}
%based techniques 
in a novel way to achieve our dual goals.
%of (i) high accuracy of secure aggregation while enforcing strong
%privacy guarantees (LDP), and (ii) robustness from model poisoning
%attacks.

The starting point of \Name{}'s design is \emph{privacy amplification
  by shuffling}~\cite{erlingsson2019amplification}, which enables
stronger (i.e., amplified) privacy with little model perturbation
(using randomizer $\mathcal{R}$) at each client.  Crucially, our
shuffling technique fundamentally differs from prior works in that we
apply \emph{intra-model} parameter shuffling rather that the
\emph{inter-model} parameter shuffling done
previously~\cite{erlingsson2019amplification,liu2021flame,
  girgis2021shuffled}.
%% indicates the
%% shuffled outputs of local randomizers provides stronger (i.e.,
%% amplified) privacy.  This means that each client needs to inject
%% smaller amount of local noise (through $\mathcal{R}$) for the same
%% final level of privacy which compensates the LDP poor utility.  In
%% this work, we provide theoretical analysis and numerical evaluations
%% of the privacy amplification by shuffling parameters in \Name.



Next, each \Name client privately chooses its \emph{shuffling pattern}
uniformly at random for each FL round.  To aggregate the shuffled (and
perturbed) model parameters, \Name client utilizes cPIR to generate a
set of PIR queries for its shuffling pattern that allows the server to
retrieve each parameter \emph{privately} during aggregation.  All the
server observes is the shuffled parameters of the model update for
each participating client, and a series of PIR queries (i.e., the
encrypted version of the shuffling patterns).  The server can
aggregate the PIR queries and their corresponding shuffled parameters
for multiple clients to get the encrypted aggregated model.  The
aggregated model is decrypted independently at each client.
%We propose different methods to decrypt the encrypted aggregated
%model based on assumptions about the underlying threat models.


\begin{comment}
utilizes a cPIR technique based on partial homomorphic encryption
(PHE)~\cite{paillier1999public, damgaard2001generalisation} that allows the server to retrieve
each parameter privately during aggregation.  All the server observes
is the shuffled parameters of the model for each participating client,
and an encrypted version of the \emph{unshuffled} parameters that is
retrieved using the cPIR technique~\vjm{Is there a name for the
  technique?}.  The server can aggregate the encrypted unshuffled
parameters of multiple clients to get the encrypted aggregated model.
We propose different  methods to decrypt the encrypted
aggregated model based on assumptions about the underlying threat
models.
\end{comment}

The combination of LDP at each client and intra-model parameter
shuffling achieves enough privacy amplification to let \Name\ preserve
high model utility.  At the same time, availability of the shuffled
parameters at the federation server lets it control a client's model
update contribution by enforcing norm-bounding, which is known to be
highly effective against model poisoning
attacks~\cite{nguyen2021flame,naseri2020local,sun2019can}.



Since \Name\ utilizes cPIR which relies on homomorphic encryption
(HE)~\cite{paillier1999public, damgaard2001generalisation}, it can be
computationally expensive, particularly for large models.  We present
computation/utility trade off hyper-parameters in \Name, that enables
us to achieve an interesting trade off between computational
efficiency and model utility.  In particular, we can adjust the
computation burden for a proper utility goal by altering the size and
number of shuffling patterns for the \Name clients.

\begin{comment}
Since \Name\ relies on PHE, it can be computationally expensive,
particularly for large models.  We present two additional variants of
\Name, called \emph{\Name-light} and \emph{\Name-heavy}, that achieve
an interesting trade off between computational efficiency and model
utility.  We continue to enforce the same privacy guarantee and model
robustness in both these variants.
\end{comment}

%Private information retrieval (PIR) is a technique to provide query
%privacy to users when fetching sensitive records from untrusted
%databases~\vjm{[Reference needed here]}.  That is, cPIR enables users
%to query and retrieve specific records from untrusted database in a
%way that the serving database cannot identify the records
%retrieved~\vjm{Presumably the cPIR reference covers this, if not
%please provide the pertinent reference}.

\begin{comment}
Operationally, in each round of \Name, clients (\emph{i}) learn their
local updates, (\emph{ii}) perturb their updates using a randomizer
$\mathcal{R}$ that provides $\varepsilon_{d}$-LDP guarantee,
(\emph{iii}) shuffle the parameters inside their randomized updates,
(\emph{iv}) create a cPIR query to retrieve each parameter privately
in the shuffled update, and (\emph{v}) send their shuffled update and
PIR query to the \Name server.  After collecting all the local updates
from the clients, the \Name server
%first checks the norm of each update to avoid poisoning attacks and then
aggregates the local updates and produces the global update for next
round.  Since this aggregated global update is encrypted, we proposed
different methods to decrypt it based on assumptions about the
underlying threat models.
\end{comment}

%After collecting all the all the shuffled updates and their cPIR
%queries from the clients, the \Name server (\emph{i}) checks the norm
%of each update to avoid poisoning attacks, (\emph{ii}) multiplies
%each clients query to its shuffled parameters to find its unshuffled
%encrypted update, (\emph{iii}) sums all the encrypted unshuffled
%parameters to find the encrypted global model which can be decrypted
%by the clients.


%############Intuituions###########
%\paragraphb{\em Intuitions on \Name's privacy amplification:} Each
%\Name client, first applies a randomize function $\mathcal{R}$ which
%is $\varepsilon_d$-LDP on its parameters, and then shuffles them
%before sending them to the server.

\begin{comment}
\paragraphb{\em Intuitions on \Name's robustness to poisoning
  attacks:} In traditional FL algorithms with secure aggregation, the
local updates are encrypted, providing malicious clients a significant
flexibility in fabricating poisoning updates.  It is
shown~\cite{blanchard2017machine} that even a single malicious client
can mount an effective untargeted attack on FedAvg by sending very
large parameters in its local update.  By contrast, \Name clients
provide their actual parameter values, without any encryption or
obfuscation, but in a shuffled order that each parameter is detached
from its position, which allows the server to check the norm of
updates before aggregating them into the global model. Please note
that unlike other robust AGRs, \emph{norm bounding} (what we have in
DP) is the only robust AGR that only needs the values of the update
parameters without access to their order by calculating the
$\bar{x_i}\gets x_i \cdot \min(1, \frac{C}{{||x_i||}_2})$ where $x_i$
is the local update vector and $C$ the maximum $\ell_2$ norm possible.
\end{comment}

%############empirical results###########
%\paragraphb{\em Empirical results:}
%We provide a formal analysis of our algorithms' privacy guarantees.
We empirically evaluate \Name on the MNIST dataset to demonstrate that
it is possible to provide LDP-FL guarantees at low model utility cost.
%with only negligible cost in final test accuracy by leveraging the
%privacy amplification effect of shuffling parameters.
We theoretically and numerically demonstrate a trade off between model
utility and computational efficiency. Specifically, \Name's
hyperparameters create \emph{shuffling windows} whose size can be
reduced to drastically cut computation overheads, but at the cost of
reducing model utility due to lower privacy amplification.  We
experiment with two representative shuffling window configurations in
\Name -- ``light'' and ``heavy''.  For a $(4.0, 10^{-5})$-LDP
guarantee, the light version of \Name, where client encryption, and
server aggregation needs $52.2$ seconds and $21$ minutes respectively,
results in a model that delivers $32.85\%$ test accuracy on MNIST.
The heavier version of \Name, where client encryption and server
aggregation needs $32.1$ minutes and $16.4$ hours respectively,
results in $72.38\%$ test accuracy.  Non-private FedAvg, CDP-FL and
LDP-FL provide $91.02\%$, $53.50\%$, and $13.74\%$ test accuracies for
the same $(\varepsilon, \delta)$-DP guarantee respectively.





\iffalse
In summary, we propose a federated learning approach that is built on using private information retrieval (PIR), 
Our key contributions are as follows:
\begin{itemize}
\item We propose the first secure aggregation protocol, \Name, by shuffling the parameters and utilizing PIR for aggregating shuffled updates.
\item We show that \Name significantly reduces the 
\item 
\item We evaluate \Name on the real-world benchmark dataset (MNIST), and show that 
\end{itemize}
\fi










==> FedPermDP.tex <==





\section{Privacy Guarantees by Shuffling Parameters}

\subsection{\Name}
In \Name, each client randomizes each value in its updates with randomizer $\mathcal{R}$ and then shuffle all the $d$ values (i.e., parameters in the local update) that each value is $\varepsilon_{w}$-LDP.
From Corollary~\ref{coll-blanket-balle-generic}, we can show Corollary~\ref{coll-FedPermDP1}. 
The intuition is that we map the clients in Corollary~\ref{coll-blanket-balle-generic} to parameters in Corollary~\ref{coll-FedPermDP1}. 
This means in \Name, the number of clients participating in shuffling ($n$) will be replaced by number of parameters ($d$).


\begin{corollary}
If $\mathcal{R}$ is $\varepsilon_{w}$-LDP, where $\varepsilon_{w} \leq \log{(d / \log{(1/\delta_{\ell})})}/2$,
\Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{d} \circ \mathcal{R}$ satisfies $(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w}) e^{\varepsilon_{w}} \sqrt{\log{(1/\delta_{\ell})}/d})$.
\label{coll-FedPermDP1}
\end{corollary}

We know that $\varepsilon_{w} = \varepsilon_{d}/d$ so Corollary~\ref{coll-FedPermDP5} shows the privacy amplification based on $\varepsilon_{d}$.

\begin{corollary}
If $\mathcal{R}$ is $\varepsilon_{w}$-LDP, where $\varepsilon_{w} = \varepsilon_{d}/d$ and $\varepsilon_{d} \leq d \cdot \log{(d / \log{(1/\delta_{\ell})})}/2$,
\Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{d} \circ \mathcal{R}$ satisfies $(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/d) e^{(\varepsilon_{d}/d)} \sqrt{\log{(1/\delta_{\ell})}/d})$.
\label{coll-FedPermDP5}
\end{corollary}










%-------------------------------------------------------------Fedperm with k1--------------------------------------------

\subsection{\Name with Window Size $k_1$}


\paragraphb{Superwindow}: If we have $w=d/k_1$ windows, then each window has $k_1$ parameters. If we look at the update $\theta$ with $d$ parameters as $\mathbb{R}^{k_1 \times w}$ (a matrix with $k_1$
rows and $w$ columns), each column is a window and each row is a superwindow. For example, for above example, each row of matrix $\theta$ is a superwindow. 
This means that in \Name, we have $k_1$ superwindows and each super window has $w=d/k_1$ elements. 

Now, since the shuffling is applied on the superwindows, then we need to make each superwindow $\varepsilon_w$-LDP using a randomizer $\mathcal{R}^w$.
Theorem~\ref{thm-FedPermDP2a} shows that \Name with $k_1$ as window size is $(\varepsilon_{\ell}, \delta_{\ell})$-DP. 

\begin{theorem}
For \Name $\mathcal{F}=\mathcal{A}  \circ \mathcal{S}_{k_1} \circ \mathcal{R}^{w}$ with window size $k_1$, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP and $\varepsilon_{w} \leq \log{(k_1 / \log{(1/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w}) e^{\varepsilon_{w}} \sqrt{\log{(1/\delta_{\ell})}/k_1}$. 
\label{thm-FedPermDP2a}
\end{theorem}

\begin{corollary}
For \Name $\mathcal{F}=\mathcal{A}  \circ \mathcal{S}_{k_1} \circ \mathcal{R}^{w}$ with window size $k_1$, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP, $\varepsilon_{w} = \varepsilon_{d}/k_1$ and $\varepsilon_{d} \leq k_1 \cdot \log{(k_1 / \log{(1/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/k_1) e^{(\varepsilon_{d}/k_1)} \sqrt{\log{(1/\delta_{\ell})}/k_1}$. 
\label{thm-FedPermDP2b}
\end{corollary}





This Theorem is the result of applying Corollary~\ref{coll-blanket-balle-generic} on the superwidnows.


%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/fedperm_epsc_k1_B.png} 
%\caption{Effect of $k_1$ and $\varepsilon_{wd}$ on the central privacy budget. We illustrate the overal amplification with Bennett inequality for the Laplace Mechanism.}
%\label{fig1}
%\end{figure}







%-------------------------------------------------------------Fedperm with k1 and k2--------------------------------------------
\subsection{\Name with Window Size $k_1$ and $k_2$ Patterns}


When we have $k_2$ patterns, it is like running \Name for $k_2$ times with $k_1$ users 
participating in FL that each one have a local update with $w=d/(k_1 k_2)$ parameters.
In this case, the size of each super window is $w=d/(k_1 k_2)$.
Therefore, each client needs to apply a randomizer $\mathcal{R}^w$ with $\varepsilon_{w}$ on its superwindows.

Theorem~\ref{thm-FedPermDP3a} shows that \Name with $k_1$ as window size and $k_2$ as the number of different shuffling patterns is $(\varepsilon_{\ell}, \delta_{\ell})$-DP. 


\begin{theorem}
For \Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{k_1}^{k_2} \circ \mathcal{R}^{w}$ with window size $k_1$, and $k_2$ shuffling patterns, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP and $\varepsilon_{w} \leq \log{( k_1 / \log{((k_2 +1)/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w}) e^{\varepsilon_{w}} \log{(k_2/\delta_{\ell})} \sqrt{k_2/k_1})$. 
\label{thm-FedPermDP3a}
\end{theorem}


\begin{corollary}
For \Name $\mathcal{F}=\mathcal{A}  \circ \mathcal{S}_{k_1}^{k_2} \circ \mathcal{R}^{w}$ with window size $k_1$, and $k_2$ shuffling patterns, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP, $\varepsilon_{w} = \varepsilon_{d} / (k_1 k_2)$ and $\varepsilon_{d} \leq (k_1 k_2) \cdot \log{( k_1 / \log{((k_2 +1)/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/(k_1 k2)) e^{(\varepsilon_{d}/(k_1 k2))} \log{(k_2/\delta_{\ell})} \sqrt{k_2/k_1})$. 
\label{coll-FedPermDP3b}
\end{corollary}




This Theorem is the result of first applying Corollary~\ref{coll-blanket-balle-generic} on the superwidnows and then applying advanced composition on $k_2$ components. 


\begin{figure}[h!]
\centering
\begin{subfigure}{.22\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{Images/fedperm_epsc_k1_B.png}  
    \caption{Impact of $k_1$ and $\varepsilon_{wd}$.}
    \label{fig:Priv1}
\end{subfigure}
\begin{subfigure}{.22\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{Images/fedperm_epsc_k1k2.png}  
    \caption{Imapct of $k_1$ and $k_2$,}
    \label{fig:Priv2}
\end{subfigure}
\begin{subfigure}{.22\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{Images/fedperm_epsc_d.png}  
    \caption{Impact of $d$ and $\varepsilon_{wd}$.}
    \label{fig:Priv3}
\end{subfigure}
\caption{We illustrate the overal amplification with Bennett inequality for the Laplace Mechanism.}
\label{fig:Priv-ALL}
\end{figure}

\paragraphb{Privacy Analysis} In Figure~\ref{fig:Priv-ALL},  we show the relationship of our introduced varibales $k_1$, $k_2$, $\varepsilon_w$ and $\varepsilon_{wd}$ on the privacy amplifiction in \Name. 
Figure~\ref{fig:Priv1} shows the relationship of 
Figure~\ref{fig:Priv2}
Figure~\ref{fig:Priv3}




\subsection{Privacy Gurantee for T rounds}
We are doing Fedperm for a sequence of T adaptive $\mathcal{F}_1,\dots, \mathcal{F}_T$ where each $\mathcal{F}_t$ for $t \in [T]$ staitisifes the privacy gurantees stated in Theroemes~\ref{} dends on using pure \Name,  or $k_1$ or $k_2$.
Now we invoke the strong compositing stated in Lemma~\ref{} to obtain the pruvacy gurantee of the \Name for $T$ rounds.  We can conlude that for any $\delta'>0$,  \Name is $(\varepsilon, \delta)$-DP for 
\begin{equation}
	\varepsilon = \sqrt{2T\log{(1/\delta')}} \varepsilon_{\ell} + T \varepsilon_{\ell} (e^{\varepsilon_{\ell}}-1),  \delta=T \delta_{\ell}+ \delta'
\end{equation}



































==> FedPerm_TM.tex <==
\section{\Name: Private Federated Learning by parameter Permutation}

\begin{comment}
FL involves mutually untrusting clients.  Hence, a \emph{poisoning
  adversary} may own or compromise some of the FL clients, called
\emph{malicious clients}, with the goal of mounting a \emph{targeted}
or \emph{untargeted} poisoning attack.  In a targeted
attack~\cite{bhagoji2019analyzing, sun2019can}, the goal is to reduce
the utility of the model on specific test inputs, while in the
untargeted attack~\cite{baruch2019a,
  fang2020local,shejwalkar2021manipulating}, the goal is to reduce the
utility for all (or most) test inputs. It is
shown~\cite{blanchard2017machine} that even a single malicious client
can mount an effective untargeted attack on FedAvg.

Using secure aggregation makes it very easy for the poisoning
adversary to craft very large updates and destroy the global model
without being detected.  In order to make FL robust to the presence of
such malicious clients, the literature has designed various
\emph{robust aggregation rules (AGR)}~\cite{blanchard2017machine,
  mozaffari2021fsl, YinCRB18,chang2019cronus}, which aim to remove or
attenuate the updates that are more likely to be malicious according
to some criterion.  Unfortunately, these robust AGRs are not usable in
an FL with secure aggregation because the parameters are encrypted or
secrete shared.  On the other hand, it has been
shown~\cite{naseri2020local,sun2019can} that LDP-FL can defend against
targeted and untargeted attacks as the model updates are bounded.

In this work, we present \Name, a novel approach to perform FL while
concurrently achieving two goals of privacy and robustness.  \Name
provides higher utility compared to LDP-FL as each client is shuffling
the parameters, so the privacy is amplified (i.e. less noise is
required for the same level of LDP).  In this section, we describe our
algorithm overview and clarify different threat models we consider in
this paper.
\end{comment}
\vjm{Removed 3 paras from here since they seem redundant.}
We now overview \Name\ and decsribe different threat models we
consider in our work.

\subsection{\Name Overview} 
Figure~\ref{fig:allDP}(d) depicts the \Name framework that consists of
three components, $\mathcal{F} = \mathcal{A} \circ \mathcal{S} \circ
\mathcal{R}^{d}$.
In \Name:
\textbf{(1)} There are $N$ total clients and $n$ clients are selected
randomly in each round.  Each selected client $i$ computes its local
update $x_i \in \mathbb{R}^d$ and applies a local
randomizer $\mathcal{R}^d$ on it to produce $y_i \in \mathbb{R}^d$.
\textbf{(2)} Now each client shuffles (i.e., $\mathcal{S}$) the
parameters inside $y_i$ to produce $y_i^{\pi_i}$ where $\pi_i$ is a
random shuffling pattern that the client $i$ produces for each
round.  Note that the shuffling occurs inside the clients and
there is no need for a trusted shuffler outside the client in \Name.
The client also creates an encrypted PIR query $c_i$. Then
the client sends $(y_i^{\pi_i}, c_i)$ to the server for aggregation.
\textbf{(3)} After collecting all the shuffled local updates, with
corresponding encrypted PIR query, from $n$ clients, the server
aggregates (i.e., $\mathcal{A}$) the local updates to produce the
global update for next round.  As this global aggregated update is
encrypted, so we propose different decryption methods relevant
different thread models discussed below.




==> test_dir/FedPerm/AdvFedPerm.tex <==
\section{Computation/Communication and Utility Tradeoff in \Name}
\label{sec:FedpermAdv}

%\subsection{Privacy and Computation/Communication Cost in \Name}

Each \Name client perturbs its local update (vector $x_i$ containing
$d$ parameters) with randomizer $\mathcal{R}^d$ which is
$\varepsilon_d$-LDP, and then shuffles its parameters.  We use the
Laplacian mechanism as the randomizer.  Based on the n\"aive
composition theorem from Lemma~\ref{lemma-PrivacyFold1}, the
client perturbs each parameter value with $\mathcal{R}$ which
satisfies $\varepsilon_{wd}$-LDP where
$\varepsilon_{wd}=\frac{\varepsilon_d}{d}$ (Appendix~\ref{sec:Laplace}
contains additional details).  Corollary~\ref{coll-FedPermDP11} shows
the privacy amplification from $\varepsilon_d$-LDP to
$(\varepsilon_{\ell}, \delta_{\ell})$-DP after the parameter
shuffling.  Corollary~\ref{coll-FedPermDP11} is derived from
Corollary~\ref{coll-blanket-balle-generic}, by substituting the number
of participating clients $n$ by the number of parameters $d$ in the
model.

\begin{corollary}
If $\mathcal{R}$ is $\varepsilon_{wd}$-LDP, where $\varepsilon_{wd} \leq
\log{(d / \log{(1/\delta_{\ell})})}/2$, \Name $\mathcal{F}=\mathcal{A}
\circ \mathcal{S}_{d} \circ \mathcal{R}^d$ satisfies
$(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O(
(1 \wedge \varepsilon_{wd}) e^{\varepsilon_{wd}}
\sqrt{\log{(1/\delta_{\ell})}/d})$.
\label{coll-FedPermDP11}
\end{corollary}

Thus, larger the number of parameters in the model, greater is the
privacy amplification.  With large models containing millions or
billions of parameters, the privacy amplification can be immense.
However, the model dimensionality also affects the computation (and
communication) cost in \Name.  Each \Name client generates a
$d$-dimensional PIR query for every parameter in the model, resulting
in a PIR query matrix containing $d^2$ entries.  This results in a
quadratic increase in client encryption time, server aggregation time,
and client-server communication bandwidth consumption.  This increase
in communication, and more importantly computation, resources is
simply infeasible for large models containing billions of parameters.
To address this problem \Name introduces additional hyperparameters
that present an interesting trade off between
computation/communication overheads and model utility.

\begin{comment}
\subsection{Computation/Communication Cost of \Name}



In this section, we first show the privacy level and
computation/communication cost of \Name and then introduce new
hyperparameters for \Name to adjust the computation/communication cost
vs.  utility tradeoff.  In particular, for a fixed privacy budget, if
we increase the computation and communication resources, we can train
a more accurate model as we need to inject less local noise (as the
result of privacy amplification of shuffling the parameters).
Corollary~\ref{coll-FedPermDP11} shows the privacy amplification from
$\varepsilon_d$-LDP to $(\varepsilon_{\ell}, \delta_{\ell})$-DP after
the parameter shuffling.  Corollary~\ref{coll-FedPermDP11} is derived
from Corollary~\ref{coll-blanket-balle-generic}, by substituting the
number of participating clients $n$ by the number of parameters $d$ in
the model.


\subsection{Privacy vs.  Computation/Communication in \Name}

Each \Name client perturbs its local update (vector $x_i$ containing
$d$ parameters) with randomizer $\mathcal{R}^d$ which is
$\varepsilon_d$-LDP, and then shuffles its parameters.  We use Laplace
Mechanism as the randomize function $\mathcal{R}$ in \Name design.
Based on the na\"ive composition theorem described in
Lemma~\ref{lemma-PrivacyFold1}, the client perturbs each parameter
value with $\mathcal{R}$ which satisfies $\varepsilon_{wd}$-LDP where
$\varepsilon_{wd}=\frac{\varepsilon_d}{d}$.  We explain more about
this parameter randomizing in Appendix~\ref{sec:Laplace}.
Corollary~\ref{coll-FedPermDP11} shows the privacy amplification from
$\varepsilon_d$-LDP to $(\varepsilon_{\ell}, \delta_{\ell})$-DP after
the parameter shuffling.  Corollary~\ref{coll-FedPermDP11} is derived
from Corollary~\ref{coll-blanket-balle-generic}, where in \Name we are
\emph{intra-model} parameter shuffling instead of \emph{inter-model}
client update shuffling in Corollary~\ref{coll-FedPermDP11}.  This
means in \Name, the number of clients participating in shuffling ($n$)
will be replaced by number of parameters ($d$).




\begin{corollary}
If $\mathcal{R}$ is $\varepsilon_{d}$-LDP, where $\varepsilon_{d} \leq \log{(d / \log{(1/\delta_{\ell})})}/2$,
\Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{d} \circ \mathcal{R}^d$ satisfies $(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}) e^{\varepsilon_{d}} \sqrt{\log{(1/\delta_{\ell})}/d})$.
\label{coll-FedPermDP11}
\end{corollary}



In \Name, each client encrypts $d^2$ values of $\{0,1\}$ for PIR query
generation, and it consumes $O(d^2)$ extra upload bandwidth to send
the PIR query along with the shuffled parameters.  This makes the
client encryption time, server aggregation time, and client upload
bandwidth consumption increase quadratically with $d$ (number of
parameters).
%Table~\ref{tab:FedpermResult1} shows encryption time (at clients),
%server aggregation time, and decryption time at clients for different
%values of $d$.
Existing deep neural networks have a large number of parameters which
makes the \Name very expensive.  In following, we present
computation/communication-utility tradeoff hyperparameters for \Name
to adjust the computation/communication burden for a proper utility
goal.
 %introduce additional mechanisms to decrease these costs.

\end{comment}


%###############################k1###########################

\subsection{\Name with Smaller Shuffling Pattern}

%In \Name, each client generates $d$ PIR queries, that each one
%requires $d$ encryptions.  To reduce the size of each PIR query, we
%need to reduce the size of shuffling patterns ($\pi_u$ for user $u$),
%which is secret for each client.  To do so,

Instead of shuffling all the $d$ parameters, the \Name client can
partition its parameters into several identically sized windows, and
shuffle the parameters in each window with the \emph{same} shuffling
pattern.  Thus, instead of creating a very large random
shuffling pattern $\pi$ with $d$ indices (i.e.,
$\pi=\textsc{RandomPermutations}[1,d]$), each client creates a
shuffling pattern with $k_1$ indices (i.e.,
$\pi=\textsc{RandomPermutations}[1,k_1]$), and shuffles
($\mathcal{S}_{k_1}$) each window with these random indices.
%Note that the same shuffling pattern will be applied inside each
%window.

The window size $k_1$ is a new \Name hyperparameter that can be used
to control the computation/communication and model utility trade off.
%Now, we can adjust \Name computation and communication cost by
%choosing a proper window size ($k_1$).
Once we set the size of shuffling pattern to $k_1$, each client needs
to perform $d \cdot k_1$ encryptions and consumes $O(d \cdot k_1)$
network bandwidth to send its PIR queries to the server.
%Note that \Name without window size means $k_1=d$.  By random
%guessing, the adversary's success rate of finding the right order of
%parameters in \Name is $\frac{1}{d!}$ as there are $d!$ possible
%permutation of parameters.  When we are shuffling with smaller
%shuffling pattern with $k_1$ indices, the adversary's success
%probability of finding the original order is $\frac{1}{k_1!}$.


\paragraphb{Superwindow:} A shuffling window size of $k_1$, partitions
each \Name client $u$'s local update $x_u$ ($d$ parameters) into
$w=d/k_1$ windows, each containing $k_1$ parameters.  Each \Name
client, independently from other \Name clients, chooses its shuffling
pattern $\pi$ uniformly at random with indices $\in [1,k_1]$, and
shuffles each window with this pattern.  This means that every
position $j$ ($1\le j \le k_1$) in each window $k$ ($1\le k \le w$)
will have the same permutation index ($\pi_j$).  Thus all of the
$j^{th}$ positioned parameters ($x_u^{(k,j)} \; \text{for} \; 1\le k
\le w$) will contain the value from the $\pi_j^{th}$ slot in window
$k$.
%be shuffled with the same pattern $\pi_j$.
For a given index $j$ ($1\le j \le k_1$), we define a
\emph{superwindow} as the set of all of the parameters $x_u^{(k,j)}$
for $1\le k \le w$.  If we structure the parameter vector $x_u$ (with
$d$ parameters) as $\mathbb{R}^{k_1 \times w}$ (a matrix with $k_1$
rows and $w$ columns), each row of this matrix is a superwindow.


%The local update $\theta$ with $d$ parameters can be seen as a set of
%windows where we have $w=d/k_1$ windows and each window has $k_1$
%parameters.  If we look at the update $\theta$ with $d$ parameters as
%$\mathbb{R}^{k_1 \times w}$ (a matrix with $k_1$ rows and $w$
%columns), we define \emph{superwindow} as each row of this matrix.
%It means that the parameters inside each superwindow gets permuted
%with the same shuffling pattern.

\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{Images/superwindow.pdf} 
\vspace{-0.15in}
\caption{\Name example with $k_1=3$ and $d=12$. The red boxes are
  showing the windows that the parameters inside them are going to be
  shuffled with the same shuffling pattern $\pi$.}
\label{fig:example}
\end{figure}

Figure~\ref{fig:example} depicts an example model containing $12$
parameters $\theta=[\theta_1, \theta_2, ..., \theta_{12}]$.  The
original \Name algorithm mandates a shuffling pattern $\pi$ with $12$
indices $\in [1,12]$, where the PIR query generates $12\times12=144$
encryptions.  However, a shuffling pattern $\pi$ of three indices
$k_1=3$ ($\pi=[3,1,2]$ in the figure) requires only $3\times3=9$
encryptions.  This shuffling pattern creates $4$ windows of size $3$
(red boxes in the 2-D matrix in the figure), and each row in the 2-D
matrix, represented more succintly by $[\Theta_A,\Theta_B,\Theta_C]$,
itself constitutes a superwindow.  The shuffling pattern $\pi=[3,1,2]$
applied to $\theta = [\Theta_A,\Theta_B,\Theta_C]$ swaps entire
superwindows to give $\mathcal{S}_{k_1}(\theta) =
[\Theta_C,\Theta_A,\Theta_B]$.


\begin{comment}

\paragraphb{Example:} Suppose one client has a model update of 12
parameters $\theta=[\theta_1, \theta_2, ..., \theta_{12}]$.  If we
want to use the original \Name, the client needs to create a shuffling
pattern $\pi$ with 12 indices $\in [1,12]$, where in PIR query
generation it needs, $12\times12=144$ encryptions.  However, if the
client create a shuffling pattern of three indices (e.g,$\pi=[3,1,2]$
with $k_1=3$), then it only requires $3 \times 3=9$ encryptions.
Figure~\ref{fig:example} shows how the client breaks the update
parameters into windows for applying the shuffling pattern $\pi$.  The
\Name client first divides the parameters into $w=4$ windows each
contains $k_1=3$ parameters (shown with red boxes), and permutes
parameters inside each window with the same shuffling pattern $\pi$.
Here, each row of the matrix is a superwindow, and the elements of
superwindows are shuffled with the same shuffling pattern.

%This means that in \Name, we have $k_1$ superwindows and each super window has $w=d/k_1$ elements. 
%If we choose $k_1=3$, then we have 4 windows where each row is a superwindow. 
%Each column is a window, and parameters inside each window are going to be shuffled. 


\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{Images/superwindow.pdf} 
\vspace{-0.15in}
\caption{\Name example with $k_1=3$ and $d=12$. The red boxes are
  showing the windows that the parameters inside them are going to be
  shuffled with the same shuffling pattern $\pi$.}
\label{fig:example}
\end{figure}


%\begin{equation}
%\theta=
%\begin{bmatrix}
%\Theta_A \\
%\Theta_B \\
%\Theta_C
%\end{bmatrix}
%=
%\begin{bmatrix}
%\theta_1 & \theta_4 & \theta_7 & \theta_{10}\\
%\theta_2 & \theta_5 & \theta_8 & \theta_{11} \\
%\theta_3 & \theta_6 & \theta_9 & \theta_{12} 
%\end{bmatrix}
%\end{equation}



Above example is equivalent to a scenario in FL when we have an external shuffler (doing inter-model parameter shuffling, where there are $3$ clients and each one has a local update of 4 parameters $\Theta_u$. 
In this case, client 1 update is 
$\Theta_A = [\theta_1, \theta_4, \theta_7, \theta_{10}]$, client 2 update is $\Theta_B = [\theta_2, \theta_5, \theta_8, \theta_{11}]$ and client 3 update is $\Theta_C= [\theta_3, \theta_6, \theta_9, \theta_{12}]$.
Now the inter-model shuffler permutes the updates $[\Theta_A, \Theta_B, \Theta_C]$ uniformly randomly with shuffling pattern $\pi=[3,1,2]$.
The output of the inter-model shuffler would be $\mathcal{S}_{k_1}(\theta)=[\Theta_C, \Theta_A, \Theta_B]$ where all the parameters in the first row of $\theta$ goes to the second row of shuffling output,  the second row goes to the third row, and so on.

%If we have $w=d/k_1$ windows, then each window has $k_1$ parameters. 

\end{comment}

Shuffling of superwindows, instead of individual parameters, leads to
a significant reduction in the computation (and communication)
overheads for \Name clients.  However, this comes at the cost of
smaller privacy amplification.  Corollary~\ref{thm-FedPermDP2a} shows
the privacy amplification of \Name from $\varepsilon_d$-LDP to
$(\varepsilon_{\ell}, \delta_{\ell})$-DP after superwindow shuffling
(with window size $k_1$).  After applying the randomizer $\mathcal{R}$
that is $\varepsilon_d$-LDP on the local parameters, each superwindow
is $\varepsilon_w$-LDP where $\varepsilon_w=w \cdot
\varepsilon_{wd}=\frac{d}{k_1} \cdot
\varepsilon_{wd}=\frac{\varepsilon_{d}}{k_1}$.  Since we are shuffling
the superwindows, we can derive Corollary~\ref{thm-FedPermDP2a} for
\Name by setting the shuffling pattern size to $k_1$ from
Corollary~\ref{coll-blanket-balle-generic}.  
%Furthermore, replacing
%the number of clients $n$ with the number of superwindows $k_1$ gives
%us:

%the shuffling is applied on the superwindows, From
%Corollary~\ref{coll-blanket-balle-generic}, we can show
%Corollary~\ref{thm-FedPermDP2a} where \Name with $k_1$ as window size
%is $(\varepsilon_{\ell}, \delta_{\ell})$-DP.


% then we need to make each superwindow $\varepsilon_w$-LDP using a
%randomizer $\mathcal{R}^w$.  Theorem~\ref{thm-FedPermDP2a} shows that
%\Name with $k_1$ as window size is $(\varepsilon_{\ell},
%\delta_{\ell})$-DP.


%For example, for above example, each row of matrix $\theta$ is a
%superwindow.  This means that in \Name, we have $k_1$ superwindows
%and each super window has $w=d/k_1$ elements.



\begin{corollary}
For \Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{k_1} \circ
\mathcal{R}^{w}$ with window size $k_1$, where $\mathcal{R}^w$ is
$\varepsilon_w$-LDP and $\varepsilon_{w} \leq \log{(k_1 /
  \log{(1/\delta_{\ell})})}/2$, the amplified privacy is
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w}) e^{\varepsilon_{w}}
\sqrt{\log{(1/\delta_{\ell})}/k_1}$.
\label{thm-FedPermDP2a}
\end{corollary}

%\begin{corollary} For \Name $\mathcal{F}=\mathcal{A} \circ
%\mathcal{S}_{k_1} \circ \mathcal{R}^{w}$ with window size $k_1$,
%where $\mathcal{R}^w$ is $\varepsilon_w$-LDP, $\varepsilon_{w} =
%\varepsilon_{d}/k_1$ and $\varepsilon_{d} \leq k_1 \cdot \log{(k_1 /
%\log{(1/\delta_{\ell})})}/2$, the amplified privacy is
%$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/k_1)
%e^{(\varepsilon_{d}/k_1)}
%\sqrt{\log{(1/\delta_{\ell})}/k_1}$.  \label{thm-FedPermDP2b} \end{corollary}





%This Theorem is the result of applying
%Corollary~\ref{coll-blanket-balle-generic} on the superwidnows.











%##############################k2###########################################
\subsection{\Name with Multiple Shuffling Patterns}

%In previous section, we assume that each \Name client permutes the
%parameters inside each window with the same shuffling pattern
%($\pi$).
An additional way to adjust the computation/communication vs. utility
trade off is by using multiple shuffling patterns.  Each \Name client
chooses $k_2$ shuffling patterns $\{\pi_1, \dots, \pi_{k_2}\}$
uniformly at random where each
$\pi_i=\textsc{RandomPermutations}[1,k_1] \; \text{for} \; 1 \le i \le
k_2$.  Then, each \Name client partitions the $d$ parameters into
$d/k_1$ windows, where it permutes the parameters of window $k$ ($1
\le k \le d/k_1$) with shuffling pattern $\pi_{i} \; \text{s.t.}\; i=k
\; \text{mod} \; k_2$.  In this case, each \Name client needs $k_2
\cdot k_1^2$ encryptions to generate the PIR queries.



%In this section, we are analyzing the privacy amplification of \Name
%when we have $k_2$ shuffling patterns.

%\paragraphb{Example:}
Figure~\ref{fig:example2} shows \Name for $d=12$, $k_1=3$ and $k_2=2$,
i.e., there are two shuffling patterns $\pi_1$ (shown with red box)
and $\pi_2$ (shown with blue box) and each one has 3 shuffling
indices.  In this example, the client partitions the 12 parameters
into $4$ windows that it shuffles with $\pi_1$ (1st and 3rd windows)
and $\pi_2$ (2nd and 4th windows).  This example is equivalent to an
FL scneario with \emph{two} external inter-model shufflers (with
shuffling patterns $\pi_1, \pi_2$) and three FL clients ($A,B,C$).
Each client sends $2$ ($w=d/(k_1 k_2)$) parameters to each shuffler
for shuffling with other clients.  Two different shuffling patterns
$\pi_1$ and $\pi_2$ are applied on $[\Theta_{A1}, \Theta_{B1},
  \Theta_{C1}]$ and $[\Theta_{A2}, \Theta_{B2}, \Theta_{C2}]$
respectively.



\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{Images/superwindow_k2.pdf} 
\vspace{-0.15in}
\caption{\Name example with $k_1=3$ and $k_2=2$. We have two shuffling patterns $\pi_1$ and $\pi_2$ shown with red and blue boxes.}
\label{fig:example2}
\end{figure}


%\begin{equation}
%\theta=
%\begin{bmatrix}
%\Theta_{A1} & \Theta_{A2} \\
%\Theta_{B1} & \Theta_{B2} \\
%\Theta_{C1}, & \Theta_{C2}
%\end{bmatrix}
%=
%\begin{bmatrix}
%[\theta_1, \theta_7] & [\theta_4, \theta_{10}]\\
%[\theta_2, \theta_8] & [\theta_5, \theta_{11}] \\
%[\theta_3, \theta_9] & [\theta_6, \theta_{12}] 
%\end{bmatrix}
%\end{equation}




%When we have $k_2$ patterns, it is like running \Name for $k_2$ times
%with $k_1$ users participating in FL that each one have a local
%update with $w=d/(k_1 k_2)$ parameters.
When we have $k_2$ shuffling patterns and each shuffling pattern has
$k_1$ indices, the size of each superwindow is $w=d/(k_1 k_2)$.
Therefore, each client perturbs each superwindow with a randomizer
$\mathcal{R}^w$ that satisfies $\varepsilon_{w}$-LDP where
$\varepsilon_w=w \cdot \varepsilon_{wd}=\frac{d}{k_1 k_2} \cdot
\varepsilon_{wd}=\frac{\varepsilon_{d}}{k_1 k_2}$.  Take
$\varepsilon_w$ to Corollary~\ref{coll-blanket-balle-generic} on the
superwindows to find the amplified local privacy and then using strong
composition in Lemma~\ref{lemma-PrivacyFold2} we can easily derive the
Theorem~\ref{thm-FedPermDP3aa} for \Name with
$\mathcal{S}_{k_1}^{k_2}$.
%Theorem~\ref{thm-FedPermDP3aa} shows that \Name with $k_1$ as window
%size and $k_2$ as the number of shuffling patterns is
%$(\varepsilon_{\ell}, \delta_{\ell})$-DP.  This Theorem is the result
%of first applying Corollary~\ref{coll-blanket-balle-generic} on the
%superwidnows and then applying advanced composition on $k_2$
%components.

\begin{theorem}
For \Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{k_1}^{k_2} \circ
\mathcal{R}^{w}$ with window size $k_1$, and $k_2$ shuffling patterns,
where $\mathcal{R}^w$ is $\varepsilon_w$-LDP and $\varepsilon_{w} \leq
\log{( k_1 / \log{((k_2 +1)/\delta_{\ell})})}/2$, the amplified
privacy is $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w})
e^{\varepsilon_{w}} \log{(k_2/\delta_{\ell})} \sqrt{k_2/k_1})$.
\label{thm-FedPermDP3aa}
\end{theorem}


%\begin{corollary}
%For \Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{k_1}^{k_2} \circ \mathcal{R}^{w}$ with window size $k_1$, and $k_2$ shuffling patterns, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP, $\varepsilon_{w} = \varepsilon_{d} / (k_1 k_2)$ and $\varepsilon_{d} \leq (k_1 k_2) \cdot \log{( k_1 / \log{((k_2 +1)/\delta_{\ell})})}/2$, 
%the amplified privacy is 
%$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/(k_1 k2)) e^{(\varepsilon_{d}/(k_1 k2))} \log{(k_2/\delta_{\ell})} \sqrt{k_2/k_1})$. 
%\label{coll-FedPermDP3b}
%\end{corollary}







\begin{figure}[h!]
\centering
%\begin{subfigure}{.22\textwidth}
%\centering
%\includegraphics[width=.99\linewidth]{Images/fedperm_epsc_k1_B.png} 
%\caption{Impact of $k_1$ and $\varepsilon_{wd}$.}
%\label{fig:Priv1}
%\end{subfigure}
\begin{subfigure}{.22\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/fedperm_epsc_k1k2.png} 
\caption{Impace of $k_1$ and $k_2$,}
\label{fig:Priv2}
\end{subfigure}
\begin{subfigure}{.22\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/fedperm_epsc_d.png} 
\caption{Impact of $d$ and $\varepsilon_{wd}$.}
\label{fig:Priv3}
\end{subfigure}
\vspace{-0.1in}
\caption{Privacy amplification of \Name from $\varepsilon_d$-LDP to
  ($\varepsilon_{\ell},\delta_{\ell}$)-DP.  We illustrate the overal
  amplification with Bennett inequality for the Laplace
  Mechanism. 
%\vjm{Use bigger fonts for legends and X-/Y-axis
   % captions in all figures.}
}
\label{fig:Priv-ALL}
\end{figure}

\subsection{Privacy Analysis} 
In Figure~\ref{fig:Priv-ALL}, we show the relationship of our introduced varibales $k_1$, $k_2$, $\varepsilon_d$ and $d$ on the privacy amplification in \Name. 
Figure~\ref{fig:Priv2} shows the privacy amplification effect from $\varepsilon_{d}$-LDP to ($\varepsilon_{\ell},\delta_{\ell}$)-DP for the local model updates after shuffling with $k_2$ shuffling patterns each with size of $k_1$. 
%Figure~\ref{fig:Priv2} shows the amplification of privacy when we have different $k_1$ and $k_2$s.
We can see that each client can use larger shuffling patterns (i.e. , increasing $k_1$) or more shuffling patterns (i.e., increasing $k_2$) and get larger privacy amplification.
However, this comes with a price where this imposes more computation/communication burden on the clients to create the PIR queries as they need to encrypt $k_2 \times k_1^2$ values 
and send them to the server, and it also imposes higher computation on the server as it should multiply larger matrices.
Figure~\ref{fig:Priv3} shows the amplification of privacy for fixed value of $k_1=100, k_2=10$ for various model sizes. 
From this figure we can see that if we want to provide same privacy level for larger models, we need to increase values of $k_1$ or $k_2$ (i.e. more computation/communication cost).















%We know that $\varepsilon_{w} = \varepsilon_{d}/d$ so Corollary~\ref{coll-FedPermDP5} shows the privacy amplification based on $\varepsilon_{d}$.
%
%\begin{corollary}
%If $\mathcal{R}$ is $\varepsilon_{w}$-LDP, where $\varepsilon_{w} = \varepsilon_{d}/d$ and $\varepsilon_{d} \leq d \cdot \log{(d / \log{(1/\delta_{\ell})})}/2$,
%\Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{d} \circ \mathcal{R}$ satisfies $(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/d) e^{(\varepsilon_{d}/d)} \sqrt{\log{(1/\delta_{\ell})}/d})$.
%\label{coll-FedPermDP5}
%\end{corollary}



%\begin{table}[h!] 
%\caption{Measured time for different operations in \Name for different number of parameters when $n=15$}
%\begin{center}
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%$d$ & Enc (s) & AGR (s) & Dec(s)\\
%\hline
%
%50 & 1.02 & 17.61 & 0.02 \\
%\hline
%
%100 & 3.46 & 70.71 & 0.05 \\
%
%\hline
%200 & 22.48 & 350.16 & 0.80 \\
%
%\hline
%300 & 29.33 & 639.50 & 1.41 \\
%
%\hline
%400 & 52.19 & 1152.18 & 1.41 \\
%
%\hline
%500 & 81.72 & 1793.07 & 2.46 \\
%
%
%\hline
%\end{tabular}
%\label{tab:FedpermResult1}
%\end{center}
%\end{table}





















\iffalse
%\subsection{\Name with Recursion}

\subsection{Computation and Communication Costs of \Name}

\begin{table*}[h!]
\caption{Communication and Computation Cost of \Name}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{\textit{Algorithm}} & Client: Number of Encs & Upload BW & Server: AGR & Prob Random Guess\\
\hline
FL with Homomorphic Enc& $d$ & $O(d)$ & $O(n  d)$ & - \\
\hline
\Name & $d^2$ & $O(d^2)$ & $O(n  d^3)$ & $\frac{1}{d!}$ \\

\hline
\Name with $k_1$ as window size & $k_1  d$ & $O(k_1  d)$ & $O(n  k_1  d^2)$ & $\frac{1}{k_1!}$ \\

\hline
{\vtop{\hbox{\strut \Name with $k_1$ as window size}\hbox{\strut and $k_2$ shuffling patterns}}} & $k_2  k_1^2$ & $O(k_2  k_1^2)$ & $O(n  k_2  k_1^2  d )$ & ${\left(\frac{1}{k_1!}\right)}^{k_2}$\\

\hline
\Name with recursion $(k_3)$ & $d  k_3  \sqrt[k_3]{d}$& $O(d  k_3  \sqrt[k_3]{d})$& $O(n  k_3  \sqrt[k_3]{d}  d^2)$ & $\frac{1}{d!}$\\

\hline
{\vtop{\hbox{\strut \Name with $k_1$ as window size,}\hbox{\strut and recursion $(k_3)$}}} & $k_1  k_3  \sqrt[k_3]{k_1}$& $O(k_1  k_3  \sqrt[k_3]{k_1})$& $O(n  k_3  k_1  \sqrt[k_3]{k_1}  d)$ & $\frac{1}{k_1!}$ \\

\hline
{\vtop{\hbox{\strut \Name with $k_1$ as window size,}\hbox{\strut $k_2$ shuffling patterns and recursion $(k_3)$}}} & $k_2  k_3^2  \sqrt[k_3]{k_1^2}$& $O(k_2  k_3^2  \sqrt[k_3]{k_1^2})$& $O(n  k_2  k_3^2  \sqrt[k_3]{k_1^2}  d )$&${\left(\frac{1}{k_1!}\right)}^{k_2}$ \\


\hline
\end{tabular}
\label{tab1}
\end{center}
\end{table*}
\fi


==> test_dir/FedPerm/Exp.tex <==
\section{Experiments}
In this section, we investigate the utility and computation trade offs
in \Name.  We use MNIST dataset and a logistic regression model with
$d=7850$ parameters to evaluate these trade offs.




\subsection{Comparison with Baselines}
We compare our results with following baselines: \textbf{(a)}
FedAvg~\cite{mcmahan2017communication} with no privacy, \textbf{(b)}
CDP-FL~\cite{mcmahan2018learning, geyer2017differential}, \textbf{(c)}
LDP-FL~\cite{wang2019collecting, liu2020fedsel} with Gaussian
Mechanism.
%We run our experiments for 50 global rounds, and in each round we use
%$N=n=15$ clients.


\begin{figure}[h!]
\centering
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/Acc2.png} 
\caption{Final test accuracy.}
\label{fig:Acc1}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/acc3.png} 
\caption{Accuracy per FL round.}
\label{fig:Acc2}
\end{subfigure}
\vspace{-0.1in}
\caption{Test accuracy for different FL algorithms for MNIST over 15 clients.}
\label{fig:AccAll}
\end{figure}


Figure~\ref{fig:Acc1} shows the test accuracy of that model that was
trained using different FL algorithms running for $T=50$ rounds.  The
MNIST dataset is divided across $n=15$ clients with a Dirichlet
distribution.  Figure~\ref{fig:Acc2} shows the test accuracy for these
algorithms per FL round when the total privacy budget is fixed to
$\varepsilon=4.0$.  We compared two versions of \Name in these
experiments: \textbf{(a)} \Name with $k_1=400$ and $k_2=1$ which is a
``light'' version where encryption and decryption time at clients
takes around $52.2$ and $2.4$ seconds respectively.  It also imposes
$21$ minutes computation time at the server. \textbf{(b)} \Name with
$k_1=800$ and $k_2=10$ which is a ``heavy'' version where client
encryption, decryption, and server aggregation time takes around
$32.1$ minutes,  $2.4$ seconds and $16.4$ hours
respectively.

As we mentioned earlier, \Name provides a trade-off between privacy
amplification and compute resources -- larger the values of $k_1$ and
$k_2$, greater are the compute resources for training, which in turn
provides higher privacy amplification that results in better model
utility.  The heavy version of \Name needs more resources to be as
fast as the lighter version, but it can provide much more utility
(because the privacy amplification is larger so the amount of noise is
added is smaller).  For instance, after $T=50$, and total privacy
budget $(4.0, 1e^{-5})$, the heavy version provides $72.38\%$ test
accuracy while the light version provides $32.85\%$ test accuracy.
From these figures we can see if we invest enough computation
resources in \Name, we can provide higher utility compared to CDP-FL,
without trusting the \Name server.  Non-private FedAvg, CDP-FL and
LDP-FL also provides $91.02\%$, $53.50\%$, and $13.74\%$ test
accuracies for the same total $(\varepsilon, \delta)$ respectively.



\subsection{Time Analysis}
We evaluate the impacts of our hyperparameters $k_1$, $k_2$, $n$, and
$d$s on the encryption, decryption and sever aggregation time in
Figure~\ref{fig:Time-ALL}.  We use Paillier encryption system and we
use a key size of $2048$ bits in our experiments.  For measuring time,
we use 64CPUs and 64GB memory for the client and server simulations.
Note that we opt to not use GPU as model training is not a bottleneck
in our system compared to HE operations.  Also note that these figures
are data independent as we are working with encryption and decryption
and homomorphic multiplication with plaintext and homomorphic
addition.

\begin{figure}[h!]
\centering
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/time_k1_v2.png} 
\caption{Impact of $k_1$.}
\label{fig:Time1}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/time_k2_v2.png} 
\caption{Impact of $k_2$.}
\label{fig:Time2}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/time_d.png} 
\caption{Impact of $d$.}
\label{fig:Time3}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[width=.99\linewidth]{Images/time_n.png} 
\caption{Impact of $n$.}
\label{fig:Time4}
\end{subfigure}
\vspace{-0.1in}
\caption{Client encryption, decryption, and server aggregation time in \Name .}
\label{fig:Time-ALL}
\end{figure}


\paragraphb{Client encryption time:} In \Name, each client must do
$k_1^2 \cdot k_2$ encryptions for its query, therefore client
encryption time has a quadratic and linear relationship with window
size ($k_1$) and number of shuffling patterns ($k_2$) respectively
(Figures~\ref{fig:Time1} and~\ref{fig:Time2}). We also show in
Figure~\ref{fig:Priv-ALL} that increasing the $k_1$ has more impact
(close to quadratic impact) compared to increasing $k_2$ on the
privacy amplification. This means that if we invest more computation
resources on the clients and are able to do more encryption, we get
greater privacy amplification by parameter shuffling.  For instance,
when we increase the $k_1$ from $100$ to $200$ (while fixing $k_2=1$),
the average client encryption time increases from $3.4$ to $13.1$
seconds for $d=7850$ parameters.  And while fixing the $k_1=100$, if
we increase the number of shuffling patterns from $1$ to $10$, the
encryption time goes from $3.4$ to $32.7$ seconds.  When we fix the
value of $k_1$ and $k_2$, the number of encryption is fixed at the
clients, so the encryption time would be constant if we increase the
number of parameters ($d$) %or number of selected clients ($n$) in
each round (Figure~\ref{fig:Time3}).% and~\ref{fig:Time4}).


\paragraphb{Client decryption time:}
%As we mention in Section~\ref{sec:FedpermAdv}, based on the threat
%model, clients are fully decrypting or partially decrypting the
%parameters.
Changing $k_1$, $k_2$, and $n$ does not have any impact on decryption
time, as each client should decrypt $d$ parameters
(Figures~\ref{fig:Time1} and~\ref{fig:Time2}).  In
figure~\ref{fig:Time3}, we show the linear relationship of decryption
time and number of parameters.  For instance by increasing the number
of parameters from ${10}^5$ to ${10}^6$, the decryption time increases
from $1.01$ to $9.91$ seconds.


\paragraphb{Server aggregation time:} In \Name, the server first
multiplies the encrypted binary mask to the corresponding shuffled
model parameters for each client participating in the training round,
and then sums the encrypted unshuffled parameters to compute the
encrypted global model.  We employ joblib to parallelize matrix
multiplication over superwindows. Thus, larger the superwindows
greater is the parallelism. However, as we increase $k_1$ and/or $k_2$
the superwindow size goes down, and hence the parallelism, which leads
to increase in running time as observed in Figures~\ref{fig:Time1} and
~\ref{fig:Time2}.
\begin{comment}
\blue{We employ joblib to parallelize operations at the server.  We
  create $ d/(k_1 k_2)$ parallel matrix broadcasting of PIR queries
  ($k_2,k_1 n , k_1$) to reshaped shuffled parameters ($d/(k_1
  k_2),k_2, 1, k_1 n$) which results in encrypted global vector with
  $d=d/(k_1 k_2) \cdot k_1 \cdot k_2$ items.  This means that
  Increasing $k_1$ or $k_2$ reduces the number of parallel operations
  ($d/(k_1 k_2)$), so it results in getting less benefit from
  multiprocessing so the server time has a close to quadratic and
  linear relatioship with increasing $k_1$ and $k_2$ respectively
  (Figure~\ref{fig:Time1} and ~\ref{fig:Time2}).}
\end{comment}
Moreover, increasing $n$, $d$ has a linear relationship with server
aggregation time (Figure~\ref{fig:Time3} and~\ref{fig:Time4}).  For
instance, when we increase the $n$ from $5$ to $10$ the server
aggregation time increases from $157.47$ to $326.72$ seconds for
$d=7850$, $k_1=100$, and $k_2=1$.


%\blue{This aggregation involves of $n \cdot d/(k_1)$ matrix
%multiplications of matrices ($k_1 \times k_1$) to ($ k_1 \times 1$), and summing
%all the $n$ result vectors (each contains $d$ encrypted parameters).
%Increasing $k_1$ or $k_2$ reduces the number of parallel operations ($d/(k_1 k_2)$), so it results in  
%getting less benefit from multiprocessing so the server time has a close to quadratic and linear relatioship 
%with  increasing $k_1$ and $k_2$ respectively (Figure~\ref{fig:Time1} and ~\ref{fig:Time2}).}
%
%
%This means that increasing $k_1$ has a
%close to quadratic relationship with server aggregation time
%(Figure~\ref{fig:Time1}). 
%
%
%
%
%\blue{We employ joblib to parallel the operations at the server. 
%We create $ d/(k_1 k_2)$ parallel matrix braodcasting of PIR queries ($k_2,n\cdot k_1, k_1$) to reshaped shuffled 
%parameters ($k_2, 1, k_1 \cdot n$) which results in encrypted global vector with $d=d/(k_1 k_2) \cdot k_1 \cdot k_2$ items.
%This means that increasing $k_1$ has a
%close to quadratic relationship with server aggregation time
%(Figure~\ref{fig:Time1}). }
%\blue{This aggregation involves of $n \cdot d/(k_1 k_2) \cdot k_2$ matrix
%multiplications of matrices ($k_1 \times k_1$) to ($ k_1 \times 1$), and summing
%all the $n$ result vectors (each contains $d$ encrypted parameters).
%Increasing $k_2$ influences the number of parallel operations and when $d/(k_1 k_2)$ is smaller 
%we are getting less benefit of multiprocessing so the server time is inreasing by increasing $k_2$ (Figure~\ref{fig:Time2}).
%And increasing  $n$, $d$ has a
%linear relationship with server aggregation time
%(Figure~\ref{fig:Time3}and~\ref{fig:Time4}).  For
%instance, when we increase the $n$ from $5$ to $10$ the server
%aggregation time increases from $157.47$ to $326.72$ seconds for
%$d=7850$, $k_1=100$, and $k_2=1$.}
%\blue{This aggregation involves of $n$ matrix
%braodcasting (i.e.,  matrices ($k_2 \cdot k_1 \cdot k_1$) to ($d/(k_1 k_2) \cdot k_2 \cdot k_1 \cdot 1$)), and summing
%all the $n$ result vectors (each contains $d$ encrypted parameters).}
%\vjm{This sentence seems illegible, I don't follow
%  it. I think your are trying to say that unshuffling a superwindow
%  requires $k_2$ matrix multiplications (of $k1 \times k1$ matrices)
%  and $k_1 \cdot k_2 \cdot n$ additions are needed for the addition of
%  the $n$ clients' unshuffled parameters (for the superwindow)?
%  Please clarify/elaborate.}.  
%This means that increasing $k_1$ has a
%close to quadratic relationship with server aggregation time
%(Figure~\ref{fig:Time1}). 
%%and depends on the matrix multiplication
%%algorithm we use (naïve algorithm needs $O(n^3)$ time complexity, but
%%existing algorithms are faster).  
%And increasing $k_2$, $n$, $d$ has a
%linear relationship with server aggregation time
%(Figure~\ref{fig:Time2}, ~\ref{fig:Time3}and~\ref{fig:Time4}).  For
%instance, when we increase the $n$ from $5$ to $10$ the server
%aggregation time increases from $157.47$ to $326.72$ seconds for
%$d=7850$, $k_1=100$, and $k_2=1$.





%\subsection{Privacy Analysis}






%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/time_k1.png} 
%\caption{Client encryption, server multiplication, and decryption time for various window sizes $(k_1)$ in \Name.}
%\label{fig1}
%\end{figure}
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/time_k2.png} 
%\caption{Client encryption, server multiplication, and decryption time for various window sizes $(k_1)$ in \Name.}
%\label{fig1}
%\end{figure}

%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/acc1.png} 
%\caption{Accuracy of \Name for different privacy budgets.}
%\label{fig1}
%\end{figure}



%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/time_d.png} 
%\caption{\Name client encryption, server multiplication, and decryption time for various number of parameters ($d$) in each round.}
%\label{fig1}
%\end{figure}
%
%
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/time_n.png} 
%\caption{\Name Server processing time for different number of selected clients ($n$) in each round.}
%\label{fig1}
%\end{figure}




==> test_dir/FedPerm/FedPerm.tex <==
\section{\Name: Private and Robust Federated Learning by parameter
  Permutation}

We assume a dual threat model setting where (i) the federation server
acts as an \emph{honest but curious} aggregator, and (ii) the
federation clients can maliciously attempt to poison the trained model
using manipulated local parameter updates.
%by manipulating its local parameter updates before sending them to
%the server for aggregation.

\begin{comment}
\subsection{\Name Overview} 
Figure~\ref{fig:allDP}(d) depicts the \Name framework that consists of
three components, $\mathcal{F} = \mathcal{A} \circ \mathcal{S} \circ
\mathcal{R}^{d}$.  In \Name: \textbf{(1)} There are $N$ total clients
and $n$ clients are selected randomly in each round.  Each selected
client $i$ computes its local update $x_i \in \mathbb{R}^d$ and
applies a local randomizer $\mathcal{R}^d$ on it to produce $y_i \in
\mathbb{R}^d$.  \textbf{(2)} Now each client shuffles (i.e.,
$\mathcal{S}$) the parameters inside $y_i$ to produce $y_i^{\pi_i}$
where $\pi_i$ is a random shuffling pattern that the client $i$
produces for each round.  Note that the shuffling occurs inside the
clients and there is no need for a trusted shuffler outside the client
in \Name.  The client also creates an encrypted PIR query $c_i$. Then
the client sends $(y_i^{\pi_i}, c_i)$ to the server for aggregation.
\textbf{(3)} After collecting all the shuffled local updates, with
corresponding encrypted PIR query, from $n$ clients, the server
aggregates (i.e., $\mathcal{A}$) the local updates to produce the
global update for next round.  As this global aggregated update is
encrypted, so we propose different decryption methods relevant
different thread models discussed below.
\end{comment}


\subsection{FedPerm: Design}

\Name utilizes computational Private Information Retrieval
(cPIR)~\cite{chor1997computationally,stern1998new} for secure
aggregation at the federation server.  In particular, \Name\ uses the
cPIR algorithm by Chang~\cite{chang2004single} that leverages the
algorithm by Paillier~\cite{paillier1999public}.
Algorithm~\ref{alg:algorithm1} depicts \Name.
%Note that \Name is orthogonal to the specific cPIR scheme used, and
%can work with other cPIR techniques such as
%SealPIR~\cite{angel2018pir}.
%We present \Name as $\mathcal{F} = \mathcal{A} \circ \mathcal{S}
%\circ \mathcal{R}^{d}$ with three building processes: randomizing
%$\mathcal{R}^{d}$, shuffling and encoding $\mathcal{S}$, and
%analyzing $\mathcal{A}$.  We describe each component in this section.
Figure~\ref{fig:allDP}(d) depicts the \Name framework that consists of
three components, $\mathcal{F} = \mathcal{A} \circ \mathcal{S} \circ
\mathcal{R}^{d}$, denoting the client-side parameter randomizer
($\mathcal{R}^d$), the client-side shuffler ($\mathcal{S}$), and the
server-side aggregator ($\mathcal{A}$).

\paragraphb{Key Distribution} Paillier is a partial HE (PHE) algorithm
that relies on a public key encryption scheme (details of Paillier HE
in Appendix~\ref{sec:HE}).  Since Paillier is employed to protect
client updates from a curious federation server, \Name\ requires an
independent key server that generates a pair of public and secret
homomorphic keys $(Pk, Sk)$.  This key pair is distributed to all
federation clients, and just the public key $Pk$ is sent to the
federation server (for aggregation).  The key server itself can be
implemented as an independent third party server, or a leader among
the federation clients may be chosen to play that
role~\cite{zhang2020batchcrypt}.


\begin{algorithm}[h!]
\caption{\footnotesize \Name where \serverbox{green} and \clientbox{blue} colors show execution by server and client respectively.}
\label{alg:algorithm1}
{\scriptsize
\textbf{Input}: number of FL rounds $T$, number of local epochs $E$,
number of selected users in each round $n$, learning rate $\eta$,
local privacy budget $\varepsilon_d,$ number of model parameters $d$,
parameter update clipping threshold $C$\\
\textbf{Output}: $\theta_{g}^{T}$
\begin{algorithmic}[1] %[1] enables line numbers
\STATE \serverbox{$\theta_g^{0} \gets$ Initialize weights}
\FOR{each iteration $t \in [T]$}
\STATE \serverbox{$U \gets$ set of $n$ randomly selected clients out of $N$ total clients}
\FOR{$u$ in $U$}
\STATE \clientbox{$\theta_{u}^t \gets \textsc{LocalUpdate}(\theta_g^{t}, \eta, E)$}
\STATE \clientbox{$\bar{\theta}_{u}^t \gets \textsc{Clip}(\theta_{u}^t, -C, C )$}
\STATE \clientbox{$\tilde{\theta}_{u}^t \gets (\bar{\theta}_{u}^t + C)/ (2C)$ }
\STATE \clientbox{$y_{u}^{t} \gets \textsc{Randomize}(\tilde{\theta}_{u}^t, \varepsilon_d)$}
\STATE \clientbox{$\pi_u \gets $ Shuffling pattern $\textsc{RandomPermutations} \in [1,d]$ }
\STATE \clientbox{$\tilde{y}_{u}^{t} \gets \textsc{Shuffle}(y_{u}^{t}, \pi_u)$}
\STATE \clientbox{$b_{u}^{t} \gets \textsc{BinaryMask}(\pi_u)$}
\STATE \clientbox{$c_{u}^{t} \gets \textsc{Enc}_{pk}(b_{u}^{t} )$}
\STATE \clientbox{Client $u$ sends $(\tilde{y}_{u}^{t}, c_{u}^{t})$ to the server}
\ENDFOR
%\STATE \serverbox{Server checks the norm of updates $\tilde{y}_{u\in U}^{t}$}
\STATE \serverbox{norm bounding: $\tilde{y}_{u}^{t} \gets \tilde{y}_{u}^{t}\cdot \min(1, \frac{M}{{||\tilde{y}_{u}^{t}||}_2})$ for $u \in U$}
\STATE \serverbox{$\bar{z} \gets \frac{1}{n} \sum_{u \in U} \left( c_{u}^{t} \times \tilde{y}_{u}^{t} \right) $}
%\STATE \clientbox{\%Threat Model 1: Decryption happens on Clinets}
\STATE \clientbox{$z \gets \textsc{Dec}_{sk}(\bar{z})$}
\STATE \clientbox{normalize $z \gets C \cdot \left(2z - 1\right)$}
\STATE \clientbox{update model $\theta_g^{t+1} \gets \theta_g^{t} + z$}
%\STATE \serverbox{\%Threat Model 2: Decryption happens on Server}
%\STATE \serverbox{$D \gets$ pick t clients randomly for decryption of $\bar{z}$ }
%\STATE \serverbox{${P}_{u \in D} \gets Dec_{sk_{u \in D}}(\bar{z}) $}
%\STATE \serverbox{Validate partial decryptions $({P}_{u \in D} )$}
%\STATE \serverbox{$z \gets \textsc{Combine}({P}_{u \in D} )$}
%\STATE \serverbox{normalizes $z \gets C \cdot \left(2z - 1\right)$}
%\STATE \serverbox{updates model $\theta_g^{t+1} \gets \theta_g^{t} + z$}

\ENDFOR
\STATE \textbf{return} $\theta_g^{T}$
\end{algorithmic}
}
%\vjm{Perhaps use color coding to indicate what part of the pseudo code
  %is executed by the server}
\end{algorithm}

%\subsubsection{Clients: Computing Local Updates}

\paragraphb{Client Local Training:} In the $t^{th}$ round, the server
randomly samples $n$ clients among total $N$ clients.  Each sampled
client locally retrains a copy of the global model it receives from
the server ($\theta_g^{t}$), optimizing the model using its local data
and local learning rate $\eta$ (Algorithm~\ref{alg:algorithm1}, line
5).

\paragraphb{Randomizing Update Parameters:} After computing local
updates $\theta_u^t$, client $u$ clips the update using threshold $C$
and normalizes the parameters to the range $[0,1]$
(Algorithm~\ref{alg:algorithm1}, lines 6-7).  Now the client applies
the randomizer (i.e., $\mathcal{R}^d$) on its local parameters to make
them $(\varepsilon_d)$-differentially private
(Algorithm~\ref{alg:algorithm1}, line 8).  We use the Laplacian
Mechanism as a local randomizer with privacy budget $\varepsilon_d$.
%, but any generic randomizer can be applied in this step which does not
%affect our corollaries later.

\paragraphb{Shuffling:} After clipping and perturbing the local
update, each client shuffles the parameters $y_u^t$ using the random
shuffling pattern $\pi_u$
%of model parameter indices $\in [1,d]$
(Algorithm~\ref{alg:algorithm1}, lines 9-10).  Shuffling amplifies the
privacy budget $\varepsilon_d$, which we discuss in
Section~\ref{sec:FedpermAdv}.

\paragraphb{Generating PIR queries:} Now the client encodes the
shuffle indices $\pi_u$ using a PIR protocol.
%To do so, the client retrieves each parameter out of $d$ model
%parameters privately.
This process comprises two steps: first creating a binary mask of the
shuffled index, and then encrypting it using the public key of HE that
the client received in first step (Algorithm~\ref{alg:algorithm1} line
11-12).  Generally, a PIR client needs access to the $j^{th}$ record
privately from an untrusted PIR server that holds a dataset $\theta$
with $d$ records; i.e. the PIR server cannot know that the client
requested the $j^{th}$ record.  To do so, the PIR client creates a
unit vector (binary mask) $\Vec{b}_j$ of size $d$ where all the bits
are set to zero except the $j^{th}$ position being set to one:
\begin{equation}\label{eq:vecquery}
{\footnotesize
\Vec{b}_{j}=
\begin{bmatrix}
0 & 0 & \dots & 1 & \dots & 0 & 0\\
\end{bmatrix}
}
\end{equation}
If the PIR client does not care about privacy, it would send
$\Vec{b}_j$ to the PIR server, and the server would generate the
client's response by multiplying the binary mask into the database
matrix $\theta$ ($ \theta_{j} = \Vec{b}_{j} \times \theta $).  A PIR
technique allows the client to obtain this response without revealing
$\Vec{b}_j$ to the PIR server.  For example in~\cite{chang2004single},
the PIR client uses HE to encrypt $\Vec{b}_j$ element by element
before sending it to the PIR server.  During the data recovery phase,
the client extracts its target record by decrypting the component of
$\textsc{Enc}(\Vec{b}_j) \times \theta$.  Equation~\ref{eq:PIR11}
shows retrieving the $j^{th}$ record by this PIR query.  Note that a
HE system has a property that $m_1 \times m_2 \gets \textsc{Dec}
\left( \textsc{Enc}[m_1] \times m_2 \right)$.
%\vspace{-0.1in}
\begin{equation}~\label{eq:PIR11}
{\footnotesize
\begin{aligned}
&\textsc{Dec} ( \textsc{Enc}(\Vec{b}_j) \times \theta )= \\
&\textsc{Dec} \left( \textsc{Enc}[0] \cdot \theta_1 + \dots + \textsc{Enc}[1] \cdot \theta_j + \dots + \textsc{Enc}[0] \cdot \theta_d \right) =\\
&\textsc{Dec} \left( \textsc{Enc}[\theta_j] \right) = \theta_j
\end{aligned}
}
\end{equation}
%\vspace{-0.1in}
A \Name client creates $d$ PIR queries to retrieve each parameter
privately.  (In Section~\ref{sec:FedpermAdv}, we discuss additional
parameters to reduce the number of PIR queries.)  In this case, the
shuffled parameters ($\tilde{y}_{u}^{t}$) are the dataset located at
the PIR server and each shuffled index in $\pi_u$ is the secret record
row number (i.e. $j^{th}$ in above) that the PIR client is interested
in.  Client $u$ first creates $b_u^t$ which is a collection of $d$
binary masks of shuffled indices in $\pi_u$, similar to PIR query
$\Vec{b}_j$ in Equation~\ref{eq:vecquery}.  Then the client encrypts
the binary masks and sends the shuffled parameters and the PIR query
(encrypted binary masks) to the server for aggregation.

\paragraphb{Correctness:} Note that for every client $u$ and every round
$t$, decrypting the multiplication of the encrypted binary masks to
the shuffled parameters produces the original unshuffled parameters.
It means that for $y_u^t = \textsc{Dec} \left( c_{u}^{t} \times
\tilde{y}_{u}^{t} \right)$. So for any $( \tilde{y},c, )$ we have:
\begin{equation}\label{eq:PIRcorrect1}
{\footnotesize
\begin{aligned}
&\textsc{Dec} \left( c \times \tilde{y} \right)= \\
&\textsc{Dec} \left(
\begin{bmatrix}
\textsc{Enc}(\Vec{b}_{\pi_1}) \\ \textsc{Enc}(\Vec{b}_{\pi_2}) \\ \dots \\ \textsc{Enc}(\Vec{b}_{\pi_d}) \\
\end{bmatrix} \times 
\begin{bmatrix}
\tilde{y}_1 \\ \tilde{y}_2 \\ \dots \\ \tilde{y}_d \\
\end{bmatrix} 
\right) =\\
&\textsc{Dec} \left(
\begin{bmatrix}
\textsc{Enc}[0] & \dots & \textsc{Enc}[1] & \dots & \textsc{Enc}[0] \\ 
\textsc{Enc}[0] & \dots & \textsc{Enc}[1] & \dots & \textsc{Enc}[0] \\ 
\dots & \dots & \dots & \dots & \dots\\ 
\textsc{Enc}[0] & \dots & \textsc{Enc}[1] & \dots & \textsc{Enc}[0] \\
\end{bmatrix} \times 
\begin{bmatrix}
y_1^{\pi} \\ y_2^{\pi} \\ \dots \\ y_d^{\pi} \\ 
\end{bmatrix}
\right) =\\
&\textsc{Dec} \left(\begin{bmatrix}
\textsc{Enc}[y_1] & \textsc{Enc}[y_2] & \dots & \textsc{Enc}[y_d] \\
\end{bmatrix} \right) = \\
& \begin{bmatrix}
y_1 & y_2 & \dots & y_d \\
\end{bmatrix}
\end{aligned}
}
\end{equation}

\paragraphb{Server: norm bounding}
After collecting all the local updates $(\tilde{y}_{u}^{t},
c_{u}^{t})$ for selected clients in round $t$, the \Name server first
applies $\ell_2$-norm bounding to the threshold $M$ on the shuffled
parameters $\tilde{y}_{u}^{t}$ (Algorithm~\ref{alg:algorithm1}, line
15).  Note that unlike other robust AGRs, \emph{norm bounding} is the
only robust AGR scheme that does not require the true position of the
parameters because it works by calculating the $\ell_2$ norm of the
parameter updates as a whole irrespective of their order
(i.e. $\ell_2(\tilde{y}_{u}^{t}) = \ell_2(y_{u}^{t})$).  Prior
works~\cite{nguyen2021flame,naseri2020local,sun2019can} have shown the
effectiveness of norm bounding in defense against poisoning attacks by
malicious clients.
%~\vjm{The pseudo code
%  lines 15-16 does not show the server dropping off the updates whose
%  norms are higher.  Also, I thought that the server could force the
%  norm to its threshold by clipping it.  Whatever it is we are doing,
%  we should make it explicit in the pseudo code and description.}.

\paragraphb{Server: Aggregation}
Then the server aggregates all the updates into global update
$\bar{z}$ (Algorithm~\ref{alg:algorithm1}, line 16).  This aggregation
is averaging the update parameters for $n$ collected updates by
calculating $\frac{1}{n} \sum_{u \in U} \left( c_{u}^{t} \times
\tilde{y}_{u}^{t} \right)$.  The expression $c_{u}^{t} \times
\tilde{y}_{u}^{t}$ has the effect of ``unshuffling'' client $u$'s
parameters.  At the same time, the resulting vector is encrypted, thus
kept hidden from the server.
\begin{comment}
Figure~\ref{fig:AGRE} shows the \Name
aggregation where \Name server is averaging the shuffled parameters
without knowing the true position of each parameter as their indices
are encrypted.
\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{Images/FedpermAGRprocess.pdf} 
\caption{\Name aggregation. The superscript $j$ of all the
  $\theta_i^j$s refers to the original index of the parameter; $i$ is
  the $i^{th}$ client participating in the training round.~\vjm{If we
    are in a space crunch, we can eliminate this figure; its is quite
    nice, but is not crucial to help readers understand the
    aggregation algorithm.}}
\label{fig:AGRE}
\end{figure}
\end{comment}

\paragraphb{Correctness of Aggregation:} In
Equation~\ref{eq:PIRcorrect1}, we show that $\forall t \in [T], u \in
U \;\; y_u^t = \textsc{Dec} \left( c_{u}^{t} \times \tilde{y}_{u}^{t}
\right)$.  
Based on the two main properties of a HE system 
\textbf{(a)} $m_1 \times m_2 \gets \textsc{Dec} \left( \textsc{Enc}[m_1] \times m_2 \right)$, 
\textbf{(b)} $m_1 + m_2 \gets \textsc{Dec} \left( \textsc{Enc}[m_1] + \textsc{Enc}[m_2] \right)$, and 
Equation~\ref{eq:PIRcorrect1}, we can derive the Equation~\ref{eq:PIRcorrect3}:
%

%~\vjm{This is not all that
  %obvious.  Perhaps refer to Paillier's property of additive
 % homomorphism to reach to this conclusion}:
\begin{equation}\label{eq:PIRcorrect3}
{\footnotesize
  \textsc{Dec} \left( \frac{1}{n} \sum_{u \in U} ( c_{u}^{t} \times \tilde{y}_{u}^{t}) \right)=\frac{1}{n} \sum_{u \in U} y_u^t
}
\end{equation}


\paragraphb{Updating Global Model} The server aggregates local updates
$(\tilde{y}_{u}^{t}, c_{u}^{t})$ without knowing the true position of
the parameters as they are detached from their positions.  Result of
aggregation $\frac{1}{n} \sum_{u \in U} \left( c_{u}^{t} \times
\tilde{y}_{u}^{t} \right)$ is vector of encrypted parameters, and they
need to be decrypted to be used for updating the global model
(Algorithm~\ref{alg:algorithm1} lines 17-19).  This decryption is done
at each client using Paillier's secret key.
%As we mentioned in Section~\ref{Sec:TM}, there are two decryption
%scenarios: \textbf{(1)} For honest-but-curious aggregator threat
%model, the decryption happens at the clients, and each client will
%update the global model locally \textbf{(2)} For curious and colluding
%participants threat model, the partial decryption happens at the
%selected $t$ clients and the server combines the partial decryptions
%to find unencrypted global update, and then announces it to the
%clients for next round training.









==> test_dir/FedPerm/FedPermDP.tex <==





\section{Privacy Guarantees by Shuffling Parameters}

\subsection{\Name}
In \Name, each client randomizes each value in its updates with randomizer $\mathcal{R}$ and then shuffle all the $d$ values (i.e., parameters in the local update) that each value is $\varepsilon_{w}$-LDP.
From Corollary~\ref{coll-blanket-balle-generic}, we can show Corollary~\ref{coll-FedPermDP1}. 
The intuition is that we map the clients in Corollary~\ref{coll-blanket-balle-generic} to parameters in Corollary~\ref{coll-FedPermDP1}. 
This means in \Name, the number of clients participating in shuffling ($n$) will be replaced by number of parameters ($d$).


\begin{corollary}
If $\mathcal{R}$ is $\varepsilon_{w}$-LDP, where $\varepsilon_{w} \leq \log{(d / \log{(1/\delta_{\ell})})}/2$,
\Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{d} \circ \mathcal{R}$ satisfies $(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w}) e^{\varepsilon_{w}} \sqrt{\log{(1/\delta_{\ell})}/d})$.
\label{coll-FedPermDP1}
\end{corollary}

We know that $\varepsilon_{w} = \varepsilon_{d}/d$ so Corollary~\ref{coll-FedPermDP5} shows the privacy amplification based on $\varepsilon_{d}$.

\begin{corollary}
If $\mathcal{R}$ is $\varepsilon_{w}$-LDP, where $\varepsilon_{w} = \varepsilon_{d}/d$ and $\varepsilon_{d} \leq d \cdot \log{(d / \log{(1/\delta_{\ell})})}/2$,
\Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{d} \circ \mathcal{R}$ satisfies $(\varepsilon_{\ell}, \delta_{\ell})$-DP with $\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/d) e^{(\varepsilon_{d}/d)} \sqrt{\log{(1/\delta_{\ell})}/d})$.
\label{coll-FedPermDP5}
\end{corollary}










%-------------------------------------------------------------Fedperm with k1--------------------------------------------

\subsection{\Name with Window Size $k_1$}


\paragraphb{Superwindow}: If we have $w=d/k_1$ windows, then each window has $k_1$ parameters. If we look at the update $\theta$ with $d$ parameters as $\mathbb{R}^{k_1 \times w}$ (a matrix with $k_1$
rows and $w$ columns), each column is a window and each row is a superwindow. For example, for above example, each row of matrix $\theta$ is a superwindow. 
This means that in \Name, we have $k_1$ superwindows and each super window has $w=d/k_1$ elements. 

Now, since the shuffling is applied on the superwindows, then we need to make each superwindow $\varepsilon_w$-LDP using a randomizer $\mathcal{R}^w$.
Theorem~\ref{thm-FedPermDP2a} shows that \Name with $k_1$ as window size is $(\varepsilon_{\ell}, \delta_{\ell})$-DP. 

\begin{theorem}
For \Name $\mathcal{F}=\mathcal{A}  \circ \mathcal{S}_{k_1} \circ \mathcal{R}^{w}$ with window size $k_1$, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP and $\varepsilon_{w} \leq \log{(k_1 / \log{(1/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w}) e^{\varepsilon_{w}} \sqrt{\log{(1/\delta_{\ell})}/k_1}$. 
\label{thm-FedPermDP2a}
\end{theorem}

\begin{corollary}
For \Name $\mathcal{F}=\mathcal{A}  \circ \mathcal{S}_{k_1} \circ \mathcal{R}^{w}$ with window size $k_1$, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP, $\varepsilon_{w} = \varepsilon_{d}/k_1$ and $\varepsilon_{d} \leq k_1 \cdot \log{(k_1 / \log{(1/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/k_1) e^{(\varepsilon_{d}/k_1)} \sqrt{\log{(1/\delta_{\ell})}/k_1}$. 
\label{thm-FedPermDP2b}
\end{corollary}





This Theorem is the result of applying Corollary~\ref{coll-blanket-balle-generic} on the superwidnows.


%\begin{figure}[t]
%\centering
%\includegraphics[width=0.9\columnwidth]{Images/fedperm_epsc_k1_B.png} 
%\caption{Effect of $k_1$ and $\varepsilon_{wd}$ on the central privacy budget. We illustrate the overal amplification with Bennett inequality for the Laplace Mechanism.}
%\label{fig1}
%\end{figure}







%-------------------------------------------------------------Fedperm with k1 and k2--------------------------------------------
\subsection{\Name with Window Size $k_1$ and $k_2$ Patterns}


When we have $k_2$ patterns, it is like running \Name for $k_2$ times with $k_1$ users 
participating in FL that each one have a local update with $w=d/(k_1 k_2)$ parameters.
In this case, the size of each super window is $w=d/(k_1 k_2)$.
Therefore, each client needs to apply a randomizer $\mathcal{R}^w$ with $\varepsilon_{w}$ on its superwindows.

Theorem~\ref{thm-FedPermDP3a} shows that \Name with $k_1$ as window size and $k_2$ as the number of different shuffling patterns is $(\varepsilon_{\ell}, \delta_{\ell})$-DP. 


\begin{theorem}
For \Name $\mathcal{F}=\mathcal{A} \circ \mathcal{S}_{k_1}^{k_2} \circ \mathcal{R}^{w}$ with window size $k_1$, and $k_2$ shuffling patterns, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP and $\varepsilon_{w} \leq \log{( k_1 / \log{((k_2 +1)/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{w}) e^{\varepsilon_{w}} \log{(k_2/\delta_{\ell})} \sqrt{k_2/k_1})$. 
\label{thm-FedPermDP3a}
\end{theorem}


\begin{corollary}
For \Name $\mathcal{F}=\mathcal{A}  \circ \mathcal{S}_{k_1}^{k_2} \circ \mathcal{R}^{w}$ with window size $k_1$, and $k_2$ shuffling patterns, where $\mathcal{R}^w$ is $\varepsilon_w$-LDP, $\varepsilon_{w} = \varepsilon_{d} / (k_1 k_2)$ and $\varepsilon_{d} \leq (k_1 k_2) \cdot \log{( k_1 / \log{((k_2 +1)/\delta_{\ell})})}/2$, 
the amplified privacy is 
$\varepsilon_{\ell}=O( (1 \wedge \varepsilon_{d}/(k_1 k2)) e^{(\varepsilon_{d}/(k_1 k2))} \log{(k_2/\delta_{\ell})} \sqrt{k_2/k_1})$. 
\label{coll-FedPermDP3b}
\end{corollary}




This Theorem is the result of first applying Corollary~\ref{coll-blanket-balle-generic} on the superwidnows and then applying advanced composition on $k_2$ components. 


\begin{figure}[h!]
\centering
\begin{subfigure}{.22\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{Images/fedperm_epsc_k1_B.png}  
    \caption{Impact of $k_1$ and $\varepsilon_{wd}$.}
    \label{fig:Priv1}
\end{subfigure}
\begin{subfigure}{.22\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{Images/fedperm_epsc_k1k2.png}  
    \caption{Imapct of $k_1$ and $k_2$,}
    \label{fig:Priv2}
\end{subfigure}
\begin{subfigure}{.22\textwidth}
    \centering
    \includegraphics[width=.99\linewidth]{Images/fedperm_epsc_d.png}  
    \caption{Impact of $d$ and $\varepsilon_{wd}$.}
    \label{fig:Priv3}
\end{subfigure}
\caption{We illustrate the overal amplification with Bennett inequality for the Laplace Mechanism.}
\label{fig:Priv-ALL}
\end{figure}

\paragraphb{Privacy Analysis} In Figure~\ref{fig:Priv-ALL},  we show the relationship of our introduced varibales $k_1$, $k_2$, $\varepsilon_w$ and $\varepsilon_{wd}$ on the privacy amplifiction in \Name. 
Figure~\ref{fig:Priv1} shows the relationship of 
Figure~\ref{fig:Priv2}
Figure~\ref{fig:Priv3}




\subsection{Privacy Gurantee for T rounds}
We are doing Fedperm for a sequence of T adaptive $\mathcal{F}_1,\dots, \mathcal{F}_T$ where each $\mathcal{F}_t$ for $t \in [T]$ staitisifes the privacy gurantees stated in Theroemes~\ref{} dends on using pure \Name,  or $k_1$ or $k_2$.
Now we invoke the strong compositing stated in Lemma~\ref{} to obtain the pruvacy gurantee of the \Name for $T$ rounds.  We can conlude that for any $\delta'>0$,  \Name is $(\varepsilon, \delta)$-DP for 
\begin{equation}
	\varepsilon = \sqrt{2T\log{(1/\delta')}} \varepsilon_{\ell} + T \varepsilon_{\ell} (e^{\varepsilon_{\ell}}-1),  \delta=T \delta_{\ell}+ \delta'
\end{equation}



































==> test_dir/FedPerm/FedPerm_TM.tex <==
\section{\Name: Private Federated Learning by parameter Permutation}

\begin{comment}
FL involves mutually untrusting clients.  Hence, a \emph{poisoning
  adversary} may own or compromise some of the FL clients, called
\emph{malicious clients}, with the goal of mounting a \emph{targeted}
or \emph{untargeted} poisoning attack.  In a targeted
attack~\cite{bhagoji2019analyzing, sun2019can}, the goal is to reduce
the utility of the model on specific test inputs, while in the
untargeted attack~\cite{baruch2019a,
  fang2020local,shejwalkar2021manipulating}, the goal is to reduce the
utility for all (or most) test inputs. It is
shown~\cite{blanchard2017machine} that even a single malicious client
can mount an effective untargeted attack on FedAvg.

Using secure aggregation makes it very easy for the poisoning
adversary to craft very large updates and destroy the global model
without being detected.  In order to make FL robust to the presence of
such malicious clients, the literature has designed various
\emph{robust aggregation rules (AGR)}~\cite{blanchard2017machine,
  mozaffari2021fsl, YinCRB18,chang2019cronus}, which aim to remove or
attenuate the updates that are more likely to be malicious according
to some criterion.  Unfortunately, these robust AGRs are not usable in
an FL with secure aggregation because the parameters are encrypted or
secrete shared.  On the other hand, it has been
shown~\cite{naseri2020local,sun2019can} that LDP-FL can defend against
targeted and untargeted attacks as the model updates are bounded.

In this work, we present \Name, a novel approach to perform FL while
concurrently achieving two goals of privacy and robustness.  \Name
provides higher utility compared to LDP-FL as each client is shuffling
the parameters, so the privacy is amplified (i.e. less noise is
required for the same level of LDP).  In this section, we describe our
algorithm overview and clarify different threat models we consider in
this paper.
\end{comment}
\vjm{Removed 3 paras from here since they seem redundant.}
We now overview \Name\ and decsribe different threat models we
consider in our work.

\subsection{\Name Overview} 
Figure~\ref{fig:allDP}(d) depicts the \Name framework that consists of
three components, $\mathcal{F} = \mathcal{A} \circ \mathcal{S} \circ
\mathcal{R}^{d}$.
In \Name:
\textbf{(1)} There are $N$ total clients and $n$ clients are selected
randomly in each round.  Each selected client $i$ computes its local
update $x_i \in \mathbb{R}^d$ and applies a local
randomizer $\mathcal{R}^d$ on it to produce $y_i \in \mathbb{R}^d$.
\textbf{(2)} Now each client shuffles (i.e., $\mathcal{S}$) the
parameters inside $y_i$ to produce $y_i^{\pi_i}$ where $\pi_i$ is a
random shuffling pattern that the client $i$ produces for each
round.  Note that the shuffling occurs inside the clients and
there is no need for a trusted shuffler outside the client in \Name.
The client also creates an encrypted PIR query $c_i$. Then
the client sends $(y_i^{\pi_i}, c_i)$ to the server for aggregation.
\textbf{(3)} After collecting all the shuffled local updates, with
corresponding encrypted PIR query, from $n$ clients, the server
aggregates (i.e., $\mathcal{A}$) the local updates to produce the
global update for next round.  As this global aggregated update is
encrypted, so we propose different decryption methods relevant
different thread models discussed below.




==> test_dir/FedPerm/app.tex <==

%\section{Differential Privacy in FL Algorithms}

\begin{figure}[h]
\centering
\includegraphics[width=0.9\columnwidth]{Images/Fedperm2_TM.pdf} 
\caption{Different threat models.}
\label{fig:TM}
\end{figure}


\section{Threat Models}\label{Sec:TM}
In this section, we describe two threat models that are of interest to
our work, and illustrated in Figure~\ref{fig:TM}.

\subsection{Honest-but-Curious Aggregator}
In this threat model, we assume that the server correctly follows the
aggregation algorithm, but may try to learn clients' private
information by inspecting the model updates sent by the
participants. This is a common assumption that previous
works~\cite{zhang2020batchcrypt, xu2019hybridalpha,
  bonawitz2017practical, truex2019hybrid} also consider.  For creating
the PIR queries, we use Paillier~\cite{paillier1999public} homomorphic
encryption. We explain different homomorphic encryption systems that
we use in Appendix~\ref{sec:HE}.  Before starting \Name, we need a key
server to generate and distribute the keys for the homomorphic
encryption (HE).  A key server generates a pair of public and secret
homomorphic keys $(Pk, Sk)$, sends them to the clients, and sends only
the public key to the server.  Either a trusted external key server or
a leader client can be responsible for this role.  For the leader
client, similar to previous works~\cite{zhang2020batchcrypt}, before
the training starts, the FL server randomly selects a client as the
leader.  The leader client then generates the keys and distributes
them to the clients and the server as above.
%This key server role can be In this threat model for distributing the
%keys for the homomorphic encryption (HE), we can have one of the
%followings: \begin{itemize} \item \emph{External Key Server:} A
%trusted external key server generates a pair of public and private
%homomorphic keys $(Pk, Sk)$, sends them the clients, and sends only
%the public key to the server.  \item \emph{Leader client:} Similar to
%previous works~\cite{zhang2020batchcrypt}, before the training
%starts, the FL server randomly selects a client as the leader who
%generates the keys and distribute them among the clients and the
%server.  \end{itemize}

The steps of \Name for this threat model (Figure~\ref{fig:TM}(a)) are
as follows:
\textbf{(1)} The pair of keys are distributed by the key server to all
the clients.
\textbf{(2)} In each round of training, the clients learn their local
updates, generate encrypted PIR query and shuffled parameters, and
send them to the server.  Next, the server aggregates the updates, and
sends the aggregated update to the clients.
\textbf{(3)} Each client can decrypt the encrypted global parameters
received from the server using the private key and updates its model.


\subsection{Curious and Colluding Clients}
In this threat model, we assume that some clients may collude with the
FL server to get private information about a victim client by
inspecting its model update.  For this threat model, we use
thresholded Paillier~\cite{damgaard2001generalisation}.  In the
thresholded Paillier scheme, the secret key is divided to multiple
shares, and each share is given to a different client.  For this
threat model, we need an external key server that generates the keys
and sends $(Pk, Sk_i)$ to each client, and sends the public key to the
server.  Now each client can partially decrypt an encrypted
message, but if less than a threshold, say $t$, combine their partial
decrypted values, they cannot get any information about the real
message.  On the other hand, if we combine $\geq t$ partial decrypted
values, we can recover the secret.  We explain how thresholeded
Paillier scheme works in Appendix~\ref{sec:HE}.

The steps of \Name for this threat model (Figure~\ref{fig:TM}(b)) are
as follows:
\textbf{(1)} The pairs of keys are distributed to the clients by the
key server.
\textbf{(2)} In each round of training, the clients learn their local
updates,generate encrypted PIR query and shuffled parameters, and send
them to the server.  Next, the server aggregates the local updates to
produce global model update (which is encrypted).
\textbf{(3)} The server randomly chooses $t$ clients to partially
decrypt the global model update. The \Name server sends the encrypted
global update to these clients.
\textbf{(4)} Each client decrypts the global model with its specific
partial secret key $Sk_i$, and sends the result back to the server.
\textbf{(5)} The server first authenticates each partial decryption
that is done by the true $Sk_i$ (by a zero-knowledge proof provided by
thresholded Paillier~\cite{damgaard2001generalisation}).  Then the
\Name server combines the partial decrypted updates and broadcasts
plain unshuffled model updates to all the clients for the next round
of \Name.

At present our implementation of \Name does not support this threat
model, and we leave it for future work.

\section{Central Differential Privacy in FL (CDP-FL)}
Algorithm~\ref{alg:CDP-FL} shows how CDP-FL works which is also
discussed in ~\cite{mcmahan2018learning, geyer2017differential,
  naseri2020local}.  In CDP-FL, the server receives model updates
capped by norm $C$, and after averaging them, it adds i.i.d sampled
noise to the parameters $\theta_g^{t+1} \gets \theta_g^{t} +
\frac{1}{n} \sum_{u \in U} \theta_u^{t} + \mathcal{N} (0, \sigma^2
\mathbb{I})$ where $\sigma \gets \frac{\Delta_2}{\varepsilon} \sqrt{2
  ln(1.25) / \delta }$ and the $\ell_2$ sensitivity is $\Delta_2=C$.

\begin{algorithm}[h!]
\caption{Central Differential Privacy in FL (CDP-FL)}
\label{alg:CDP-FL}
\textbf{Input}: number of FL rounds $T$, number of local epochs $E$,
number of all the clients $N$, number of selected users in each round
$n$, total privacy budget $TP$, probability of subsampling clients
$q$, learning rate $\eta$, noise scale $z$, bound $C$
\\ \textbf{Output}: global model $\theta_{g}^{T}$
\begin{algorithmic}[1] %[1] enables line numbers
\STATE  $\theta_g^{0}  \gets$ Initialize weights
\STATE Initialize MomentAccountant$(\varepsilon,  \delta,  N)$

\FOR{each iteration $t \in [T]$}
	\STATE $U \gets$ set of $n$ randomly selected clients out of $N$ total clients with probability of $q$
	\STATE $p_t \gets $ MomentAccountant.getPrivacySpent()  \COMMENT{\% privacy budget spent till this round}
	\IF{$p_t > TP$} 
		\STATE \textbf{return} $\theta_g^{T}$ \COMMENT{\% if spent privacy budget is passed over the threshold finish FL training}
	\ENDIF
    	\FOR{$u$ in $U$}
		\STATE $\theta \gets \theta_g^{t}$
		\FOR{local eopoch $e \in [E]$}
			\FOR{batch $b \in [B]$}
				\STATE $\theta \gets \theta - \eta \triangledown L(\theta,  b)$ 
				\STATE $\triangle \gets \theta - \theta_g^{t}$
				\STATE $\theta \gets \theta_{g}^{t} + \triangle \min{(1,  \frac{C}{{||\triangle||}_2})}$
			\ENDFOR
		\ENDFOR
		\STATE Client $u$ sends $\theta_{u}^{t}=\theta-\theta_{g}^{t}$ to the server
	\ENDFOR
	\STATE $\sigma \gets z C/q$
	\STATE  $\theta_g^{t+1} \gets \theta_g^{t} +  \frac{1}{n} \sum_{u \in U} \theta_u^{t} + \mathcal{N} (0,  \sigma^2 \mathbb{I}) $
	\STATE MomentAccountant.accumulateSpentBudget$(z)$
\ENDFOR
\STATE \textbf{return} $\theta_g^{T}$
\end{algorithmic}
\end{algorithm}






%\subsection{Local Differential Privacy in FL}
%In this setting,  each client utilizes differentialy private stochastic gradient descent (DP-SGD)~\cite{abadi2016deep} to train a private model on top of its data.  
%Algorithm~\ref{alg:LDP-FL} shows how DP-SGD in local differentaially private FL works.
%
%Please note that in a mini-batch,  the gradient for each data item is computed and clipped speprtedly to limit the sensitivity of each data item on the output of loss function's gradient.


%\begin{algorithm}[h!]
%\caption{Local Differential Privacy in FL (LDP-FL)}
%\label{alg:LDP-FL}
%\textbf{Input}:  number of FL rounds $T$, number of local epochs $E$,  number of all the clients $N$,  number of selected users in each round $n$,  sampling probability $p$,  
%learning rate $\eta$,  noise scale $z$,  bound $C$ \\
%\textbf{Output}: global model $\theta_{g}^{T}$
%\begin{algorithmic}[1] %[1] enables line numbers
%\STATE  $\theta_g^{0}  \gets$ Initialize weights
%
%\FOR{each iteration $t \in [T]$}
%	\STATE $U \gets$ set of $n$ randomly selected clients out of $N$ total clients
%    	\FOR{$u$ in $U$}
%		\STATE $\theta_0 \gets \theta_g^{t}$
%		\FOR{local eopoch $e \in [E]$}
%			\FOR{$(x,y) \in $ random batch from training dataset wtih probability $p$}
%				\STATE $g_e (x_i) \gets  \triangledown_{\theta_e} L(\theta_e, (x_i,y_i))$ 
%			\ENDFOR
%			\STATE $\bar{g}_e (x_i) \gets g_e (x_i) \min{(1,  \frac{C}{{||g_e (x_i)||}_2})}$
%			\STATE ${\tilde{g}}_e \gets \frac{1}{pD} \left( \sum_{i \in batch} \bar{g}_e (x_i) +  \mathcal{N} (0,  C^2 \sigma^2 \mathbb{I}) \right)$ 
%			\STATE $\theta_{e+1} \gets \theta_e - \eta {\tilde{g}}_e$
%	\ENDFOR
%	\STATE Client $u$ sends $\theta_{u}^{t}=\theta_{E}$ to the server
%	\ENDFOR
%	\STATE updates model $\theta_g^{t+1} \gets \frac{1}{n} \sum_{u \in U} \theta_{u}^{t}$
%	\ENDFOR
%\STATE \textbf{return} $\theta_g^{T}$
%\end{algorithmic}
%\end{algorithm}





%\subsection{Client Shuffling Differential Privacy in FL}









%/section{Privacy Backgrounds}

\section{Laplace Mechanism}~\label{sec:Laplace}
The most common mechanism for achieving pure $\varepsilon_{\ell}$-DP
is Laplace mechanism~\cite{}, where

\begin{definition}
Let $f: \mathcal{X}^n \rightarrow \mathbb{R}^{k}$.  The
$\ell_1$-sensitivity of $f$ is:
\begin{equation}
\Delta_1^{(f)} = \max_{X, X'} {|| f(X) - f(X')||}_1
\end{equation}
where $X, X' \in \mathcal{X}^n$ are neighbering datasets differing
from each other by a single data record.
\end{definition}

Sensitivity gives an upper bound on how much the output of the
randomizer can change by switching over to a neighboring dataset as
the input.

\begin{definition}
Let $f: \mathcal{X}^n \rightarrow \mathbb{R}^{k}$. The Laplace
mechanism is defined as:
\begin{equation}
\mathcal{R} (X) = f(X) + [Y_1,  \dots, Y_k]
\end{equation}
Where the $Y_i$s are drawn i.i.d from
Laplace$(\Delta^{(f)}/\varepsilon)$ random variable.  This
distribution has density of
$p(x)=\frac{1}{2b}\exp{\left(-\frac{|x|}{b} \right)}$ where $b$ is the
scale and equal to $\Delta^{(f)}/\varepsilon$.
\end{definition}

In \Name, each client $i$ applies the Laplace mechanism as a
randomizer $\mathcal{R}$ on its local model update $(x_i)$.  Each
model update contains $d$ parameters in range of $[0,1]$, so the
sensitivity of the entire input vector is $d$.  It means that applying
$\varepsilon_d$-DP on the vector $x_i$ is equal to applying
$\varepsilon_{wd}=\varepsilon_{d}/d$ on each parameter independently.
Therefore, applying $\varepsilon_d$-DP randomizer $\mathcal{R}$ on the
vector $x_i$ means adding noise from Laplace distribution with scale
$b=\frac{1}{\varepsilon_{wd}}=\frac{1}{\frac{\varepsilon_d}{d}}=\frac{d}{\varepsilon_d}$.

%The major strength of the Gaussan mechanims is that it draw noise from normal distribution with L2 sensitivity and in which L2 sensitivity is much lower than L1 sensitivity, the Gaussian mechanism allows adding much less noise.

\iffalse
\section{\Name Privacy Gurantee for T rounds}
We are doing \Name for a sequence of $T$ rounds $\mathcal{F}_1,\dots,
\mathcal{F}_T$ where each $\mathcal{F}_t$ for $t \in [T]$ satisfies
the privacy gurantees stated above for different settings of \Name.
Now we invoke the strong composition theorem stated in
Lemma~\ref{lemma-PrivacyFold2} to obtain the privacy gurantee of the
\Name for $T$ rounds.  We can conclude that for any $\delta'>0$, \Name
is $(\varepsilon, \delta)$-DP for
\begin{equation}
	\varepsilon = \sqrt{2T\log{(1/\delta')}} \varepsilon_{\ell} + T \varepsilon_{\ell} (e^{\varepsilon_{\ell}}-1),  \delta=T \delta_{\ell}+ \delta'
\end{equation}
\fi


\section{Background}
\subsection{Robustness to poisoning attacks} 
Most of the distributed learning algorithms, including FedAvg~\cite{mcmahan2017communication}, 
operate on mutually untrusted clients and server. This makes distributed learning susceptible to the threat of poisoning~\cite{kairouz2019advances, shejwalkar2021back}. 
A \emph{poisoning adversary} can either own or control a few of FL clients, called \emph{malicious clients}, and instruct them to share malicious updates with the central server in order to reduce the performance of the global model. There are two approaches to poisoning FL: \emph{untargeted}~\cite{baruch2019a, fang2020local,shejwalkar2021manipulating} attacks aim to reduce the utility of global model on arbitrary test inputs; and \emph{backdoor}~\cite{bagdasaryan2020backdoor,wang2020attack, xie2019dba} attacks aim to reduce the utility on test inputs that contain a specific signal called the trigger.

In order to make FL robust to  the presence of such malicious clients, the literature has designed various \emph{robust aggregation rules (AGR)}~\cite{blanchard2017machine, DBLP:conf/icml/MhamdiGR18, YinCRB18,mozaffari2021fsl}, which aim to remove or attenuate the updates that are more likely to be malicious according to some criterion. For instance, Multi-krum~\cite{blanchard2017machine} repeatedly removes updates that are far from the geometric median of all the updates, and Trimmed-mean~\cite{YinCRB18} removes the largest and smallest values of each update dimension and calculates the mean of the remaining values.
It is not possible to use these AGRs in secure aggregation as the parameters are encrypted.

\subsection{Private Information Retrieval (PIR)}
Private information retrieval (PIR) is a technique to provide query
privacy to users when fetching sensitive records from untrusted
database servers.  That is, PIR enables users to query and retrieve
specific records from untrusted database server(s) in a way that the
servers cannot identify the records retrieved.  There are two major
types of PIR protocols. The first type is \emph{computational PIR}
(CPIR)~\cite{chang2004single} in which the security of the protocol
relies on the computational difficulty of solving a mathematical
problem in polynomial time by the servers, e.g., factorization of
large numbers. Most of the CPIR protocols are designed to be run by a
single database server, and therefore to minimize privacy leakage they
perform their heavy computations on the whole database (even if a
single entry has been queried). Most of these protocols use
homomorphic encryption (Section~\ref{sec:HE}) to make their queries
private.  The second major class of PIR is \emph{information-theoretic
  PIR} (ITPIR)~\cite{mozaffari2020heterogeneous}.  ITPIR protocols
provide information-theoretic security, however, existing designs need
to be run on more than one database servers, and they need to assume
that the servers do not collude.  Our work uses computational PIR
(cPIR) protocols to make the shuffling private.

\subsection{Homomorphic Encryption (HE)}\label{sec:HE}
Homomorphic encryption (HE) allows application of certain arithmetic
operations (e.g., addition or multiplication) on the ciphertexts
without decrypting them.  Many recent works~\cite{chang2004single}
advocate using partial HE, that only supports addition, to make the FL
aggregation secure.  In this section we describe two important HE
systems that we use in our paper.

\paragraphb{Paillier}
%Existing works~\cite{} use Paillier~\cite{paillier1999public} to
%provide secure aggregation in FL.
An additively homomorphic encryption system provides following
property:

\begin{equation}
  Enc(m_1) \circ Enc(m_2) = Enc(m_1 + m_2)
\end{equation}
where $\circ$ is a defined function on top of the ciphertexts. 

In these works, the clients encrypt their updates, send them to the
server, then the server can calculate their sum (using the $\circ$
operation) and sends back the encrypted results to the clients.  Now,
the clients can decrypt the global model locally and update their
models.  Using HE in these scenario does not produce any accuracy loss
because no noise will be added to the model parameters during the
encryption and decryption process.
%The process is as follows:
%\begin{itemize}
%	\item \emph{Key generation:} 
%	\item \emph{Encryption:} 
%	\item \emph{Decryption:} 
%\end{itemize}


\paragraphb{Thresholded Paillier}
In~\cite{damgaard2001generalisation}, the authors extend the Paillier
system and proposed a thresholded version.  In the thresholded
Paillier scheme, the secret key is divided to multiple shares, and
each share is given to a different participant.  Now each participant
can partially decrypt an encrypted message, but if less than a
threshold, say $t$, combine their partial decrypted values, they
cannot get any information about the real message.  On the other hand,
if we combine $\geq t$ partial decrypted values, we can recover the
secret.  In this system, the computations are in group
$\mathbb{Z}_{n^2}$ where $n$ is an RSA modulus.  The process is as
follows:

\begin{itemize}
\item \emph{Key generation:} First find two primes $p$ and $q$
  that statisfies $p=2p'+1$ and $q=2q'+1$ where $p',q'$ are
  also prime.  Now set the $n=pq$ and $m=p'q'$.  Pick $d$ such
  that $d=0\; \text{mod} \; m$ and $d=1 \; \text{mod} \;
  n^2$. Now the key server creates a polynomial
  $f(x)=\sum_{i=0}^{k-1} a_i x^i \; \text{mod} \; n^2m$ where
  $a_i$ are chosen randomly from $\mathbb{Z}^{*}_{n^2m}$ and
  the secret is hidden at $a_0=d$.  Now each secret key share
  is calculated as $s_i=f(i)$ for $\ell$ shareholders and the
  public key is $n$. For verification of correctness of
  decryption another public value $v$ is also generated where
  the verification key for each shareholder is $v_i=v^{\Delta
    s_i} \; \text{mod} \; n^2$ and $\Delta=\ell$.
\item \emph{Encryption:} For message $M$, a random number $r$
  is chosen from $\mathbb{Z}^{*}_{n^2}$ and the output
  ciphertext is $c=g^{M} \cdot r^{n^2} \; \text{mod} \; n^2$.
\item \emph{Share decryption:} The $i^{th}$ shareholder
  computes $c_i = c^{2 \Delta s_i}$ for ciphertext $c$. And
  for zero-knowlege proof, it provides $\log_{c^4}
  {(c_i^2)}=\log_{v} {(v_i)}$ which provides gurantee that the
  shareholder really uses its secret share for decryption
  $s_i$.
\item \emph{Share combining:} After collecting $k$ partial
  decryption, the server can combine them into the original
  plain-text message $M$ by $c'=\Pi_{i\in [k]}
  c_i^{2\lambda_{0,i}^S} \; \text{mod} \; n^2$ where
  $\lambda_{0,i}^S=\Delta \Pi_{i' \in [k] , i'\ne i}
  \frac{-i}{i-i'}$.  And use it to generate the $M$.
\end{itemize}


\section{Discussion and Future Work}
\label{sec:future-work}
\paragraphb{Utilizing recursion in cPIR.}  A solution to reduce the
number encryptions and upload bandwidth at the clients would be using
recursion in our cPIR.  In this technique, the dataset is represented
by a $k_3$-dimensional hypercube, and this allows the PIR client to
prepare and send $k_3 \sqrt[k_3]{d}$ encrypted values where $k_3$
would be another hyperparameter.  For future work, we can use this
technique and reduce the number of encryptions which makes the upload
bandwidth consumption lower too.  For instance, if we have one
shuffling pattern $k_2=1$, the number of encryption decreases from
$k_1 d$ to $ k_3 \sqrt[k_3]{k_1} d$.

\paragraphb{Plugging newer PIR protocol.}  \Name utilizes cPIR for
private aggregation, and in particular we use ~\cite{chang2004single}
which is based on Paillier. However, any other cPIR protocol can be
used in \Name. For example, SealPIR~\cite{angel2018pir} can be used to
reduce the number of encryptions at the client. SealPIR is based on a
SEAL which is a lattice based fully HE. The authors show how to
compress the PIR queries and achieve size reduction of up to
$274\times$. We defer analyzing \Name with other cPIR schemes to
future work.

\paragraphb{Combination of an external client shuffler for more
  privacy amplification.}  For further privacy amplification, we can
use an external shuffler that shuffles the $n$ sampled clients'
updates similar to FLAME~\cite{liu2021flame}.  For future work, we can
use double amplification by first shuffling the parameters at the
clients (i.e. , detaching the parameter values from their position)
and then shuffle the client's updates at the external shuffler (i.e.,
detaching the updates from their client’s ID).




%\section{Reproducibility Checklist}
%
%
%
%This paper:
%\begin{itemize}
%\item Includes a conceptual outline and/or pseudocode description of AI methods introduced: \textbf{yes}
%\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results: \textbf{yes}
%\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper: \textbf{yes}
%\item Does this paper make theoretical contributions? \textbf{yes} \\
%If yes, please complete the list below.
%\item All assumptions and restrictions are stated clearly and formally.  \textbf{yes}
%\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
%\item Proofs of all novel claims are included. (yes/partial/no)
%\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
%\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
%\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
%\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
%\item Does this paper rely on one or more datasets? (yes/no)
%\item If yes, please complete the list below.
%\item A motivation is given for why the experiments are conducted on the selected datasets. (yes/partial/no/NA)
%\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)
%\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
%\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)
%\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)
%\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)
%\end{itemize}




\iffalse

\section{Private Information Retrieval (PIR)}
PIR algorithms have been suggested to be used in various application scenarios involving  untrusted database servers~\cite{olumofin2010privacy,mittal2011pir,gupta2016scalable,pir-ecommerce,hafiz2017querying,cappos2013avoiding,borisov2015dp5,piotrowska2017annotify,li2017rpir}, from retrieving Tor relay information~\cite{mittal2011pir} to privacy-preserving querying of location services~\cite{ghinita2008private} to registering Internet domains~\cite{olumofin2010privacy}. 



 Private information retrieval (PIR) is a technique to provide query privacy to users when fetching sensitive records from untrusted databases. 
There are two major types of PIR protocols. The first type is \emph{computational PIR} (CPIR)~\cite{chor1997computationally, kushilevitz1997replication, aguilar2007lattice, aguilar2016xpir, brakerski2014efficient, cachin1999computationally, dong2014fast, kiayias2015optimal, lipmaa2017simpler, stern1998new, angel2018pir} in which the security of the protocol relies on the computational difficulty of  solving a mathematical problem in polynomial time by the servers, e.g., factorization of large numbers. Most of the CPIR protocols are designed to be run by a single database server, and therefore to  minimize privacy leakage they  perform their heavy computations on the whole database (even if a single entry has been queried). Consequently, existing CPIR protocols suffer from very high computation overheads. 
 The second major class of PIR is \emph{information-theoretic PIR} (ITPIR)~\cite{demmler2014raid,henry2013one, beimel2002robust, chor1995private, gertner1998random, goldberg2007improving, beimel2002breaking, devet2012optimally}. ITPIR protocols provide information-theoretic security, however,  existing designs need to be run on more than one database servers, and they need to assume that the servers do not collude. Existing ITPIR protocols impose lower computation overheads compared to CPIR algorithms, but at the price of requiring the non-collusion assumption for the servers. Therefore, (multi-server) ITPIR protocols are best fit to scenarios involving multiple (potentially competing) data owners who collaborate to run a service privately, therefore colluding is not in their best interest, e.g., \cite{li2017rpir, mittal2011pir, borisov2015dp5}. Our work focuses on this class of  PIR, i.e., multi-server PIR protocols. 


\paragraphb{Computational PIR (CPIR) protocols}
Most of CPIR protocols use a single server which is computationally bounded for retrieving data. It means the security of these protocols is based on a very difficult mathematical problem, and if the adversary finds a solution for the problem, or if she has enough time and computation resources, some data will be leaked. 

\paragraphb{Stern et al.\ CPIR} Stern et al.~\cite{stern1998new} propose a CPIR protocol that its algorithm is based on additively homomorphic cryptosystem which has these functions: (i) $Gen$: function of generating public and private keys $pk, sk$ and system parameters , (ii) $Enc$: Encryption function with public key ,and (iii) $Dec$: Decryption function. 

The important point in this scheme is that the cryptosystem is non-deterministic i.e. the $Enc$ is a randomize function that encrypts the same input to different output each time. $Dec$ function will cancel the effect of the random variable that was used in $Enc$ function. The most famous non-deterministic cryptosystem that is used for CPIR is Paillier~\cite{paillier1999public}. 

XPIR~\cite{aguilar2016xpir} proposes a new CPIR based on this protocol by looking at each record of the database as a polynomial (the elements of the databases are encoded as coefficients of the polynomial). However, the bandwidth consumption is not very good, so SealPIR~\cite{angel2018pir} introduce a way to compress the queries in this system.

\paragraphb{Kushilevitz and Ostrovsky CPIR} \label{app:kush}
One of the merits of CPIR is that the client can run the protocol recursively to reduce the bandwidth consumption. This idea was used by Kushilevitz and Ostrovsky~\cite{kushilevitz1997replication} in their scheme for improving the communication cost. First, they split the database into several virtual blocks, and each one of these blocks contains some of the real blocks, then the client sends her query for a specific virtual block, then server will calculate the result of that query on the database and will look at the result as a new database, the next query will be applied to this temporary database, and this process continues until one vector of size $s$ will be sent to the client, and client can recover her requested index out of this result.





\section{Poisoning Attacks and Byzanthine-Robust Aggregation Rules in FL}
FL involves mutually untrusting  clients. 
Hence, a \emph{poisoning adversary} may own or compromise some of the FL clients, called \emph{malicious clients}, with the goal of mounting a \emph{targeted} or \emph{untargeted} poisoning attack. In a targeted attack~\cite{bhagoji2019analyzing, sun2019can}, the goal is to reduce the utility of the model on specific test inputs, while in the untargeted attack~\cite{baruch2019a, fang2020local,shejwalkar2021manipulating}, the goal is to reduce the utility for all (or most)  test inputs. It is shown~\cite{blanchard2017machine} that even a single malicious client can mount an effective untargeted attack on FedAvg. 

In order to make FL robust to  the presence of such malicious clients, the literature has designed various \emph{robust aggregation rules (AGR)}~\cite{blanchard2017machine, DBLP:conf/icml/MhamdiGR18, YinCRB18,chang2019cronus}, which aim to remove or attenuate the updates that are more likely to be malicious according to some criterion. For instance, Multi-krum~\cite{blanchard2017machine} repeatedly removes updates that are far from the geometric median of all the updates, and Trimmed-mean~\cite{YinCRB18} removes the largest and smallest values of each update dimension and calculates the mean of the remaining values.
% 
% In order to make FL robust to  the presence of such malicious clients, the literature has proposed multiple aggregation rules (AGRs)~\citep{blanchard2017machine,mhamdi2018the,xie2018generalized,diakonikolas2019sever} with theoretical robustness guarantees. 
Unfortunately, these robust AGRs are not very effective in  non-convex FL settings and multiple works have demonstrated strong targeted~\cite{wang2020attack,bhagoji2019analyzing} and untargeted attacks~\cite{shejwalkar2021manipulating,fang2020local} on them.

\fi



==> test_dir/FedPerm/bg.tex <==
\section{Preliminaries}

%To provide privacy guarantees in FL, different \emph{differentially
%  private federated learning} algorithms has been introduced.
%  Differential Privacy provides statistical guarantees for the
%  leaking information that an adversary can infer by inspecting the
%  output of a randomized mechanism.  In this section, we first
%  describe different FL algorithms (illustrated in
%  Figure~\ref{fig:allDP}), and then introduce properties we use
%  throughout the paper.  Table~\ref{table:notation} shows the
%  notations we use in this paper.

%We now present existing FL algorithms (see Figure~\ref{fig:allDP}),
%and their properties that are relevant to \Name{}'s design.
%Table~\ref{table:notation} shows the notations we use in this paper.

%\subsection{Notations}



\begin{comment}
\begin{table}
\centering
\small
{\footnotesize
\caption{List of notations}
\label{table:notation}
\begin{tabular}{ |c|c| }
\hline
$\mathcal{A}$ & Analyzer (e.g. FL server)\\
\hline
$\mathcal{R}$ & Randomizer function \\
\hline
$\mathcal{S}$ & Shuffler \\
\hline
$N$ & Total number of clients participating in FL \\
\hline
$n$ & Number of selected clients in each round of FL \\
\hline
$d$ & Number of parameters in Model \\
\hline 
$x_i$ & Local update for $i^{th}$ client $\in \mathbb{R}^d$\\
\hline
$k_1$ & Window size \\
\hline 
$k_2$ & Number of shuffling Patterns\\
\hline
 $\mathcal{S}_{k_1}^{k_2}$ & {\vtop{\hbox{\strut Shuffling function with $k_2$ shuffling patterns}\hbox{\strut each pattern consits of $k_1$ indices}}} \\
\hline
%$\mathcal{S}_{k_1}^{k_2}$ & Shuffling function with $k_2$ shuffling patterns each consits of $k_1$ indices. \\
%\hline
$\pi$ & Shuffling pattern\\
\hline
$\varepsilon_{\ell}$ & Local differential privacy budget after amplification\\
\hline
$\varepsilon_{d}$ & Local differential privacy budget before amplification\\
\hline
%$E$ & Number of local epochs\\
%\hline
%$T$ & Number of global rounds\\
%\hline
%$\eta$ & Local learning rate\\
%\hline
\end{tabular}
}
\end{table}
\end{comment}






%/subsection{Secure Aggregation in FL} Secure
%aggregation~\cite{bonawitz2017practical} is proposed to limit the
%server inferences from the local updates, i.e., the server is only
%learning the aggregated updates and not learning anything from the
%clients' updates.





%\section{Federated Learning with Differential Privacy} We first
%illustrate how existing differential private federated learning work
%in Figure~\ref{fig:allDP}, and then introduce properties that will be
%used throughout the paper.  To provide privacy guarantees in FL,
%different \emph{differentially private federated learning} algorithms
%has been introduced.  Differential Privacy provides statistical
%guarantees for the leaking information that an adversary can infer by
%inspecting the output of a randomized mechanism.
%############Existing DP-FL works########### The existing works are
%categorized in three groups: \textbf{(1)} \emph{Centralized
%differentially private FL (CDP-FL)}~\cite{mcmahan2018learning,
%geyer2017differential} in which the clients send their raw model
%updates to a trusted server, and the server aggregates them into a
%global model and randomizes the global model.  \textbf{(2)}
%\emph{Locally differentially private FL
%(LDP-FL)}~\cite{wang2019collecting, liu2020fedsel} in which each
%client randomizes its local update before sending then to an
%untrusted server.  The CDP-FL provides better utility with cost of
%trusting the server, but the LDP-FL preserves strong local privacy
%with cost of low utility.  \textbf{(3)} \emph{Differentially private
%FL by shuffling updates
%(DP-FL-S)}~\cite{girgis2021shuffled,liu2021flame} in which.


\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{Images/Fedperm1.pdf} 
\vspace{-0.1in}
\caption{Different models of differential privacy in Federated
  Learning. Red dots are showing the trust boundaries.}
\label{fig:allDP}
\end{figure}


%\subsection{Non-Private Federated Learning (FL)}
In FL~\cite{mcmahan2017communication, kairouz2019advances,
  konevcny2016federated}, $N$ clients collaborate to train a global
model without directly sharing their data.  In round $t$, the
federation server samples $n$ out of $N$ total clients and sends them
the most recent global model $\theta^t$. Each client re-trains
$\theta^t$ on its private data
%starting from the $\theta^t$
using stochastic gradient descent (SGD), and sends back the model
parameter updates ($x_i$ for $i^{th}$ client) to the server. The
server then aggregates (e.g., averages) the collected parameter
updates
%($x_i$ for $i \in [n]$)
and updates the global model for the next round ($\theta^t \gets
\theta^{t-1} + \frac{1}{n} \sum_{i=1}^n x_i$).
%  FL can be either cross-device or
%cross-silo~\cite{kairouz2019advances}. In cross-device FL, N is large
%(from few thousands to billions) and only a small fraction of clients
%is chosen in each FL training round, i.e., $n \ll N$. By contrast, in
%cross-silo FL, N is moderate (up to 100) and all clients are chosen
%in each round, i.e., $n = N$.  In this work, we evaluate the
%performance of \Name and other FL baselines for both cross-device and
%cross-silo FL under realistic production FL settings.


\subsection{Central Differential Privacy in FL (CDP-FL)}
In CDP-FL~\cite{mcmahan2018learning, geyer2017differential},
illustrated in Figure~\ref{fig:allDP}(a) , a \emph{trusted} server
first collects all the clients' raw model updates ($x_i \in
\mathbb{R}^d$), aggregates them into the global model, and then
perturbs the model with carefully calibrated noise to enforce
differential privacy (DP) guarantees.  The server provides
participant-level DP by the perturbation.  Formally, consider
\emph{adjacent} datasets ($X, X' \in \mathbb{R}^{n\times d}$) that
differ from each other by the data of one federation client.  Then:

%The privacy goal of CDP-FL is providing indistinguishability for any
%outputs for all the neighboring datasets ($X, X' \in
%\mathbb{R}^{n\times d}$) that are different by replacing one user's
%data.  Following definition shows this goal:

\begin{definition} [Centralized Differential Privacy (CDP)]
A randomized mechanism $\mathcal{M}: \mathcal{X} \rightarrow
\mathcal{Y}$ is said to be $(\varepsilon, \delta)$-differential
private if for any two adjacent datasets $X, X' \in \mathcal{X}$, and
any set $Y \subseteq \mathcal{Y}$:
\begin{equation}
\Pr [\mathcal{M}(X) \in Y] \leq e^{\varepsilon} \Pr [\mathcal{M}(X')
  \in Y] +\delta
\end{equation}
\end{definition}
where $\varepsilon$ is the privacy budget (lower the $\varepsilon$,
higher the privacy), and $\delta$ is the failure probability.



\subsection{Local Differential Privacy in FL (LDP-FL)}
%\red{ in which each client randomizes its local update before sending
%then to an untrusted server.  The CDP-FL provides better utility with
%cost of trusting the server, but the LDP-FL preserves strong local
%privacy with cost of low utility.}
CDP-FL relies on availability of a trusted server for collecting raw
model updates.  On the other hand, LDP-FL~\cite{wang2019collecting,
  liu2020fedsel} does not rely on this assumption and each client
perturbs its output locally using a randomizer $\mathcal{R}$
(Figure~\ref{fig:allDP}(b)).  If each client perturbs its model
updates locally by $\mathcal{R}$ which satisfies $(\varepsilon_{\ell},
\delta_{\ell})$-LDP, then observing collected updates
$\{\mathcal{R}(x_1), \dots, \mathcal{R}(x_n)\}$ also implies
$(\varepsilon_{\ell}, \delta_{\ell})$-DP~\cite{dwork2014algorithmic}.

\begin{definition} [Local Differential Privacy (LDP)]
A randomized mechanism $\mathcal{R}: \mathcal{X} \rightarrow
\mathcal{Y}$ is said to be $(\varepsilon_{\ell},
\delta_{\ell})$-locally differential private if for any two inputs $x,
x' \in \mathcal{X}$ and any output $y \in \mathcal{Y}$,:
\begin{equation}
\Pr [\mathcal{R}(x) = y] \leq e^{\varepsilon_{\ell}} \Pr
    [\mathcal{R}(x') = y] +\delta_{\ell}
\end{equation}
\end{definition}

In LDP-FL, each client perturbs its local update ($x_i$) with
$\epsilon_{\ell}$-LDP.  Unfortunately, LDP hurts the utility,
especially for high dimensional vectors.  Its mean estimation error is
bounded by $O(\frac{\sqrt{d \log{d}}}{\varepsilon_{\ell} \sqrt{n}})$
meaning that for better utility we should increase the privacy budget
or use larger number of users in each
round~\cite{bhowmick2018protection}.



\subsection{Privacy Amplification by Shuffling Clients' updates}
Recent works~\cite{liu2021flame, girgis2021shuffled} utilize the
privacy amplification effect by shuffling model parameters across
client model updates from participating clients to improve the LDP-FL
utility (illustrated in Figure~\ref{fig:allDP}(c)).  FL frameworks
based on shuffling clients' updates consists of three building
processes: $\mathcal{M}=\mathcal{A} \circ \mathcal{S} \circ
\mathcal{R}$.  Specifically, they introduce a shuffler $\mathcal{S}$,
which sits between the FL clients and the FL server, and it shuffles
the locally perturbed updates (by randomizer $\mathcal{R}$) before
sending them to the server for aggregation ($\mathcal{A}$).  More
specifically, given parameter index $i$, $\mathcal{S}$ randomly
shuffles the $i^{th}$ parameters of model updates received from the
$n$ participant clients.  The shuffler thus detaches the model updates
from their origin client (i.e. anonymizes them).  Previous
works~\cite{balle2019differentially, balcer2019separating,
  ghazi2019scalable} focused on shuffling one-dimensional data $x \in
X$, and corollary~\ref{coll-blanket-balle-generic} shows the privacy
amplification effect by shuffling.
%But Recent works~\cite{liu2021flame, girgis2021shuffled} use
%shuffling in FL for privacy amplification.  SLDP-FL introduces a
%shuffler, which sits between the FL clients and the FL server, and it
%shuffles the locally randomized updates before sending them to the
%server.  in SLDP-FL, The shuffler detaches the model updates from
%their origin client (i.e. anonymizes them).


%\begin{lemma}~\cite{balle2019privacy}
%For $\sqrt{\frac{14 \log{(2/\delta_c)}(b-1)}{n-1}}<\varepsilon_c\leq 1$,
%if $R_{\gamma,b}$ satisfies $\varepsilon_{\ell}$-LDP, we have $(\varepsilon_{c}, \delta_{c})$ 
%for shuffling the randomized outputs where $\varepsilon_c = \sqrt{\frac{14 \log{(2/\delta_c)} (e^{\varepsilon_\ell}+b-1)}{n-1}}$
%\label{thm-blanket-balle-radnomizerR}
%\end{lemma}

\begin{corollary}~\cite{balle2019privacy}
In shuffle model, if $R$ is $\varepsilon_{\ell}$-LDP, where
$\varepsilon_{\ell} \leq \log{(n / \log{(1/\delta_c)})}/2$.  $M$
statisfies $(\varepsilon_{c}, \delta_{c})$-DP with $\varepsilon_{c}=O(
(1 \wedge \varepsilon_{\ell}) e^{\varepsilon_{\ell}}
\sqrt{\log{(1/\delta_c)}/n})$ where '$\wedge$' shows minimum function.
\label{coll-blanket-balle-generic}
\end{corollary}


From above corollary, the privacy amplification has a direct
relationship with $\sqrt{n}$ where $n$ is the number of selected
clients for aggregation, i.e., increasing the number of clients will
increase the privacy amplification.  Note that in \Name, the clients
are responsible for shuffling, and instead of shuffling the $n$
clients' updates (inter-model shuffling), each client locally shuffles
its $d$ parameters (intra-model shuffling).  In real-world settings
there is a limit on the value of $n$, so the amount of amplification
we can achieve is also limited.  However, in \Name we can see much
more amplification because we are shuffling the parameters and $n \ll
d$.





\subsection{Privacy Composition}
We use following naive and strong composition
theorems~\cite{dwork2010boosting} in this paper:

\begin{lemma}[N{\"a}ive Composition]
$\forall \varepsilon \geq 0, t \in \mathbb{N}$, the family of $\varepsilon$-DP mechanism 
satisfies $t\varepsilon$-DP under $t$-fold adaptive composition.
\label{lemma-PrivacyFold1}
\end{lemma}

\begin{lemma}[Strong Composition]
$\forall \varepsilon, \delta, \delta' > 0, t \in \mathbb{N}$, the family of $(\varepsilon, \delta)$-DP mechanism satisfies
$(\sqrt{2t \ln{(1/\delta'})} \cdot \varepsilon + t \cdot \varepsilon (e^{\varepsilon} - 1), t \delta + \delta' )$-DP
under $t$-fold adaptive composition. 
\label{lemma-PrivacyFold2}

\end{lemma}




==> test_dir/FedPerm/intro.tex <==
\section{Introduction}
Federated Learning (FL) is a distributed learning paradigm where
mutually untrusting \emph{clients} collaborate to train a shared
model, called the \emph{global model}, without explicitly sharing
their local training data. FL training involves a \emph{server} that
aggregates, using an \emph{aggregation rule} (AGR), model updates that
the clients compute using their local private data.  The aggregated
\emph{global model} is thereafter broadcasted by the server to a
subset of the clients.  This process repeats for several rounds until
convergence or a threshold number of rounds.  Though highly promising,
FL faces multiple challenges~\cite{kairouz2019advances} to its
practical deployment.  Two of these challenges are (i) data privacy
for clients' training data, and (ii) robustness of the global model in
the presence of malicious clients.

The data privacy challenge emerges from the fact that raw model
updates of federation clients are susceptible to privacy attacks by an
adversarial server as demonstrated by several recent
works~\cite{li2022,lim2021,nasr2019comprehensive,wei2020,zhu2019deep}.
Two classes of approaches can address this problem in significantly
different ways: First, \emph{Local Differential
  Privacy}~\cite{duchi13,kasiviswanathan08,truex20,warner65} in FL
(LDP-FL) enforces a strict theoretical privacy guarantee to model
updates of clients.  The guarantee is enforced by applying carefully
calibrated noise to the clients' local model updates using a local
randomizer $\mathcal{R}$.  In addition to the privacy guarantee,
LDP-FL can defend against poisoning attacks by malicious clients, thus
providing robustness to the global model
~\cite{nguyen2021flame,naseri2020local,sun2019can}.  However, the
model update perturbation needed for the LDP guarantee significantly
degrades model utility.

The other approach to enforce client data privacy is \emph{secure
  aggregation (sAGR)}, where model update aggregation is done using
cryptographic techniques such as homomorphic encryption or secure
multi-party computation~\cite{bonawitz2017practical,
  zhang2020batchcrypt, bell2020secure,fereidooni2021safelearn}.  sAGR
protects privacy of clients' data from an adversarial server because
the server sees just the encrypted version of clients' model updates.
Moreover, this privacy is enforced without compromising global model
utility.  However, the encrypted model updates themselves provide the
perfect cover for a malicious client to poison the global
model~\cite{fereidooni2021safelearn, nguyen2021flame} -- the server
cannot tell the difference between a honest model update and a
poisoned one since both are encrypted.
\begin{comment}
%So perhaps we can remove it or demote it to a footnote.
Furthermore, the trained model
remains susceptible to \emph{inference attacks}~\vjm{Citations
  needed}.
\end{comment}

\begin{comment}
It has been shown that sharing raw local updates with an
\emph{untrusted} server compromises clients'
privacy~\cite{nasr2019comprehensive, zhu2019deep}.  To provide local
privacy guarantees in FL against the untrusted server, two main
approaches are suggested: \emph{Locally differentially private
  federated learning (LDP-FL)}~\cite{wang2019collecting,
  liu2020fedsel} and \emph{secure aggregation
  (sAGR)}~\cite{bonawitz2017practical}.  In LDP-FL, each client
perturbs its local update by applying a randomize function
$\mathcal{R}$ which is $\varepsilon_d$-LDP, before sending to the
untrusted server.  Secure aggregation is also proposed to limit the
server inferences from the local updates, i.e., the server is only
learning the aggregated updates and not learning anything from the
clients' updates.  Secure aggregation can be achieved using different
techniques such as fully or partially homomorphic encryption or secret
sharing.  LDP-FL provides formal privacy guarantee, and it has been
shown~\cite{naseri2020local,sun2019can} that LDP-FL can defend against
poisoning attacks.  However, LDP-FL is notorious for low utility, and
this results in significant accuracy drop in the final trained model.
On the other hand, secure aggregation provides good accuracy, but it
is vulnerable to poisoning attacks as the server cannot utilize any
robust AGR to exclude the malicious poisoning updates from
aggregation.
\end{comment}

%############Fedperm###########
In this paper we answer the dual question: \emph{Can we design an
  efficient federated learning algorithm that achieves local privacy
  for participating clients at a low utility cost, while ensuring
  robustness of the global model from malicious clients?}
%The key question we try to answer is: \emph{Can we design an efficient
%  federated learning algorithm that achieves both local privacy and
%  robustness?}
To that end, we present \emph{\Name}, a new FL protocol that combines
LDP~\cite{duchi13,kasiviswanathan08,warner65}, model parameter
shuffling~\cite{erlingsson2019amplification}, and \emph{computational
  Private Information Retrieval
  (cPIR)}~\cite{chor1997computationally,chang2004single,
  aguilar2016xpir, angel2018pir}
%based techniques 
in a novel way to achieve our dual goals.
%of (i) high accuracy of secure aggregation while enforcing strong
%privacy guarantees (LDP), and (ii) robustness from model poisoning
%attacks.

The starting point of \Name{}'s design is \emph{privacy amplification
  by shuffling}~\cite{erlingsson2019amplification}, which enables
stronger (i.e., amplified) privacy with little model perturbation
(using randomizer $\mathcal{R}$) at each client.  Crucially, our
shuffling technique fundamentally differs from prior works in that we
apply \emph{intra-model} parameter shuffling rather that the
\emph{inter-model} parameter shuffling done
previously~\cite{erlingsson2019amplification,liu2021flame,
  girgis2021shuffled}.
%% indicates the
%% shuffled outputs of local randomizers provides stronger (i.e.,
%% amplified) privacy.  This means that each client needs to inject
%% smaller amount of local noise (through $\mathcal{R}$) for the same
%% final level of privacy which compensates the LDP poor utility.  In
%% this work, we provide theoretical analysis and numerical evaluations
%% of the privacy amplification by shuffling parameters in \Name.



Next, each \Name client privately chooses its \emph{shuffling pattern}
uniformly at random for each FL round.  To aggregate the shuffled (and
perturbed) model parameters, \Name client utilizes cPIR to generate a
set of PIR queries for its shuffling pattern that allows the server to
retrieve each parameter \emph{privately} during aggregation.  All the
server observes is the shuffled parameters of the model update for
each participating client, and a series of PIR queries (i.e., the
encrypted version of the shuffling patterns).  The server can
aggregate the PIR queries and their corresponding shuffled parameters
for multiple clients to get the encrypted aggregated model.  The
aggregated model is decrypted independently at each client.
%We propose different methods to decrypt the encrypted aggregated
%model based on assumptions about the underlying threat models.


\begin{comment}
utilizes a cPIR technique based on partial homomorphic encryption
(PHE)~\cite{paillier1999public, damgaard2001generalisation} that allows the server to retrieve
each parameter privately during aggregation.  All the server observes
is the shuffled parameters of the model for each participating client,
and an encrypted version of the \emph{unshuffled} parameters that is
retrieved using the cPIR technique~\vjm{Is there a name for the
  technique?}.  The server can aggregate the encrypted unshuffled
parameters of multiple clients to get the encrypted aggregated model.
We propose different  methods to decrypt the encrypted
aggregated model based on assumptions about the underlying threat
models.
\end{comment}

The combination of LDP at each client and intra-model parameter
shuffling achieves enough privacy amplification to let \Name\ preserve
high model utility.  At the same time, availability of the shuffled
parameters at the federation server lets it control a client's model
update contribution by enforcing norm-bounding, which is known to be
highly effective against model poisoning
attacks~\cite{nguyen2021flame,naseri2020local,sun2019can}.



Since \Name\ utilizes cPIR which relies on homomorphic encryption
(HE)~\cite{paillier1999public, damgaard2001generalisation}, it can be
computationally expensive, particularly for large models.  We present
computation/utility trade off hyper-parameters in \Name, that enables
us to achieve an interesting trade off between computational
efficiency and model utility.  In particular, we can adjust the
computation burden for a proper utility goal by altering the size and
number of shuffling patterns for the \Name clients.

\begin{comment}
Since \Name\ relies on PHE, it can be computationally expensive,
particularly for large models.  We present two additional variants of
\Name, called \emph{\Name-light} and \emph{\Name-heavy}, that achieve
an interesting trade off between computational efficiency and model
utility.  We continue to enforce the same privacy guarantee and model
robustness in both these variants.
\end{comment}

%Private information retrieval (PIR) is a technique to provide query
%privacy to users when fetching sensitive records from untrusted
%databases~\vjm{[Reference needed here]}.  That is, cPIR enables users
%to query and retrieve specific records from untrusted database in a
%way that the serving database cannot identify the records
%retrieved~\vjm{Presumably the cPIR reference covers this, if not
%please provide the pertinent reference}.

\begin{comment}
Operationally, in each round of \Name, clients (\emph{i}) learn their
local updates, (\emph{ii}) perturb their updates using a randomizer
$\mathcal{R}$ that provides $\varepsilon_{d}$-LDP guarantee,
(\emph{iii}) shuffle the parameters inside their randomized updates,
(\emph{iv}) create a cPIR query to retrieve each parameter privately
in the shuffled update, and (\emph{v}) send their shuffled update and
PIR query to the \Name server.  After collecting all the local updates
from the clients, the \Name server
%first checks the norm of each update to avoid poisoning attacks and then
aggregates the local updates and produces the global update for next
round.  Since this aggregated global update is encrypted, we proposed
different methods to decrypt it based on assumptions about the
underlying threat models.
\end{comment}

%After collecting all the all the shuffled updates and their cPIR
%queries from the clients, the \Name server (\emph{i}) checks the norm
%of each update to avoid poisoning attacks, (\emph{ii}) multiplies
%each clients query to its shuffled parameters to find its unshuffled
%encrypted update, (\emph{iii}) sums all the encrypted unshuffled
%parameters to find the encrypted global model which can be decrypted
%by the clients.


%############Intuituions###########
%\paragraphb{\em Intuitions on \Name's privacy amplification:} Each
%\Name client, first applies a randomize function $\mathcal{R}$ which
%is $\varepsilon_d$-LDP on its parameters, and then shuffles them
%before sending them to the server.

\begin{comment}
\paragraphb{\em Intuitions on \Name's robustness to poisoning
  attacks:} In traditional FL algorithms with secure aggregation, the
local updates are encrypted, providing malicious clients a significant
flexibility in fabricating poisoning updates.  It is
shown~\cite{blanchard2017machine} that even a single malicious client
can mount an effective untargeted attack on FedAvg by sending very
large parameters in its local update.  By contrast, \Name clients
provide their actual parameter values, without any encryption or
obfuscation, but in a shuffled order that each parameter is detached
from its position, which allows the server to check the norm of
updates before aggregating them into the global model. Please note
that unlike other robust AGRs, \emph{norm bounding} (what we have in
DP) is the only robust AGR that only needs the values of the update
parameters without access to their order by calculating the
$\bar{x_i}\gets x_i \cdot \min(1, \frac{C}{{||x_i||}_2})$ where $x_i$
is the local update vector and $C$ the maximum $\ell_2$ norm possible.
\end{comment}

%############empirical results###########
%\paragraphb{\em Empirical results:}
%We provide a formal analysis of our algorithms' privacy guarantees.
We empirically evaluate \Name on the MNIST dataset to demonstrate that
it is possible to provide LDP-FL guarantees at low model utility cost.
%with only negligible cost in final test accuracy by leveraging the
%privacy amplification effect of shuffling parameters.
We theoretically and numerically demonstrate a trade off between model
utility and computational efficiency. Specifically, \Name's
hyperparameters create \emph{shuffling windows} whose size can be
reduced to drastically cut computation overheads, but at the cost of
reducing model utility due to lower privacy amplification.  We
experiment with two representative shuffling window configurations in
\Name -- ``light'' and ``heavy''.  For a $(4.0, 10^{-5})$-LDP
guarantee, the light version of \Name, where client encryption, and
server aggregation needs $52.2$ seconds and $21$ minutes respectively,
results in a model that delivers $32.85\%$ test accuracy on MNIST.
The heavier version of \Name, where client encryption and server
aggregation needs $32.1$ minutes and $16.4$ hours respectively,
results in $72.38\%$ test accuracy.  Non-private FedAvg, CDP-FL and
LDP-FL provide $91.02\%$, $53.50\%$, and $13.74\%$ test accuracies for
the same $(\varepsilon, \delta)$-DP guarantee respectively.





\iffalse
In summary, we propose a federated learning approach that is built on using private information retrieval (PIR), 
Our key contributions are as follows:
\begin{itemize}
\item We propose the first secure aggregation protocol, \Name, by shuffling the parameters and utilizing PIR for aggregating shuffled updates.
\item We show that \Name significantly reduces the 
\item 
\item We evaluate \Name on the real-world benchmark dataset (MNIST), and show that 
\end{itemize}
\fi









